Input to the ESPPU: The LUXE Experiment

This document presents an overview of LUXE (Laser Und XFEL Experiment), an experiment that will combine the high-quality and high-energy electron beam of the European XFEL with a high-intensity laser, to explore the uncharted terrain of strong-field quantum electrodynamics. The scientific case, facility, and detector setup are presented together with an overview of the foreseen timeline and expected capital costs.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document

# Copyright (C) 2002-2022 CERN for the benefit of the ATLAS collaboration
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to remove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_pdflatex instead of run_latexmk to use explicit
# pdflatex/biber commands to compile.

# You can use the target version to check your TeX Live version.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2020
LATEX    = latex
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf
TLVERS   = $(shell pdflatex --version | grep -Go 'TeX Live [0-9]*' | grep -Go '[0-9].*')
# TLOKAY   = $(shell test $(TLVERS) -ge $(TEXLIVE) && echo true)
TWIKI    = https://twiki.cern.ch/twiki/bin/view/AtlasProtected/PubComLaTeXFAQ

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = mydocument

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with latexmk.
default: run_latexmk
# Use pdflatex/biber instead to compile.
# default: run_pdflatex

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: version clean cleanpdf help

# Check TeX Live version
version:
	@echo "Checking version"
	@echo "TLVERS $(TLVERS), TEXLIVE $(TEXLIVE)"
	if [ $(TLVERS) -lt $(TEXLIVE) ]; then \
		echo "Your TeX Live version ($(TLVERS)) is older than $(TEXLIVE). Please consult $(TWIKI)"; \
	fi

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bib/*.bib
%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata newauxmat

newpapertexmf: TEMPLATE=atlas-paper
newpapertexmf: newdocumenttexmf newfiles newpapermetadata newauxmat

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

newnotetexmf: TEMPLATE=atlas-note
newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

newbooktexmf: TEMPLATE=atlas-book
newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex \
	  >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

newdata:
	sed s/atlas-document/$(BASENAME)/ template/atlas-hepdata-main.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-hepdata-main.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

newdocument:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newdocumenttexmf:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' | \
	  sed 's/\\RequirePackage{latex\/atlaslatexpath}/% \\RequirePackage{latex\/atlaslatexpath}/' \
	  >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	# touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newauxmat:
	cp template/atlas-auxmat.tex $(BASENAME)-auxmat.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make run_latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for HepData material give the commands:"
	@echo "make newdata [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-hepdata-main"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo "make version to check your TeX Live version"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.lof *.lot *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx *.tdo \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp

cleanpdf:
	-rm $(BASENAME).pdf
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-hepdata-main.pdf

cleanps:
	-rm $(BASENAME).ps
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-hepdata-main.ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^


==> authorlists/authorlist-inst.tex <==
\setcounter{Maxaffil}{2000} 
 \author{ I.~Levy}
 \affil {Department of Physics, Nuclear Research Centre-Negev, P.O. Box 9001, Beer Sheva 84190, Israel}
\author{N.~Cavanagh}
\author{K.~Fleck}
\author{G.~Sarri}
\author{M.~Streeter}
\affil{School of Mathematics and Physics, The Queen’s University of Belfast, BT7 1NN, Belfast, United Kingdom}
\author{M.~Bruschi}
\author{A.~Sbrizzi}
\affil{INFN, Bologna, Italy}
\author{U.~Acosta}
\author{B.~K{\"a}mpfer}
\affil{ Helmholtz-Zentrum Dresden-Rossendorf, 01328 Dresden, Germany\\
{\rm and}\\
TU~Dresden, 01062 Dresden, Germany}
\author{M.~Gostkin}
\author{A.I.~Titov}
\author{A.~Zhemchugov}
\affil{ Joint Institute for Nuclear Research ( JINR), Dubna 141980, Russia} 
\author{F.~Qu\'er\'e}
  \affil{LIDYL, CEA, CNRS, Universit\'e Paris-Saclay, CEA Saclay, 91 191 Gif-sur-Yvette, France}
\author{T.~Blackburn}
\affil{University of Gothenburg, SE-41296 Gothenburg, Sweden}
 \author{T.~Ma}
\author{Y.~Soreq}
  \affil{Physics Department, Technion—Israel Institute of Technology, Haifa 3200003, Israel}
  \author{M.~Altarelli}
  \affil{Max Planck Institute for Structure and Dynamics of Matter, Hamburg, 22761, Germany}
\author{R.~A{\ss}mann}
\author{T.~Behnke}
\author{O.~Borysov}
\author{R.~Brinkmann}
\author{F.~Burkart}
\author{K.~B{\"u}{\ss}er}
\author{W.~Decking}
%\author{B.~Heinemann$^{a,b}$}
\author{B.~Heinemann\footnote {\bf corresponding author: beate.heinemann@desy.de} \footnote{also at Albert-Ludwigs-Universit{\"a}t-Freiburg}}
\author{L.~Helary}
\author{M.~Hoffmann}
\author{X.~Huang}
\author{R.~Jacobs}
\author{J.~List}
%\author{W.~Lohmann$^{c}$}
\author{W.~Lohmann\footnote{also at BTU, Cottbus and RWTH, Aachen}}
\author{E.~Negodin}
\author{R.~Prasad}
\author{A.~Ringwald}
\author{S.~Schmitt}
\author{S.~Schuwalow}
\author{M.~Shchedrolosiev}
\author{D.~Thoden}
   \affil{Deutsches Elektronen-Synchrotron (DESY), Hamburg, 22607, Germany} 

%\author{M.~Zepf $^{d}$}
\author{M.~Zepf \footnote{also at Helmholtz Institut Jena,  07743 Jena, Germany}}
  \affil{Friedrich Schiller Universit{\"a}t Jena, Jena, 07743, Germany}
\author{A.~S{\"a}vert}
\author{D.~Seipt}
\author{T.~Teter}
  \affil{Helmholtz Institut Jena,  07743 Jena, Germany}
\author{M.~Firlej}
\author{T.~Fiutowski}
\author{M.~Idzik}
\author{J.~Moron} 
\author{K.~Swientek}
\affil{AGH University of Science and Technology, Faculty of Physics and Applied Computer 
Science, Krakow, Poland}

\author{M.~Borysova}
\author{H.~Lahno}
  \affil{ Institute for Nuclear Research NASU (KINR), Kyiv, 03680, Ukraine}
% \author{J.~Hallford$^{f}$}
\author{J.~Hallford\footnote{also at  Deutsches Elektronen-Synchrotron (DESY), Hamburg, 22607, Germany }}
\author{A.~Hartin}
\author{M.~Wing\footnote{also at  Deutsches Elektronen-Synchrotron (DESY), Hamburg, 22607, Germany }}
  \affil{University College London, London, WC1E 6BT, United Kingdom}
 \author{ A.~Fedetov}
\author{A.~Mironov}
  \affil{National Research Nuclear University MEPhI, Kashirskoe sh. 31, Moscow, 115409, Russia}
 \author{S.~Rykovanov}
  \affil{Skolkovo Institute of Science and Technology (Skoltech), Moscow 121205, Russia}
  \author{U.~Dosselli, M.~Morandin, M.~Zanetti}
  \affil{INFN, Padova, Italy}
 \author{B.~King}
\author{T.~Heinzl}
\author{A.~Ilderton}
\author{A.J.~Macleod}
\author{S.~Tang}
  \affil{University of Plymouth, Plymouth PL4 8AA, United Kingdom}

\author{O.~Davidi}
\author{G.~Perez}
\author{A.~Santra}
 \author{N.~Tal Hod}
  \affil{Weizmann Institute of Science, Rehovot, 7610001, Israel}
\author{Z.~Bai\footnote{ also at Weizmann Institute of Science, Rehovot, 7610001, Israel}}
\affil{Department of Physics, Southern University of Science and Technology, Shenzhen 518055, China}
\author{S.~Boogert}
  \affil{John Adams Institute at Royal Holloway, Department of Physics, Royal Holloway, Egham, TW20 0EX, Surrey, United Kingdom}
\author{H.~Abramowicz}
\author{Y.~Benhammou}
\author{S.~Huang}
\author{A.~Levanon}
\author{A.~Levy}
\author{I.~Pomerantz}
  \affil{Tel Aviv University, Tel Aviv, 6997801, Israel}



                                                           %




==> authorlists/authorlist.tex <==

\author[1]{H. Abramowicz}
\author[2,3]{U.~Acosta}
\author[4]{M. Altarelli}
\author[5]{R.~A{\ss}mann}
\author[6,7]{Z.~Bai}
\author[5]{T.~Behnke}
\author[1]{Y.~Benhammou}
\author[8]{T.~Blackburn}
\author[9]{S.~Boogert}
\author[5]{O.~Borysov}
\author[5,10]{M.~Borysova}
\author[5]{R.~Brinkmann}
\author[11]{M.~Bruschi}
\author[5]{F.~Burkart}
\author[5]{K.~B{\"u}{\ss}er}
\author[12]{N.~Cavanagh}
\author[6]{O.~Davidi}
\author[5]{W.~Decking}
\author[13]{U.~Dosselli}
\author[3]{N.~Elkina}
\author[14]{A.~Fedotov}
\author[15]{M.~Firlej}
\author[15]{T.~Fiutowski}
\author[12]{K.~Fleck}
\author[16]{M.~Gostkin}
\author[5]{C.~Grojean\thanks{also at HU Berlin}}
\author[5,17]{J.~Hallford}
\author[18,19] {H.~Harsh}
\author[17]{A.~Hartin}
%\author[3]{I.~Hartl}
\author[5,20]{B.~Heinemann\thanks{corresponding author: beate.heinemann@desy.de}}
\author[21]{T.~Heinzl}
\author[5]{L.~Helary}
\author[5,20]{M.~Hoffmann}
\author[1]{S.~Huang}
\author[5,15,20]{X.~Huang}
\author[15]{M.~Idzik}
\author[21]{A.~Ilderton}
\author[5]{R.~Jacobs}
\author[2,3]{B.~K{\"a}mpfer}
\author[21]{B.~King} 
\author[10]{H.~Lahno}
\author[1]{A.~Levanon}
\author[1]{A.~Levy}
\author[22]{I.~Levy}
\author[5]{J.~List}
\author[5]{W.~Lohmann\thanks{also at BTU Cottbus und RWTH Aachen}}
\author[23]{T.~Ma}
\author[21]{A.J.~Macleod}
\author[6]{V. Malka}
\author[5]{F.~Meloni}
\author[14]{A.~Mironov}
\author[13]{M.~Morandin}
\author[15]{J.~Moron}
\author[5]{E.~Negodin}
\author[6]{G.~Perez}
\author[1]{I.~Pomerantz}
\author[24]{R.P{\"o}schl}
\author[5]{R.~Prasad}
\author[25]{F.~Qu\'er\'e}
\author[5]{A.~Ringwald}
\author[26]{C.~R\"odel}
%\author[3]{M.~Saimpert}
\author[27]{S.~Rykovanov}
\author[18,19] {F. Salgado}
\author[6]{A.~Santra}
\author[12]{G.~Sarri}
\author[18]{A.~S{\"a}vert}
\author[28]{A.~Sbrizzi\thanks{also at University of Udine, Udine, Italy}}
\author[5]{S.~Schmitt}
\author[2,3]{U.~Schramm}
\author[5]{S.~Schuwalow}
\author[18]{D.~Seipt}
\author[29]{L.~Shaimerdenova}
\author[5]{M.~Shchedrolosiev}
\author[29]{M.~Skakunov}
\author[23]{Y.~Soreq}
\author[12]{M.~Streeter}
\author[15]{K.~Swientek}
%\author[6]{T.~Teter}
%\author[21]{A.~Titov}
\author[6]{N.~Tal~Hod}
\author[21]{S.~Tang}
\author[18,19]{T.~Teter}
\author[5]{D.~Thoden}
\author[16]{A.I.~Titov}
\author[29]{O.~Tolbanov}
\author[3]{G.~Torgrimsson}
\author[29]{A.~Tyazhev}
\author[5,17]{M.~Wing}
\author[13]{M.~Zanetti}
\author[29]{A.~Zarubin}
\author[3]{K.~Zeil}
\author[18,19]{M.~Zepf}
\author[16]{A.~Zhemchukov}

\affil[1]{Tel Aviv University, Tel Aviv, 6997801, Israel}
\affil[2]{TU~Dresden, 01062 Dresden, Germany}
\affil[3]{Helmholtz-Zentrum Dresden-Rossendorf, 01328 Dresden, Germany}
\affil[4]{Max Planck Institute for Structure and Dynamics of Matter, 22761 Hamburg, Germany}
\affil[5]{Deutsches Elektronen-Synchrotron (DESY), 22607 Hamburg, Germany}
\affil[6]{Weizmann Institute of Science, Rehovot, 7610001, Israel}
\affil[7]{Department of Physics, Southern University of Science and Technology, Shenzhen 518055, China}
%
\affil[8]{University of Gothenburg, SE-41296 Gothenburg, Sweden}
\affil[9]{John Adams Institute at Royal Holloway, Department of Physics, Royal Holloway, Egham, TW20 0EX, Surrey, UK}
\affil[10]{Institute for Nuclear Research NASU (KINR), Kyiv, 03680, Ukraine}
\affil[11]{INFN and University of Bologna, Bologna, Italy}
\affil[12]{School of Mathematics and Physics, The Queen’s University of Belfast, Belfast, BT7 1NN, UK}
\affil[13]{INFN and University of Padova, Padova, Italy}
\affil[14]{National Research Nuclear University MEPhI, Kashirskoe sh. 31, Moscow, 115409, Russia}
\affil[15]{Faculty of Physics and Applied Computer Science, AGH University of Science and Technology,  Krakow, Poland} 
\affil[16]{Joint Institute for Nuclear Research ( JINR), Dubna 141980, Russia}
\affil[17]{University College London, London, WC1E 6BT, UK}
\affil[18]{Helmholtz Institut Jena,  07743 Jena, Germany}
\affil[19]{Friedrich Schiller Universit{\"a}t Jena, 07743 Jena, Germany}
\affil[20]{Albert-Ludwigs-Universit{\"a}t Freiburg, 79085 Freiburg, Germany}
\affil[21]{University of Plymouth, Plymouth, PL4 8AA, UK}
\affil[22]{Department of Physics, Nuclear Research Centre-Negev, P.O. Box 9001, Beer Sheva 84190, Israel}
\affil[23]{Physics Department, Technion—Israel Institute of Technology, Haifa 3200003, Israel}
\affil[24]{Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affil[25]{LIDYL, CEA, CNRS, Universit\'e Paris-Saclay, CEA Saclay, 91 191 Gif-sur-Yvette, France}
\affil[26]{Institute of Nuclear Physics, TU Darmstadt, 64289 Darmstadt, Germany}
\affil[27]{Skolkovo Institute of Science and Technology (Skoltech), Moscow 121205, Russia}
\affil[28]{INFN Trieste, Trieste, Italy}
\affil[29]{National Research Tomsk State University NI TSU, TSU, Russia}


%\newpage

==> bib/doc/Makefile <==
# Makefile for creating documentation for ATLAS LaTeX
# Usually called from a subdirectory

TEXLIVE  = 2020
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = dummy

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *.fls *.fdb_latexmk *.listing .*.lb *~

cleanpdf:
	-rm $(BASENAME).pdf


==> bib/doc/atlas_latex/atlas_latex-text.tex <==
% !TEX root = atlas_latex.tex

%-------------------------------------------------------------------------------
% Body of the guide to the use of the ATLAS LaTeX package
%-------------------------------------------------------------------------------
\section{Introduction}
\label{sec:intro}
%-------------------------------------------------------------------------------

This collection of ATLAS \LaTeX\ templates, style files and documentation
can be used for papers, preprints and notes, both public and internal. 
All necessary files are collected in a single package called \Package{atlaslatex}.
The package is available from the web pages of the Publication Committee~\cite{pubcom} and from 
Git~\cite{pubcom-git}.

\ADOCnew{09-00-00} The package should work for \TeX\ Live versions from 2013 onwards.
\ADOCnew{II-JJ-KK} indicates the version number of ATLAS \LaTeX\ when new features are added.
\ADOCold{II-J-KK} indicates the version number when a feature is removed or made obsolete.

The collection replaces and improves on the previous packages.
In particular it supersedes:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{atlasnote-00-04-05}
\item \texttt{atlascover-00-00-11}
\item \texttt{atlaspreprint-00-00-05}
\item \texttt{atlasbib-00-00-04}
\end{itemize}
\Cref{sec:oldnote} summarises the changes that have been made and
how you can adapt your documents to use the new package.
\Cref{sec:oldcover} summarises the changes to the cover macros.

The package includes the \Package{atlasdoc} class, useful style files
and documentation of the package.
The package also defines a standard ATLAS style for papers.
This style should be used for paper drafts and for submission to the arXiv and the journal.
This option is the default. Add the option \Option{atlasstyle=false} to the \Package{atlasdoc} class if you do not want to use this style.
The documentation is provided as both PDF files and \LaTeX\ documents
that should provide examples of how to use the package and how to write
good \LaTeX.

The design principle is that you have a main document and 
the style files and \Package{atlasdoc} class are in a subdirectory \File{latex}.
The logos that are needed are kept in a \File{logos} directory.
These subdirectories can of course be links to a centrally maintained \texttt{latex} directory.
See below and \cref{sec:texmf} for how to proceed if you want to use and/or install
the package in a central place.

The usual procedure is that for each document that you create,
you first unpack the latest version of \Package{atlaslatex} and
then create your main document in the top-level directory.
This structure means that it is easier to update the style files if a new version of
\Package{atlaslatex} is released. 
Each document can then be independent of the \Package{atlaslatex} release.

%------------------------------------------------------------------------------
\section{Getting started}
%------------------------------------------------------------------------------

To create a new document you can issue one of the commands:
%
\begin{bashlisting}
make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]
make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]
\end{bashlisting}
depending on whether you want to write a paper/CONF Note/Pub Note draft or
an ATLAS not draft.
%
The command copies \File{atlas-document.tex} and
\File{atlas-paper-metadata.tex} or \File{atlas-note-metadata.tex}
to \File{mydocument.tex} and \File{mydocument-metadata.tex}.%
\footnote{The \File{Makefile} should work for regular Linux and MacOSX distributions.
For Windows, you probably have to execute the tasks in the \File{Makefile} by hand.}
The selected \TeX\ Live version is set with the \Option{TEXLIVE} option. The default is 2020.
The \texttt{make newpaper|newnote} command also creates empty files \File{mydocument-defs.sty} and \File{mydocument.bib}.
By default the document will be an ATLAS note draft.
Use \texttt{make newpaper} for an ATLAS paper draft (including CONF and PUB notes).
% If you want it to be a paper draft, add the option \Option{PAPER} to the document class.
Replace the option \Option{PAPER} with \Option{CONF} or \Option{PUB} as appropriate.

In the \File{Makefile} you should change the \texttt{BASENAME} to the name of your document.
You can then compile your document with the command: \texttt{make}.
You can try the command \texttt{make run\_latexmk} instead,
which invokes \texttt{latexmk}, a Perl script that is cleverer than the \texttt{Makefile}.
You can also make this command the default.
Have a look at \File{Makefile} for other things you can adjust.

If you install \Package{atlaslatex} in a central directory such as \File{\$\{HOME\}/texmf} the basic command is one of:
%
\begin{bashlisting}
make newpapertexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
make newnotetexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
make newbooktexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
\end{bashlisting}
%
See \cref{sec:texmf} for more details.

In order to make a new document of book form like a TDR, use one of the commands:
%
\begin{bashlisting}
make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]
make newbooktexmf [BASENAME=mydocument] [TEXLIVE=YYYY]
\end{bashlisting}
%
By default, this will pass the option \Option{BOOK} to \Package{atlasdoc}.
Use \verb|make newbooktexmf| for a book with \Package{atlaslatex} in a central directory.

Note that you have to specify the language of your document as an option in the
\Macro{documentclass} command. Typical settings are
\begin{itemize}
\item UKenglish (or british);
\item USenglish (or american).
\end{itemize}

As mentioned above the default \TeX\ Live version is currently set to 2020.
This should be the only option you have to adjust if you use different versions of \LaTeX.
You should be able to always set a version lower than the one you have installed to maintain compatibility with older versions.
To test compatibility with arXiv, try a setting of 2020.
%This will, among other things, automatically switch from the \Package{newtx} fonts to \Package{txfonts} if you
%are using the ATLAS preprint style.

\ADOCnew{01-07-00} You should include the command \Macro{maketitle} after your\\
\verb|\begin{document}| if you want the document title to be printed.

Add the option \Option{atlasstyle=false} to the \Macro{documentclass} if you do not want to typeset your document in the ATLAS preprint style.

%------------------------------------------------------------------------------
\section{ATLAS \LaTeX\ and the Physics Office GitLab project}
%------------------------------------------------------------------------------

With the move of ATLAS software and documents to Git,
new opportunities are available to streamline the production of documents
and smooth the process of submitting them to arXiv and journals.
This project is called PO-GitLab in the following~\cite{atlas-PO-gitlab}.

In order for the new tools to work smoothly some file-naming conventions should be followed.
If the Physics Office set up the Git repository, the files should already have the correct names.
The conventions are documented on
\url{https://gitlab.cern.ch/atlas-physics-office/gitlab-integration/wikis/newproject}.
For paper drafts, in short:
\begin{itemize}
  \item the main file should have the name GROUP-YEAR-NUM-PAPER.tex;
  \item the metadata file should have the name GROUP-YEAR-NUM-PAPER-metadata.tex
  \item the auxiliary material should be included in a file with the name GROUP-YEAR-NUM-PAPER-auxmat.tex
\end{itemize}

In addition:
\begin{itemize}
  \item figures must be included using the \Macro{includegraphics} command;
\end{itemize}

%-------------------------------------------------------------------------------
\section{Title, author and document numbers}
\label{sec:metadata}
%-------------------------------------------------------------------------------

An ATLAS document usually collects a series of labels over time.
These include the reference code of the analysis, e.g.\ \texttt{BPHY-2013-04}, 
the ATLAS note number and the CERN preprint number.
In addition the abstract and title are needed on the front page of the document and also on various cover pages.
The editors of the document, the editorial board members and the contributors to the analysis
also need to be specified at some point.

While all this information can be collected in the main file of the document, 
it is probably better to put it all in a separate document.
By default this file is called \texttt{mydocument-metadata.tex}.

\ADOCnew{04-00-00} As the metadata needed for ATLAS notes and ATLAS papers are somewhat different,
separate templates are used.


%-------------------------------------------------------------------------------
\subsection{Authors and Contributors}
\label{sec:contribute}
%-------------------------------------------------------------------------------

You can include an author's ORCID using the \Macro{AtlasOrcid} macro:\\
\verb+\AtlasOrcid[0000-0002-03-9876]{John Postdoc}+.
This command will be used in the ATLAS Collaboration author lists.

The supporting documentation for an ATLAS note (not the paper draft) should contain a list of the contributors to the analysis.
A style file \Package{atlascontribute.sty} has been written to help with the creation of such a list.
The macros in the style file can also build the author list at the same time.
Two basic macros are used to add names to the author list and list of contributions:
\Macro{AtlasContributor} and \Macro{AtlasAuthorContributor}. 
The first macro adds a person to the list of contributors, while the second one also adds the person
to the author list. I assume that in almost all cases you will want to use \Macro{AtlasAuthorContributor}.
An optional argument can be added to \Macro{AtlasAuthorContributor}, which contains the author's ORCID.
The author's name becomes a link to the ORCID.
Typical commands are:
\begin{tcblisting}{listing only}
\AtlasAuthorContributor{Joe Student}{a}{fake background estimate.}
\AtlasAuthorContributor{Jane Student}{b}{top background estimate.}
\AtlasAuthorContributor[0000-0002-03-9876]{John Postdoc}{a}{editor of internal note.}
\AtlasContributor{Jo Helper}{useful contributions in a few places.}
\affil[a]{University of Nowhere}
\affil[b]{University of Somewhere}
\end{tcblisting}
If a person should be added to the author list, you also need to add an appropriate affiliation using the macro \Macro{affil}.
The optional argument is a letter or number that should also be given as the second argument to
\Macro{AtlasAuthorContributor}.

You can keep the list of authors and contributors separate
by using \Macro{author} for the authors and \Macro{AtlasContributor} for the contributors.
You print the list of contributors by giving the command \Macro{PrintAtlasContribute}.
Note that \Macro{PrintAtlasContribute} has an argument that gives the fraction of the line width
to be used for the name of the person.
The list should either be printed before the table of contents or after the conclusions
(i.e.\ where the Acknowledgements appear in a paper).

Note that the \Package{authblk} package assumes that you will also have affiliations for each author.
You can avoid them by using the syntax \verb|\author{[ ]{Author Name}}|.
Note that a space is needed in the optional argument.
This means that a space appears between the author name and the comma after it, which is not so nice.
Alternatively you can make the author list using the syntax:\\
\verb|\author{Joe Student \and Jane Student \and John Postdoc}| and avoid the use of the
\Package{authblk} package by giving the option \Option{authblk=false} to \Package{atlascontribute}.

Note that the \Package{atlascontribute} package requires that the packages 
\Package{array} and \Package{booktabs} be installed.
If the list of contributors is very long, it may spread over more than one page.
The \Package{tabular} environment does not like this.
Add the option \Option{longtable} to use \Package{longtable},
or the option \Option{xtab} to use \Package{xtab}.
This option of course also requires that the \Package{xtab} or \Package{longtable} package is installed.


%-------------------------------------------------------------------------------
\subsection{Special author lists}
%-------------------------------------------------------------------------------

Sometimes a PUB note has a special author list.
Hence a link to this list should be added to the front page.
This can be achieved with the following code snippet that should be used for the author:
\begin{tcblisting}{listing only}
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
\usepackage{authblk}
\author{The ATLAS Collaboration%
\thanks{The full author list can be found at:\\
  \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2014-YYY/authorlist.pdf}}
}
\end{tcblisting}

\ADOCnew{01-07-00} The first two lines are needed if you do not use the standard ATLAS preprint style.
Note that \Package{atlasdoc} has to be loaded with the option \Option{maketitle=false}
and \Macro{maketitle} should be added after \verb|\begin{document}|.

\ADOCold{07-00-00} In order that the footnote and the copyright statement do not overlap,
you may need to pass the option \Option{copyrightoffset=1em} to the \Package{atlasdoc} class.


%-------------------------------------------------------------------------------
\subsection{Metadata commands}
%-------------------------------------------------------------------------------

The standard list of metadata commands are given below.
More are available for the draft cover page when a paper, CONF note or PUB note draft
is circulated to the collaboration.\\
See \texttt{template/atlas-document-metadata.tex} for more details.

\begin{itemize}
  \item \Macro{AtlasTitle\{<Title>\}} typesets the paper title. If not
    given, you get either an error or a dummy title will be produced.

  \item \Macro{author\{<Author>\}} typesets the paper author. If not
    explicitly given, \enquote{The ATLAS Collaboration} will be used by
    default. Note that the \verb|\author{}| command is pretty limited
    in case you want to display multiple author names and multiple
    affiliations. For this use case the \verb|authblk.sty| package is
    provided; this is a typical example of its use:
    \begin{verbatim}
\usepackage{authblk}
\renewcommand\Authands{, } % avoid ``. and'' for last author
\renewcommand\Affilfont{\itshape\small} % affiliation formatting

\author[a]{First Author}
\author[a]{Second Author}
\author[b]{Third Author}

\affil[a]{One Institution}
\affil[b]{Another Institution}
    \end{verbatim}
    See also \cref{sec:contribute} if you want to combine the creation of a list of authors and contributors.

    If you do not want each institute on a separate line, uncomment the lines in the metadata file:
    \begin{verbatim}
\makeatletter
\renewcommand\AB@affilsepx{, \protect\Affilfont}
\makeatother
    \end{verbatim}


  \item \Macro{AtlasAbstract\{<The abstract text>\}} typesets the
    abstract on the front page and cover page.

  \item \Macro{date\{<Date>\}} typesets the paper date. If not
    explicitly given, the current date (\verb|\today|) will be used.

  \item \Macro{AtlasVersion\{<Draft Version>\}} displays the draft
    version on the front page, a DRAFT banner on all the other page
    headings, and adds line numbers to all text to easy commenting and
    reviewing.
    Should be included when paper draft is circulated to ATLAS.
    Highly recommended for all documents in the draft stage.
    In the future, the steering of whether the document is a draft or not will be done
    using the option \Option{atlasdraft}.
    \ADOCnew{04-03-00} If \Option{atlasdraft=true} or \Macro{AtlasVersion} is not empty,
    the document is declared as a draft.

  \item \Macro{AtlasJournal\{<Journal Name>\}} displays the phrase \emph{to
    be submitted to Journal Name} at the bottom of the front page and
    on the cover page.
    Should be included when a paper draft is circulated to ATLAS.

  \item \Macro{AtlasRefCode\{<Reference code>\}} displays the ATLAS
    standard reference code, e.g.\ \texttt{BPHY-2014-03}, on the front page and
    the cover page. Not shown on the front page if the note number is given.

  \item \Macro{AtlasNote\{<Note number>\}} displays the note number
    for a CONF, PUB, INT or COM note, e.g.\ \texttt{ATLAS-CONF-2014-23},
    on the front page and cover page.
    If the note number is given, the reference code is not shown.

  \item \Macro{PreprintIdNumber\{<CERN preprint number>\}} displays the CERN
    preprint number on the front page.
    
  \item \Macro{AtlasDate\{<Date>\}} set by the Physics Office as the date of submission of a paper.

  \item \Macro{AtlasJournalRef\{<Journal reference>\}} displays the journal reference
    on the preprint front page.
    This should be used for the arXiv update after the paper has been published.

  \item \Macro{AtlasDOI\{<Journal reference>\}} displays the DOI
    on the preprint front page.
    This should be used for the arXiv update after the paper has been published.

  \item \Macro{arXivId\{<arXiv identifier>\}} displays the arXiv reference
    on the front page.

\end{itemize}
%
\texttt{template/atlas-document.tex} contains a basic skeleton that can be
used to start typing a new note using the \texttt{atlasdoc} class. Many of
the custom commands described above are used in this example file, in
order to demonstrate their use.

Links to supporting documentation should also be included on the cover page of draft papers circulated to ATLAS.
They can be included using
\verb|\AtlasCoverSupportingNote{Short title}{CDS link}|.
It is also possible to give a TWiki page instead, but this is deprecated.\\
As mentioned above, see \texttt{template/atlas-document-metadata.tex} for more details.


%-------------------------------------------------------------------------------
\section{The \texttt{atlasdoc} class}
\label{app:atlasdoc}
%-------------------------------------------------------------------------------

This document has been typeset using the \texttt{atlasdoc.cls} class.

The \texttt{atlasdoc} class can use either the standard \LaTeX\ \texttt{article} class
as its basis or the \KOMAScript\ \texttt{sctartcl} class.
All the usual commands and options you usually use
with \texttt{article}  or \texttt{scrartcl} should work with it. 
You turn on the use of \KOMAScript\ with the option \texttt{koma}.
For instance, a standard document can be produced using this simple preamble:
%
\begin{tcblisting}{listing only}
  \RequirePackage{latex/atlaslatexpath}
  \documentclass[UKenglish]{atlasdoc}
  \usepackage{atlaspackage}
  \usepackage{atlasphysics}
  \graphicspath{{logos/}{figs/}}
\end{tcblisting}
%
Note that the document language must be specified, otherwise \texttt{babel} will complain.

The \LaTeX\ packages that are used in the document are mostly specified in 
\texttt{latex/atlaspackage.sty}.

The style file \texttt{latex/atlasphysics.sty} defines a lot of useful
macros for particles and more. See the separate document
\texttt{atlas\_physics.pdf}~\cite{atlas-physics} for details.

If you do not want to use \Package{biblatex} you need to add the option \Option{biblatex=false} when you
include \texttt{atlaspackage}.
Have a look at the \texttt{latex/atlaspackage.sty} to see how \texttt{biblatex} is included.
In your main document you use \Macro{addbibresource} in the preamble to include your \texttt{.bib} files.
Note that the backend \Package{biber} returns with an error if it finds an empty \texttt{.bib} file.
A style file \File{latex/atlasbiblatex.sty} is available that adjusts the format of the references to the usual ATLAS conventions.

As mentioned above, you have to specify the document language as an option to \Package{atlasdoc}.
Several more options can be set.
In the following the default option is in boldface.
\begin{description}
\item[\Option{atlasstyle=true|{\normalfont false}}] turn on (default) or off the use of the ATLAS style for the document;
\item[\Option{atlasdraft={\normalfont true}|false}] this is a draft version of the document;
\item[\Option{coverpage}] include an ATLAS draft cover page;
\item[\Option{cernpreprint}] make the front page for a CERN preprint.
  The option \Option{preprint} works as well, but is deprecated;
\item[\Option{NOTE}] the document is an ATLAS note (default);
\item[\Option{PAPER}] the document is an ATLAS paper (draft);
\item[\Option{CONF}] the document is a CONF note;
\item[\Option{PUB}] the document is an PUB note;
\item[\Option{BOOK}] the document is book form like an LOI or TDR;
\item[\Option{HEPDATA}] a separate document with detailed tables etc.\ for HEPData;
\item[\Option{texlive=2020}] adjust if you use an older version of \TeX\ Live like 2013.
  A value less than 2013 adjusts a few \Package{biblatex} options.
  A value less than 2012 uses \Package{txfonts}.
\item[\Option{paper=a4|{\normalfont letter}}] set the paper size;
\item[\Option{titlesize=normal|{\normalfont small}}] use normal or reduced size fonts for the title page;
\item[\Option{tocdepth=2}] depth of table of contents. The default is to include subsections (2);
\item[\Option{floatopt=true|{\normalfont false}}] adjust the options (default) governing number and placement of floats on a page;
\item[\Option{tableheading=true|{\normalfont false}}] adjust table caption spacing for captions above the table;
\item[\Option{mathlines=true|{\normalfont false}}] put line numbers on equations;
\item[\Option{linenofix=true|{\normalfont false}}] fix line numbers around AMS math environments with using the \Package{linenomath} environment;
\item[\Option{texmf}] use the syntax \Macro{usepackage\{package\}}
  instead of \Macro{usepackage\{latex/package\}} to include packages.
  \emph{\ADOCold{10.0.0} With the move to the \Package{atlaslatexpath} style file, this option is obsolete}.
\item[\Option{newtx}] use the \Package{newtxtext} and \Package{newtxmath} packages for fonts 
  (default for \TeX Live > 2012);
\item[\Option{txfonts}] use the \Package{txfonts} package for fonts instead of the default
  (default for older \TeX Live versions);
\item[\Option{abstract=true|\normalfont{false}}] the document contains an abstract.
  This option is only needed together with the \Option{BOOK} option,
  if the book does not have an abstract;
\item[\Option{atlaslogo=true|{\normalfont false}}] show the ATLAS logo on the title page;
\item[\Option{cernlogo=true|{\normalfont false}}] show the CERN logo on the title page;
\item[\Option{cmslogo={\normalfont true}|false}] include the CMS logo on the title page;
\item[\Option{extralogo=\normalfont{filename}}] include an extra logo on the title page;
\item[\Option{showframe={\normalfont true}|false}] load the \Package{showframe} package, to display frames showing the boxes for text body, header, footer and margin;
\item[\Option{shownote={\normalfont true}|false}] show the PUB note number.
  This is turned off by default for the final version of PUB notes.
  It does not affect other document types.
\item[\Option{mhchem={\normalfont true}|false}] include \Package{mhchem} before \Package{xpatch} to avoid
  an error with \TeX\ Live 2014.
  \emph{\ADOCold{07-00-00} This option has no effect};
\item[\Option{datetop=true|{\normalfont false}}] put the date at the top of the title page;
  \emph{\ADOCnew{07-00-00} No date is printed if this option is set to false};
\item[\Option{titleextraheight=0em}] extra height that could be needed for the title, if it is very long.
  \emph{\ADOCold{07-00-00} This option has no effect};
\item[\Option{copyrightoffset=0em}] adjust the position of the copyright, if it is not completely correct.
  \emph{\ADOCold{07-00-00} This option has no effect};
\end{description}

\ADOCnew{11.4.0} The option \Option{tableheading} leads to better spacing of table captions above a table (the ATLAS default).
With this option, and in general,you should use \Macro{centering}
and not \Macro{begin\{center\}}\ldots\Macro{end\{center\}} to centre tables and figures.
If you want to place a caption explicitly you can use
the macros \Macro{captionabove} and \Macro{captionbelow}.

\ADOCnew{04-03-00} It is intended to replace using the definition of \Macro{AtlasVersion} to decide if this a final version of a document.
In a later version the default value will be set to \Option{false},
so that this option simply has to be removed when a document is final.

\ADOCnew{13.3.0} The options \Option{cmslogo} and \Option{extralogo} have been added to allow
the CMS Collaboration logo, or another logo, to be added to the CERN preprint page next to the ATLAS logo.
The logos are included with the same height as the ATLAS logo.
The extra logo should probably be added to the \File{logos} directory.
Using the option \Option{cmslogo} implies that the author and the copyright will be changed automatically.
If you use the option \Option{extralogo}, do not forget to adjust \Macro{author} (and copyright) accordingly,
if the paper is published together with another collaboration.

The \Option{atlaslogo} and \Option{cernlogo} options are for cases where a paper has a limited set of authors
and so should not necessarily include these logos.
In this case you may want to tweak the \Package{hyperref} document information,
the title page and also the draft label using the following commands:
\begin{verbatim}
% Author and title for the PDF file
\hypersetup{pdftitle={Limited author document},pdfauthor={J.~Smith et al.}}
% Tweak the title page
\AtlasHeading{System Paper}
\AtlasDraftHeading{DRAFT}
\end{verbatim}

The following options were removed.
% They are mostly still available in \Package{atlasdoc1}.
\begin{description}
\item[maketitle={\normalfont true}|false] turn on or off the creation of a title page within \Macro{AtBeginDocument}.
  \ADOCold{02-00-00} If the option is false, but you still want a title, give the command \Macro{maketitle} after
  \verb|\begin{document}|.
  This is the recommended way of proceeding;
\item[nomaketitle]\mbox{}
  \ADOCold{01-07-00}  do not create a title page; equivalent to \Option{maketitle=false};
\item[koma=true|{\normalfont false}] use the \KOMAScript\ base class \Package{scrartcl} instead of \Package{article};
  \ADOCold{02-00-00} No longer an option.
\item[\Option{letterpaper}] set the paper size to letter.
  \ADOCold{07-00-00} This option does not work anymore
  --- use \Option{paper=letter} instead;
\item[\Option{a4paper}] set the paper size to A4;
  \ADOCold{07-00-00} This option does not work anymore
  --- use \Option{paper=a4} instead;
\item[\Option{letter}] set the paper size to letter.
  \ADOCold{02-00-00} This option does not work anymore
  --- use \Option{paper=letter} instead;
\end{description}
Note that the options \Option{CONF} and \Option{PUB} get passed to \Package{atlascover.sty}
as they only influence the cover pages.
%The option \Option{BOOK} uses book instead of article as the base class.

The
\href{http://www.tex.ac.uk/cgi-bin/texfaq2html?label=floats}{UK List of FAQ}
recommends changing several default \LaTeX\ options so that there are fewer problems
with figure and table placement.
It is certainly worth reading that page for further advice.
As it is very hard to really test how well these options work
they can be turned on or off in \Package{atlasdoc} via the option \Option{floatopt=true|false}.
The default value is set to \Option{true}.

\ADOCnew{02-00-00} \KOMAScript\ elements are used to create the title pages.
In particular, \Macro{publishers} is used for the abstract and copyright.
The space and position for this may need to be adjusted,
if you have a very long title. 
It is very helpful to turn on the \Option{showframe} option when doing such adjustments.
\ADOCold{07-00-00} Use the options
\Option{titleextraheight} and \Option{copyrightoffset} to make adjustments.


%-------------------------------------------------------------------------------
\subsection{Packages, dependencies and \Package{atlaspackage}}
\label{sec:atlaspackage}
%-------------------------------------------------------------------------------

The \Package{atlasdoc} class depends on these packages, whose presence in
your system is required:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \Package{babel}: become language aware;
\item \Package{scrlayer-scrpage}: defines the header for draft mode
  and for auxiliary material documents.
  For \TeX\ Live 2014 and earlier \Package{scrpage2} is used instead.
\item \Package{fontenc}: output font encoding;
\item \Package{hyperref}: add hyperlinks and ability to click on cross-references;
\item \Package{graphicx}: include graphics in the document;
\item \Package{lineno}: add line numbers to documents;
\item \Package{newtxtext} and \Package{newtxmath}: the standard ATLAS document font.
  If this is not available, you can fall back to \Package{txfonts};
\item \Package{xcolor}: add colours to \LaTeX;
\item \Package{ifthen}: improved handling of conditionals;
\item \Package{kvoptions}: process options passed to packages.
%\item \Package{scrdate, scrtime}: Current date and time for use in the header.
\end{itemize}
These should be installed in any modern \LaTeX\ installation.
See \cite{latex-faq} for details on which collections are needed to get these packages
for your operating system.

% Note that under Ubuntu versions 12.04 and 14.04, \Package{lineno} can be found in the
% \Package{texlive-humanities} package!
If you cannot find the \Package{lineno} package, it is also included in the \File{obsolete} directory.
Copy it to your main directory, or to \verb|${HOME}/texmf/tex/latex| in order to make
it centrally available.

Both the class \Package{atlasdoc} and all style files:
\Package{atlasbiblatex}, \Package{atlascontribute}, \Package{atlascover}, \Package{atlaspackage}, \Package{atlasphysics}
and \Package{atlastodo} need the package \Package{kvoptions} 
so that they can process options where a value for an option should be set.

\Package{atlasdoc} and \Package{atlascover} both need \texttt{hyperref}. 
Have a look at one of these packages to see how to include it by hand.
You can also simply use \texttt{atlaspackage.sty}

The style file \texttt{atlaspackage.sty} includes further packages.
You can steer how many by using the option \Option{minimal}, \Option{default} or \Option{full}.
The minimal set is:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{mathtools}: extra useful maths environments -- this includes \Package{amsmath} and some bug fixes;
\item \texttt{inputenc}: allow ä, ö, ø, ß, etc. to be input directly;
\item \texttt{hyperref}: add hyperlinks and ability to click on cross-references;
\item \texttt{placeins}: adds commands to force figure and table output before a certain position in the text.
\end{itemize}

The default set adds in addition:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{booktabs}: nicer tables. Use \Macro{toprule}, \Macro{midrule} and \Macro{bottomrule} instead of \Macro{hline};
\item \texttt{csquotes}: smart quotes that incorporate language dependence;
\item \texttt{siunitx}: units package with extra functionality for tables;
\item \texttt{subfig}: more than one plot in a figure;
% \item \texttt{tocloft}: extra options for typesetting table of contents etc.;
\item \texttt{cleveref}: automatically include \enquote{Fig.}, \enquote{Section} etc. when cross-referencing;
\item \texttt{bookmark}: better construction of index or outline in PDF viewers.
\end{itemize}

Finally the full set includes further packages that may be useful:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \texttt{mhchem}: chemical elements and molecules;
\item \texttt{diffcoeff}: mathematics for physics;
\item \texttt{rotating} rotate figures, tables, etc.;
\item \texttt{xfrac} nicer fractions;
\item \texttt{multirow} construction for table cells that span more than one row of the table.
\item \texttt{longtable} newer version of \Package{supertabular}, which allows tabular environments to go over more than one page.
  As an alternative you can include the use the option \Option{xtab} to use the \Package{xtab} package instead.
\end{itemize}
The above packages are all included if you turn on the full set.
You can turn them on individually if you use the minimal or standard set.
If you pass the \Option{xtab} option, it will be included instead of \Package{longtable}.
\ADOCold{12.0} If you are using an older \TeX\ Live version (earlier than 2016),
you will probably get an error when using the \Option{full} option,
as the \Package{diffcoeff} package was first released in 2016.
If this is the case, include the packages you want by passing the appropriate options to \Package{atlaspackage}.
\ADOCnew{12.1} \Package{diffcoeff} will not be included for \TeX\ Live versions older than 2016 (defined by the \Option{texlive} option).

The full list of options is:
\begin{description}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item[\Option{biblatex=true|{\normalfont false}}] turn on/off use of \Package{biblatex} and \Package{biber/bibtex};
\item[\Option{backend={\normalfont bibtex}|biber}] specify the backend to use with \Package{biblatex}.
  Specify \Option{backend=bibtex} to use \Package{bibtex} instead;
\item[\Option{hyperref=true|{\normalfont false}}] turn on/off use of the \Package{hyperref} package;
\item[\Option{bookmark=true|{\normalfont false}}] turn on/off use of the \Package{bookmark} package;
\item[\Option{siunitx=true|{\normalfont false}}] turn on/off use of the \Package{siunitx} package;
\item[\Option{eVkern={\normalfont true}|false}] apply a kern of -0.1em to \si{\eV} in order to move \enquote{e} and \enquote{V} closer together.
  This option is set by default if you use the \Option{txfonts} fonts;
\item[\Option{percentspace={\normalfont true}|false}] include or not the default space between a number and the \% sign;
\item[\Option{cleveref=true|{\normalfont false}}] turn on/off use of the \Package{cleverref} package;
\item[\Option{capsref=true|{\normalfont false}}] capitalise Section, Figure etc.\ when using \Package{cleverref};
\item[\Option{abbrevref=true|{\normalfont false}}] abbreviate Fig.\ etc.\ when using \Package{cleverref};
\item[\Option{mhchem={\normalfont true}|false}] turn on/off use of the \Package{mhchem} package;
\item[\Option{diffcoeff={\normalfont true}|false}] turn on/off use of the \Package{diffcoeff} package;
\item[\Option{physics={\normalfont true}|false}] turn on/off use of the \Package{physics} package;
\item[\Option{rotating={\normalfont true}|false}] turn on/off use of the \Package{rotating} package;
\item[\Option{xfrac={\normalfont true}|false}] turn on/off use of the \Package{xfrac} package;
\item[\Option{multirow={\normalfont true}|false}] turn on/off use of the \Package{multirow} package;
\item[\Option{longtable={\normalfont true}|false}] turn on/off use of the \Package{longtable} package;
\item[\Option{xtab={\normalfont true}|false}] turn on/off use of the \Package{xtab} package;
\item[\Option{subcaption={\normalfont true}|false}] use \Package{subcaption} instead of \Package{subfig};
  \Package{subcaption} is supposed to be a newer, better and more general package than \Package{subfig} or
  \Package{subfigure};
  % It is probably best to only use it with \TeX\ Live 2012 or later;
\item[\Option{subfigure={\normalfont true}|false}] use the deprecated package \Package{subfigure} 
  instead of \Package{subfig};
\item[\Option{subfig=true|{\normalfont false}}] use the somewhat deprecated package \Package{subfig};
\item[\Option{texlive=2020}] set if you use an older version of \TeX\ Live like 2013.
  % A value less than 2013 adjusts a few \Package{biblatex} options.
  % A value less than 2012 uses \Package{txfonts} and the old (Version 1) option names for \Package{siunitx}.
  % A value less than 2010 uses the old option names for \Package{csquotes}.
  Use \Option{texlive=2020} to test options for arXiv submissions;
\item[\Option{txfonts={\normalfont true}|false}] load the \Package{txfonts} package and adjust loading of \Package{mathtools/amsmath} for duplicate symbols;
\item[\Option{lineno=true|{\normalfont false}}] load the \Package{lineno} package.
\end{description}

\File{lineno.sty} and \File{authblk.sty} are also provided in \File{obsolete},
just in case they are not in your standard \LaTeX\ installation
and for some reason you cannot download them from CTAN (\url{https://ctan.org}).

Depending on the font you use, you may find that the \enquote{e} and \enquote{V} in \si{\eV}, \si{\MeV} etc.\
are too far apart.
You can pass the option \Option{eVkern} to \Package{atlaspackage} in order to move them 0.1em closer together.\footnote{%
This option has no effect for \TeX\ Live 2011 and older, as \Package{siunitx}
adjusted the spacing internally using the parameter \Option{eVcorra}.}
This is the amount used in the \File{atlasunit.sty} for \Macro{gev} etc.
which is included by passing the option \Option{unit=true} to \Package{atlasphysics}.
If you use \Package{siunitx}, I recommend setting \Option{unit=false},
so that you use one consistent set of definitions throughout your document.

The \Package{siunitx}~\cite{siunitx} package puts a (non-breaking) small space between a number and the \% sign,
as for any other unit.
It says that this is as required by the SI system of units~\cite{SI}.
In Section~5.4.7 of the brochure one can find:
\begin{quotation}
  The internationally recognized symbol \% (percent) may be used with the SI.
  When it is used, a space separates the number and the symbol \%.
  The symbol \% should be used rather than the name \enquote{percent}.
  In written text, however, the symbol \% generally takes the meaning of “parts per hundred”.
\end{quotation}
However, conventions between publishers appear to differ~\cite{percentspace}.
Many people are used to there being no space and this is also the ATLAS convention.
Pass the option \Option{percentspace=true} to include the space.
% This option only works for \TeX\ Live versions 2011 and later.

There used to be a problem using the \Package{tikz} package with \Package{atlasnote}.
With \Package{atlasdoc} this problem seems to have gone away.
\Package{tikz} is not included in \Package{atlaspackage}.
If you want to use it, just add the usual \verb|\usepackage{tikz}| to your preamble.

Other packages that have been used at some point include:
\begin{description}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
\item \Package{savesym}: needed to avoid errors if \Package{txfonts} is used, 
  as \Package{txfonts} and \Package{amsmath} define the same symbols;
\item \texttt{footmisc}: extra footnote options. 
  These mess up the \Option{atlasstyle} settings.
\end{description}


%-------------------------------------------------------------------------------
\subsection{Cover pages}
\label{sec:cover}
%-------------------------------------------------------------------------------

The package also provides cover pages for the circulations of ATLAS drafts and 
for the front page for the CERN preprint version of an ATLAS paper.
A further cover page is provided for a document containing detailed tables associated with a preprint/paper.
The style file can be found in \texttt{latex/atlascover.sty}.

If you wish to use the \texttt{atlascover} package with the 
\texttt{atlasdoc} class, you should usually use the \texttt{coverpage} option of the class:
\begin{verbatim}
  \documentclass[coverpage,UKenglish]{atlasdoc}
\end{verbatim}
instead of the the usual \texttt{usepackage} command: this will ensure
that the cover page is produced before the title page of the document.

\ADOCnew{01-07-00} You can include \texttt{atlascover} with \Macro{usepackage} if you prefer.
\ADOCold{01-07-00} You need the option \texttt{maketitle=false}
and you should include the \Macro{maketitle} command after \verb|\begin{document}|.

The following options can be passed on to the \Package{atlascover} package:
\begin{description}
\item[\Option{coverpage}] outputs the standard ATLAS paper draft cover page;
\item[\Option{CONF}] the document is a CONF note;
\item[\Option{PUB}] the document is an PUB note;
\item[\Option{LANGEDIT}] prints the language editor's name and email address;
% \item[\Option{cernpreprint}] the title page should be in the form of a CERN preprint;
%   The option \Option{preprint} works as well, but is deprecated;
%\item[\Option{preprint}] the title page should be in the form of a CERN preprint;
% \item[\Option{auxmat}] the title page for a document containing auxiliary material from a paper;
\item[\Option{coverfontsize}] the base font size used for the cover (default is 11pt). Adjust this for long abstracts;
\item[\Option{twocolumn}] use this option if your document is formatted in two columns;
\item[\Option{atlasdoc}] this option is set by \Package{atlasdoc} and is not usually needed by the user.
\end{description}

\ADOCnew{01-04-00} If you use \Package{atlascover} standalone, use the option \Option{coverpage=true} to
actually output a cover page. 
This makes the use of options more consistent.
\ADOCnew{02-00-00} The options \Option{cernpreprint}, \Option{preprint}
and \Option{auxmat} are no longer available in \Package{atlascover}.
You should pass these to \Package{atlasdoc} instead, as the title pages are now part of the main class.

Some papers have a very long abstract, such that it does not fit on the cover page.
You can reduce the font size used on the cover by setting the option \Option{coverfontsize}.
The default value is 11pt. Try 10.5pt or 10pt instead to get the abstract onto the page.

It used to be the case that some journal styles, especially JHEP,
produced an ATLAS draft cover page that was offset.
You could use the options \Option{hoffset} and \Option{voffset} to move the text around.\\
JHEP needed \verb|hoffset=1in, voffset=1in|.\\
revtex (APS journals) looked better with  \verb|hoffset=-0.25in, voffset=-0.25in|.\\
\ADOCnew{01-04-00} These offsets are ignored,
as the problems with spurious offsets have been eliminated.

The option \Option{clearpage}, which used to exist, has no effect.


%-------------------------------------------------------------------------------
\section{ATLAS preprint style}
\label{sec:atlasstyle}
%-------------------------------------------------------------------------------

This style should be used for the preparation of paper drafts,
as well as for the submission of papers to the arXiv and journals.
The journals will then convert the documents to the style appropriate for the journal.
% As some experience has to be gained with this package,
% feedback on any problems that occur with the style are very welcome.

Documents are typeset by default in the standard ATLAS preprint style.
The use of this style can be turned off by using the option
\Option{atlasstyle=false}.
This style uses \KOMAScript\ as the base class.
Further settings include:
\begin{description}
\item[Layout:] \Option{DIV=14} and an extra \SI{5}{\mm} for the binding;
\item[Paragraph:] the paragraph indentation is set to zero and 
  there is a half-line separation between paragraphs;
\item[Figures and tables:] a small font size is used for the captions.
  Captions are not indented.
  They should be below both figures and tables;
\item[Font:] the default fonts are from the \Package{newtx} package.
  These are very similar to \Package{txfonts} that have been used up to now,
  but have a better spacing in a few cases;
\item[Section headers:] the standard serif font is used.
\end{description}

The default fonts for ATLAS documents are \Package{newtxtext} and \Package{newtxmath}.
These are more modern variants of the package \Package{txfonts} that has been used in
ATLAS documents in the past.
%However, arXiv currently uses an older version of \TeX\ Live (2011) that does not include the
%\Package{newtx} fonts. 
%In ATLAS papers, please add the option \Option{texlive=2011} to \Package{atlasdoc}.
%As soon as arXiv switches to a newer version of \TeX\ Live this option may have to be adjusted
%or will no longer be necessary.

In general, if you have problems with the \Package{newtx} fonts,
you can switch to \Package{txfonts} by including the option \Option{txfonts} with \Package{atlasdoc}.


%-------------------------------------------------------------------------------
\section{CERN preprints and arXiv}
\label{sec:preprint}
%-------------------------------------------------------------------------------

If you are writing an ATLAS paper and it has been approved by the collaboration,
you have to make a version with the CERN preprint title page and prepare the 
paper for submission to arXiv.

If your paper draft is within the PO-GitLab project, the following steps will be
performed by the Physics Office using the GitLab Continuous Integration tools.
Before asking the Physics Office to do this,
you should check that your paper draft follows the ATLAS conventions.

In order to turn the paper into a CERN preprint,
you should replace the option \Option{PAPER} by \Option{cernpreprint} in \Package{atlasdoc}.
The CERN preprint number is given via the macro \Macro{PreprintIdNumber}.
At the same time you should pass the option \Option{texlive=2020} to
\Package{atlasdoc}.
This is because arXiv contains a 2020 \TeX\ Live installation.
Summarising, a typical \Macro{documentclass} command would be:
\begin{tcblisting}{listing only}
\pdfoutput=1
\RequirePackage{latex/atlaslatexpath}
\documentclass[cernpreprint, atlasdraft=false, texlive=2020, UKenglish]{atlasdoc}
\end{tcblisting}
The \Macro{pdfoutput} command tells arXiv that a PDF file should be produced directly.
You should also turn off ATLAS draft cover page --- remove the option \Option{coverpage=true}.
% If you move the class and style files to the same directory as the main file,
% you need to add the option \Option{texmf} to the \Macro{documentclass}.

If your paper should include the CMS logo, pass the option \Option{cmslogo} to \Package{atlasdoc}.
If your paper should include another logo next to the ATLAS logo,
pass the filename of the other logo to \Package{atlasdoc} using the \Option{extralogo} option.

You can test whether your document compiles with \TeX\ Live 2020 by setting your \texttt{PATH} on \texttt{lxplus} to
{\small
\begin{verbatim}
export PATH=/cvmfs/sft.cern.ch/lcg/external/texlive/2020/bin/x86_64-linux:${PATH}
\end{verbatim}
}

Note that you should submit the \File{bbl} file and not the \File{bib} to arXiv.
Depending on which journal you submit to, you should turn on or off the printing of the titles in the bibliography.
Further details on how to proceed can be found on the Physics Office TWiki~\cite{atlas-physicsoffice} --- see
the Section on \enquote{Guidelines for paper submission}.
APS journals have special requirements on the directory structure and the filenames for figures.
This is handled by the PO-GitLab tools.
%JINST uses a very old version of \LaTeX\ (2004).
% Neither \Package{biblatex} nor \Package{siunitx} are available
% and \KOMAScript\ does not contain the \Macro{KOMAoptions} command.
% See the Physics Office TWiki~\cite{atlas-physicsoffice} for more information.

It also makes sense to clean up the metadata file at this point.
You get rid of line numbering by making sure that neither \Macro{AtlasVersion} nor \Macro{draftversion} are defined.
I recommend moving the relevant definitions into the main \TeX\ file so that the metadata file is no longer needed.
If you clean things up, the \Package{atlascover} package is no longer needed.
The metadata commands that are needed in addition to the title, author and abstract are:
\begin{itemize}
  \item \Macro{AtlasJournal\{<Journal Name>\}}
  \item \Macro{PreprintIdNumber\{<CERN preprint number>\}}
  \item \Macro{AtlasDate\{<Date>\}} set by the Physics Office
  \item \Macro{AtlasJournalRef\{<Journal reference>\}} once it exists
  \item \Macro{AtlasDOI\{<Journal reference>\}} once it exists
  \item \Macro{arXivId\{<arXiv identifier>\}} once it exists
\end{itemize}

More details on arXiv recommendations can be found at
\url{https://arxiv.org/help/submit_tex}.


%-------------------------------------------------------------------------------
\section{ATLAS TDR and LOI documents}
\label{sec:book}
%-------------------------------------------------------------------------------

If you include the option \Option{BOOK}, \Package{atlasdoc} uses the \Package{scrbook}
as the document class.
This option is geared to long documents such as TDRs and LOIs.
Such a document has various numbers which can be set as follows:
\begin{itemize}\setlength{\parskip}{0pt}\setlength{\itemsep}{0pt}
  \item \Macro{AtlasRefCode}: ATLAS reference code, e.g.\ ATLAS-TDR-099.
  \item \Macro{PreprintIdCode}: LHCC reference code, e.g.\ CERN-LHCC-2017-099.
  \item \Macro{AtlasDate}: Official date of the document.
\end{itemize}
The title will be typeset flushleft, rather than the usual centering.
A typical title would be:
\begin{verbatim}
  \AtlasTitle{Technical Design Report\\
  for the ATLAS Detector Upgrade}
\end{verbatim}

If you want to add images to the front and back covers,
the template contains commented out commands that allow you to do this.
The \Package{pdfpages} package seems to work very well for such things.
The images can be in \texttt{pdf}, \texttt{png} or \texttt{jpg} format.
Unlike \Macro{includegraphics} you should include the filename extension.

Note that the title page will only be correctly formatted if you use 
\TeX\ Live 2013 or newer. If you are using an older version add \Macro{flushleft}
to \Macro{AtlasTitle}.

%-------------------------------------------------------------------------------
\section{ATLAS notes}
\label{sec:note}
%-------------------------------------------------------------------------------

If you include the macro \Macro{AtlasNote} in your preamble,
the note number will be printed under \enquote{ATLAS NOTE} at the top of your document.
This can be used for any sort of ATLAS note, including CONF, PUB and INT notes.


%-------------------------------------------------------------------------------
\section{Auxiliary and HEPData material}
\label{sec:auxmat}
%-------------------------------------------------------------------------------

Many papers have extra plots and tables that should be made public,
but are not submitted to arXiv and the journal.
These should be collected in a file \File{mydocument-auxmat.tex},
which is included in the draft document during its circulation within ATLAS,
This is transparent for editors if they use use PO-GitLab system,
but has to be done manually for other papers.

Some papers have many pages of extra tables and plots that are mainly of use to theorists
who need extra information.
Such material should usually included in the paper draft until it is ready for
submission to arXiv and to the journal.
The default name for the file containing the information is \File{mydocument-hepdata.tex}.
At the submission stage it should be moved into a separate document.
A skeleton document created using the command \verb|make newdata BASENAME=...|.
The front page for this document is formatted using the \Option{HEPDATA} option.
If you use this option you should specify the arXiv preprint identifier
using the macro \Macro{arXivId} and the HEPData record using the macro
\Macro{HepDataRecord}.
This information is then included on the cover page in the form of clickable links.

Use of this option also adds the arXiv preprint identifier to the top
of every page of the document.

If you want to create an HEPData document with an older \TeX\ Live version such as 2013, 
use the command \texttt{make newdata TEXLIVE=2013}.


%-------------------------------------------------------------------------------
\section{Symbols in \texttt{atlasphysics.sty}}
\label{sec:atlasphysics}
%-------------------------------------------------------------------------------

Many useful symbols are defined in \texttt{atlasphysics.sty}.
While this used to be a very long file, it has now been split into several smaller files,
which can be included or not using options.
The definitions can be found in a separate document \File{atlas\_physics.pdf}.


%-------------------------------------------------------------------------------
\section{Snippets and templates for standard text}
\label{sec:atlassnippets}
%-------------------------------------------------------------------------------

The Publication Committee provides standard texts giving examples
for the description of the ATLAS detector, and the appropriate references,
as well as other text snippets that may be useful to avoid too much use of ATLAS jargon.
For example, the ATLAS detector description can be found in \File{template/atlas-detector.tex}

You can find some text snippets that can be used in papers in \File{latex/atlassnippets.sty}.
To use them, provide the \Option{snippets} option to \Package{atlasphysics}.
Text snippets can also be found on the web pages~\cite{pubcom-snippet}.
Comments and/or suggestions on improvements are very welcome and
should be given to the Publication Committee.

In addition, CP and analysis groups have started providing templates for supporting (INT) notes.
These are included in a subdirectory of the \File{template} directory.
For now (2018-10-29) there are some templates from the EXOT group.


%-------------------------------------------------------------------------------
\section{Adding notes}
\label{sec:todo}
%-------------------------------------------------------------------------------

When writing a paper, you or others often want to add notes so that things are not forgotten.

The \Package{atlastodo} package provides a macro \Macro{ATLnote} that can be used to define notes with separate colours for each author.
This macro uses the \Package{todonotes} package,
which is also used for language editor comments.
For example:
\begin{tcblisting}{listing only}
\ATLnote{JS}{Jane}{magenta!20}{magenta}
\end{tcblisting}
adds macros \Macro{JSnote} and \Macro{JSinote} for notes in the margin and inline.
Note that you must use the inline variant for notes inside captions and other floating objects.
Turn off the output of any notes by passing the option \Option{output=false}
to the \Package{atlastodo} package.

The following options can be passed on to the \Package{atlastodo} package:
\begin{description}
\item[\Option{output}\OptionTFT] turn off the output of any notes;
\item[\Option{shift}\OptionTFT] adjust the margin to allow more space for notes;
\item[\Option{version=2\textbar\normalfont{1}}] version number.
\end{description}

If you want a list of all the notes,
add \Macro{listoftodos} somewhere in your document.
The \Package{todonotes} package also include a macro \Macro{missingfigure}
that is very useful if you want to include a figure, but do not yet have the plot.

The following code produces the paragraph below.
\begin{tcblisting}{listing only}
Here is an \JSnote[example paragraph]{Illustration of macro}
that shows how to use the macro. If you want a comment
without it being associated with text omit the optional argument.
\JSnote{This is a comment without associated text.}
This is some fill text between the comments.
\JSnote[Text to be improved.]{This is a comment with assoicated text.}
If you prefer your comments to be inline use the \Macro{JSinote} macro.
\JSinote{Here is an inline comment.}
\end{tcblisting}
Here is an \JSnote[example paragraph]{Illustration of macro}
that shows how to use the macro. If you want a comment
without it being associated with text omit the optional argument.
\JSnote{This is a comment without associated text.}
This is some fill text between the comments.
\JSnote[Text to be improved.]{This is a comment with assoicated text.}
If you prefer your comments to be inline use the \Macro{JSinote} macro.
\JSinote{Here is an inline comment.}

\ADOCold{12.0} Version 1 of \Package{atlastodo} had two argument:
the first for the text to be commented on and the second for the comment.
\ADOCnew{13.0} Version 2 of \Package{atlastodo} has one option argument
for the text to be commented on and a required one for the comment.

As mentioned above, notes in captions and other floating objects must be inline.
If you include a note in a caption,
you should also provide a short caption that does not include the note.
If you do not you will get errors in the list of figures and/or tables.
Here is an example with a short caption:
\begin{tcblisting}{listing only}
\caption[A nice plot.]{A nice plot. \IBinote{This need to be improved.}}
\end{tcblisting}

%-------------------------------------------------------------------------------
\section{Language editor commands}%
\label{sec:langedit}
%-------------------------------------------------------------------------------

The \Package{todonotes} has been used to add a few macros that should be of use
for language editors. The commands are in the \Package{atlascomment} style file.
This file is included if the \Option{LANGEDIT} is passed to \Package{atlasdoc}.
The commands added are:
\begin{description}
  \item[\Macro{LEecomment}] adds a comment about a change, or suggested change.
\end{description}
The commands takes two arguments: the relevant text and the explanation/suggestion.

Such comments are probably also useful for paper editors.
Have a look at this style file and the \Package{todonotes} documentation on how
you can set up your own macros.


%-------------------------------------------------------------------------------
\section{Scripts}%
\label{sec:script}
%-------------------------------------------------------------------------------

Four scripts are provided in the \File{scripts} directory to help updating existing documents:
\begin{description}
  \item[\File{atlaslatex\_update.sh}] Script to update the \Package{atlaslatex} version
    to the latest master version in Git.
  \item[\File{atlaslatex\_2020.sh}] Script to update the \Package{atlaslatex} version
    to be compatible with the 2020 version of TeX Live and \LaTeX.
  \item[\File{atlaslatex\_selfupdate.sh}] Script to update the scripts themselves.
  \item[\File{tex\_dollars.py}] Script to change from use of \TeX\ primitive \verb|$...$|
    to the \LaTeX\ macro \verb|\(...\)|.
\end{description}
Have a look at the scripts for the available options.


%-------------------------------------------------------------------------------
\section{Miscellaneous \LaTeX{} tips}%
\label{sec:latex}
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
\subsection{Line numbers}

Line numbers can be printed using the \Package{lineno} package, 
which is included by default.
Line numbers are automatically turned on if you set \Macro{AtlasVersion} (or \Macro{draftversion})
or you pass the option \Option{atlasdraft=true} to \Package{atlasdoc}.
In general, you can turn them on and off in a document by using the \Macro{linenumbers} or \Macro{nolinenumbers} commands.
Note that if \Macro{AtlasVersion} or option \Option{atlasdraft=true} are set,
you will always get line numbers on the standard title page.
Hence, for papers, CONF and PUB notes it is important to comment out \Macro{AtlasVersion} in order to suppress the line numbers for the final version.

In order to avoid line numbers going slightly wrong around figures and tables,
separate the \Package{figure} and \Package{table} environment from the rest of the text using blank lines.

\ADOCnew{08-04-00} Line numbering around AMS Math \LaTeX\ environments such as \Package{align}
should just work.
The code that does this is inside \File{atlasdoc.cls}.
If this causes problems, pass the option \Option{linenofix=false} to \Package{atlasdoc}.
You can set the option \Option{mathlines=false} to turn off numbering the lines in equations.
% Some debugging of this option is still ongoing, so it is currently set to \Option{false}.

For older versions of \Package{atlaslatex},
if you use AMS Math \LaTeX\ environments line numbering may be interrupted around the environment.
Enclose the environment in a \Package{linenomath} environment to fix this problem:
\begin{tcblisting}{listing only}
\begin{linenomath}
\begin{equation*}
  E = m c^{2}
\end{equation*}
\end{linenomath}
\end{tcblisting}
If you are using the environment \Package{linenomath} you may have to set the option \Option{mathlines=false}to avoid spurious line numbers.


%-------------------------------------------------------------------------------
\subsection{Definitions}

You can use \verb|\ensuremath| in definitions, so that they will work
in both text mode and math mode, e.g.\
\verb|\newcommand{\UoneS}{\ensuremath{\Upsilon(\text{1S})}\xspace}| to get
\UoneS in either mode (\verb|\UoneS{}| or \verb|$\UoneS$|).

I highly recommend that you also terminate every definition with \Macro{xspace},
as then you can use the definitions without having to terminate them with
\enquote{\textbackslash\textvisiblespace} or \enquote{\{\}}.


%-------------------------------------------------------------------------------
\subsection{Figures}

Use the \Package{graphicx} package to include your plots and figures. 
The use of older packages like \Package{espfig} is deprecated.
Since the \Package{graphicx} package is required by the \Package{atlasdoc}
class, it is automatically loaded when using it, and there is no need
to explicitly include it in the document preamble.

Always include your graphics file without giving the file extension.
For instance, if you want to include the \File{figure.eps}
file, you should use a syntax like this:
\begin{verbatim}
  \includegraphics[width=\textwidth]{figure}
\end{verbatim}
This will allow you to compile your document using either \LaTeX{} or
pdf\LaTeX{} without changing your source file: you can in fact have
both \File{figure.eps} and \File{figure.pdf} in your working directory,
and the proper one will be picked up according to the processing method
you choose.

Figures should be in general be made available in either \texttt{eps} (or \texttt{pdf}) format.
\texttt{png} format can be used for event displays.
However, ATLAS papers should only include \texttt{pdf} figures (and \texttt{png}).
This also implies that pdf\LaTeX{} should be used for compilation.
% Additionally, a \texttt{pdf} version of the plots can be
% useful in case \verb|pdflatex| is used to produce a publication.
%Colour versions are appropriate for talks, and black-and-white
%versions are necessary for the publication itself.

It is a good habit to keep your graphics files in a separate
sub-directory (e.g.\ in \File{figures/}. 
In this case you can include them by mentioning it explicitly every time:
\begin{verbatim}
  \includegraphics[width=\textwidth]{figures/figure}
\end{verbatim}
or by telling the \Package{graphicx} package where to look
for them, by using this command:
\begin{verbatim}
  \graphicspath{{figures/}}
\end{verbatim}

If you use a modern version of \TeX\ Live, it creates PDF files automatically from EPS files
(if they do not exist) when you use \File{pdflatex}.
An EPS file with the name \File{picture1.eps} will lead to a PDF file with the name
\File{picture1-eps-converted-to.pdf}.
If you have a lot of figures in many different directories, you may want to clean up the PDF files every so often.
You can use the command \verb|make cleanepstopdf| to achieve this.
You should adjust the top-level figures directory in the \File{Makefile} accordingly.


%-------------------------------------------------------------------------------
\subsection{Subfigures}

An example figure can be seen in Figure~\ref{fig:example}.
The standard options to use for the positioning are \Option{htbp}.
If you get a couple of lines of text at the top of the page,
make sure the figure is separated from the rest of the text with blank lines and/or try dropping the \Option{h} option.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.5\columnwidth]{AtlasExample}
  \caption{An example ATLAS figure.}
  \label{fig:example}
\end{figure}

A figure with subfigures can be made as shown in the example of
Figure~\ref{fig:subfigexample}. In this example the \Package{subfig} package is used.
The syntax with the \Package{subcaption} and \Package{subfigure} packages is very similar.
The following commands were used to produce Figure~\ref{fig:subfigexample}:
{\footnotesize
\begin{verbatim}
\begin{figure}[htbp]
  \centering
  \subfloat[One subfigure example]{
    \includegraphics[width=0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample1}
  }
  \subfloat[Another subfigure example]{
    \includegraphics[width= 0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample2}
  }
  \caption{Subfigure example.
    \protect\subref{fig:SubfigureExample1} shows the cross-section as a function of $E_{\text{T,jet}}$ and 
    \protect\subref{fig:SubfigureExample2} shows exactly the same thing!}
  \label{fig:subfigexample}
\end{figure}
\end{verbatim}
}

You refer to the main figure using the usual \verb|\ref| command, e.g.\ see \Fig{\ref{fig:subfigexample}}.
You can refer to the subfigures using either the syntax \verb|\ref{fig:subfiglabel}| 
(e.g.\ see \Fig{\ref{fig:SubfigureExample2}}) or\\
\verb|\ref{fig:mainfiglabel}\subref{fig:subfiglabel}|
(e.g.\ see \Fig{\ref{fig:subfigexample}\subref{fig:SubfigureExample1}}).
Note that if you use the \Package{subfig} package and want to use the labels of the subfigures in the caption,
you have to use the syntax \verb|\protect\subref{fig:SubfigureExample1}|.
The packages \Package{subfigure} and \Package{subcaption} do not need protect, but it does not do any harm.

\begin{figure}[htbp]
  \centering
  \subfloat[One subfigure example.]{
    \includegraphics[width=0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample1}
  }
  \subfloat[Another subfigure example.]{
    \includegraphics[width= 0.45\textwidth]{AtlasExample}
    \label{fig:SubfigureExample2}
  }
  \caption{Subfigure example.
    \protect\subref{fig:SubfigureExample1} shows the cross-section as a function of $E_{\text{T,jet}}$ and 
    \protect\subref{fig:SubfigureExample2} shows exactly the same thing!}
  \label{fig:subfigexample}
\end{figure}


%-------------------------------------------------------------------------------
\subsection{Positions of figures and tables}

In an ATLAS paper, all figures and tables should be printed before the conclusions.
You can achieve this by using the macro \Macro{FloatBarrier} from the
\Package{placeins} package.

In general, as mentioned above, you should separate the figure and table environments from the text by blank lines.
This helps the line numbers. The standard options to use for the placement are \Option{[htbp]}.


%-------------------------------------------------------------------------------
\subsection{Math mode macros}%
\label{sec:math}
%-------------------------------------------------------------------------------

The correct \LaTeX\ macros for math mode are \textbackslash(\ldots\textbackslash)
and not \(\$\ldots\$\) (which are \TeX\ primitives),
even though the \TeX\ primitives are used by most people.
\ADOCnew{06-00-00} The standard ATLAS bibliography and template files use the correct \LaTeX\ macros and
the documentation, example files will also be adjusted to use them.

If you are using a version of \LaTeX\ from before 2015, you may have problems
if you use the \LaTeX\ delimiters in captions and want to make as list of tables or figures.
If this is the case, just switch to \TeX\ primitives in the caption (or subcaption).


%-------------------------------------------------------------------------------
\subsection{\pT or \ET, that is the question}

Bold math should be automatically invoked in titles.
This short section tests whether that works properly.
It is of course good if things like \pT and \ET are automatically in bold face in
a header and normal font in the text (and table of contents).

With the current setup, this works OK. 
However, if you just use the option \Option{koma}, which then typesets titles using a sans serif font,
the $p$ and $E$ are typeset with a serif font and \textsf{T} is typeset with a sans serif font,
which is probably not what one wants!
Work is still ongoing to find the optimal set of options
--- search for \texttt{detect} in the \Package{siunitx} manual, to see the complete set of possibilities.
This is not a problem for the ATLAS preprint style as it uses a serif font for the section titles.


%------------------------------------------------------------------------------
\section{Recommended packages}

A vast number of \LaTeX\ packages are available.
In this section I collect a few useful packages that I recommend using.

\begin{description}
  \item[cleveref] Means that constructs like \verb|Fig.~\ref{fig:one}| or
  \verb|\Fig{\ref{fig:one}}| are no longer necessary.
  Instead just use \verb|\cref{fig:one}|.
  The package decides if it is a figure, table or equation and
  adds the appropriate text.
  At the beginning of sentences use \Macro{Cref}.
  This package is included by default if you use \Package{atlaspackage}.
  You can customise its use with the \Option{capsref} and \Option{abbrevref} options.
  If you include the package yourself, use \Macro{usepackage\{cleveref\}} to get \enquote{fig.} etc. and
  use \Macro{usepackage[capitalize]\{cleveref\}} to get \enquote{Fig.} etc.

  \item[heppennames] A package that defines most elementary particle, mesons and baryons in a
  consistent way. Optionally the symbols can be upright or italic.
  The package is included if you pass the option \Option{hepparticle} to \Package{atlasphysics}.
  You can use the package \Package{hepnicenames} instead, which uses more intuitive names for the particles,
  but is not as systematic.

  \item[diffcoeff] A useful package for differentials.
  \ADOCnew{12.0.0} The package is included if you pass the option \Option{full} to \Package{atlaspackage}.
  If the document language is set to \Option{USenglish},
  a slanted \textit{d} is used in differentials,
  while an upright \textrm{d} is used for other languages.
  I recommend \Macro{dl2x} to get a nice spacing for the differential in an integral,\\
  % diffcoeff tweaks for older TeX Live versions.
  \ifthenelse{\AtlasTeXLiveVersion < 2018}{%
    \emph{Examples are not complete as \Package{diffcoeff} package not available for older versions of TeX Live.\\}}{}
  e.g.\ \verb|\int f(x) \dl2x| gives 
  \ifthenelse{\AtlasTeXLiveVersion < 2018}{XXX, while}{\(\int f(x) \dl2x\), while}\\
  \verb|\int f(x) \dl0x| or \verb|\int f(x) \dl x| gives  
  \ifthenelse{\AtlasTeXLiveVersion < 2018}{XXX.}{\(\int f(x) \dl0x\).}
    
  Alternatives are \Package{esdiff} and \Package{derivative},
  but the \Package{derivative} is probably too new to be used in papers.
  You can use a package such as \Package{braket} for Dirac notation etc.

  The package \Package{physics} can also be used for differentials, matrices and more.
  As the name suggests it is geared to physics usage.
  However, the \LaTeX\ community is not very enthusiastic about the way the package is written.
  
  The \Package{commath} package is another alternative,
  but I find the \Package{physics} package to be more reliable when different fonts are used.

  \item[todonotes] Very nice package for adding notes.
  It is used by the \File{atlastodo.sty} style file.
  See \File{atlascomment.sty} for a further example.
\end{description}


%------------------------------------------------------------------------------
\subsection{Other (useful) packages}

In this section I collect a few useful packages that may be useful when preparing a document.
Note that I have only had a cursory read of their documentation,
so some work amy be needed to get them working as they are supposed to.
\begin{description}
  \item[snapshot] As the first paragraph of the documentation quotes:
    \begin{quotation}
      The \Package{snapshot} package helps the owner of a \LaTeX\ document obtain a list of the external dependencies of the document,
      in a form that can be embedded at the top of the document.
      To put it another way, it provides a snapshot of the current processing context of the document,
      insofar as it can be determined from inside \LaTeX.
  \end{quotation}
  It can also be used to arrange that the document is processed with the same versions of everything.
  I tried the package once, and it gave an error compiling.
  However, even if the compilation gives and error
  you can look at the resulting \File{.dep} file to get a list of all packages and versions used in a document.
  This may be helpful for debugging problems.

  \item[changes] The \Package{changes} package is another way of recording changes and adding comments.
    The \Package{todonotes} package is used to do some of this and is integrated into the \Package{atlastodo} style file.
    The \Package{changes} is supposed to work much like change markup in LibreOffice, Microsoft Office etc.
\end{description}


%-------------------------------------------------------------------------------
\section{Remarks on units and symbols}%
\label{sec:siunitx}
%-------------------------------------------------------------------------------

It is highly recommended to use a units package to format your units properly.
The package \Package{siunitx} works very well and is the package of choice.
Alternatives include \Package{units} and \Package{hepunits},
which is based on \Package{SIunits}.

The basic command to use in \Package{siunitx} is \verb|\SI{20}{\GeV}| to get
\SI{20}{\GeV}. 
There are also several other useful commands for specifying ranges:
\verb|\numrange| for a range of numbers and \verb|SIrange| for a range of numbers with a unit. 
Options exist for specifying how they are formatted.
The options can be set for an individual command or for the whole document.
For example, in this document I have specified the options:\\
\verb|\sisetup{separate-uncertainty, range-units=single, list=units=single}|
and\\
\verb|\sisetup{group-digits=integer, group-minimum-digits=4, detect-all}|.

In addition several extra units are defined:
\begin{itemize}
\item \verb|\micron| for \si{\micron};
\item \verb|\mrad| for \si{\mrad};
\item \verb|\nb| for \si{\nb};
\item \verb|\pb| for \si{\pb};
\item \verb|\fb| for \si{\fb}.
\end{itemize}
Use the syntax \verb|\SI{20.3}{\per\fb}| to get \SI{20.3}{\per\fb}.

Some things to note about using \Package{siunitx}:
\begin{itemize}
\item It tries to isolate itself from other packages.
  If you just want to write \si{\GeV} in your text,
  then you must write \verb|\si{\GeV}|.
\item It also contains two new column specifiers for tables ``S'' and ``s'',
  which are extremely useful for formatting tables properly.
\end{itemize}

% The option names are somewhat different for \TeX\ Live 2009,
% as this contained \Package{siunitx} Version 1.
% You can use the older options by including \Package{atlaspackage} with the 
% option \Option{texlive=2009}.
% You also have to turn off the inclusion of \File{atlasunits.sty} by including the option \Option{units=false} with
% the \Package{atlasphysics} package.


%-------------------------------------------------------------------------------
\section{\texttt{atlaslatex} directories and Git}
\label{sec:gitsvn}
%-------------------------------------------------------------------------------

There is some flexibility in how you set up your directory structure for using \Package{atlaslatex}.
By default the \Package{atlaslatex} style files are in the \File{latex} subdirectory and the
logos are in \File{logos}. This structure assumes that you will make a separate directory tree
for each document that you create.
If you want to include these files in Git or SVN, note that you only need to add the
\File{latex}, \File{logos} and \File{bib} directories of the \Package{atlaslatex} package to Git.
In order to create a new document, you also need the \File{template} directory.
For a paper, you also need the \File{acknowledgements} directory.

If you want use a centrally installed \Package{atlaslatex} package, then you would usually unpack the\\
\File{atlaslatex-X.Y.Z.tds.zip} file into your \File{texmf} tree --- see \cref{sec:texmf}.

If you want to use another setup, you should adjust the directory in \File{latex/atlaslatexpath.sty} appropriately.
This would enable you to maintain a single copy of each \Package{atlaslatex} version and easily switch between versions.
For example, you specify:
\verb|\def\input@path{{../atlaslatex-10.0.0/latex/}}|
in \File{latex/atlaslatexpath.sty}
to use version 10.0.0 of the \Package{atlaslatex} package, which you have unpacked into the directory tree
\File{../atlaslatex-10.0.0}.
Such a structure makes it very easy to switch between \Package{atlaslatex} versions without breaking anything!

% If you want to use another setup, you should set the variable \Macro{ATLASLATEXPATH} appropriately
% at the beginning of your document. This would enable you to maintain a single copy of each 
% \Package{atlaslatex} version and easily switch between versions.
% For example, you give the command\\
% \verb|\newcommand*{\ATLASLATEXPATH}{../atlaslatex-01-08-00/}|
% to use version 01-08-00 of the \Package{atlaslatex} package, which you have unpacked into the directory tree
% \File{../atlaslatex-01-08-00}.
% Such a structure makes it very easy to switch between \Package{atlaslatex} versions without breaking anything!


%-------------------------------------------------------------------------------
\section{Platforms and \LaTeX\ versions}
\label{sec:version}
%-------------------------------------------------------------------------------

The \Package{atlasdoc} class should in principle work both with \LaTeX{} and pdf\LaTeX{}.
However, the collection is no longer tested with \LaTeX,
so I strongly recommend to use pdf\LaTeX, which is the default.

I would expect everything to work with \TeX\ Live 2013 or later.
You should just set the option \Option{texlive} appropriately.
This is best done in the document class, as the option is then passed to all other packages.
Examples of changes include some option names for \Package{siunitx}.

% If for example you have \TeX\ Live 2013, add the option \Option{texlive=2013} to the document class.
% This will then include \Package{siunitx} with the correct options for Version 1.
% It will also switch to \Option{unit=false} to \Package{atlasphysics}
% and use option \Option{txfonts} in \Package{atlasdoc}.

\ADOCnew{04-00-00} If you use the \Package{biblatex} package,
the default is to use the \texttt{biber} backend.
% For \TeX\ Live versions earlier than 2013, it may be better to use \texttt{bibtex}.
% To do this, pass the option \Option{backend=bibtex} to \Package{atlaspackage}.

The \Package{atlaslatex} package should work under Linux, macOS and Windows.
Details on the installations that I use for testing things
and how you should set up your system can be found on the PubCom LaTEX FAQ~\cite{latex-faq}.


%-------------------------------------------------------------------------------
\section{Installation of \Package{atlaslatex} in \File{texmf} tree}%
\label{sec:texmf}
%-------------------------------------------------------------------------------

As discussed above, the \texttt{atlasdoc} class and the style files can all be found in the 
\File{latex} subdirectory. The template documents are usually set up to pick up the style files from there.
If you want to use the centrally installed version,
you should first copy \File{Makefile}, the \File{template} directory and the \File{bib} directory from 
\File{\$\{HOME\}/texmf/source/atlaslatex} to the directory where you want to create your document.
For the main document, you can then use the command 
\texttt{make newpapertexmf}, \texttt{make newnotetexmf} or \texttt{make newbooktemmf} to get a template which uses the
centrally installed style files.

If you want to install the package in a central area, use the \File{atlaslatex-X.Y.Z.tds.zip} file.
Change your directory to \File{\$\{HOME\}/texmf} and unzip the file there.
% To do it by hand you can do:
% \begin{itemize}
% \item unpack the tarball;
% \item copy the \texttt{latex} directory to \File{\$\{HOME\}/texmf/tex/latex/atlaslatex};
% \item copy the contents of the \File{bib} directories 
%   to \texttt{\$\{HOME\}/texmf/bib}.
% \end{itemize}
% It is more complicated to checkout part of a Git repository.
% Hence the method described above is the recommended way of installing
% \Package{atlaslatex} in your \File{texmf} tree.
% You can also checkout the two directory trees from SVN:
% {\small
% \begin{verbatim}
% cd ~/texmf/tex/latex
% svn co svn+ssh://svn.cern.ch/reps/atlasgroups/pubcom/latex/atlaslatex/trunk/latex atlaslatex
% cd ~/texmf
% svn co svn+ssh://svn.cern.ch/reps/atlasgroups/pubcom/latex/atlaslatex/trunk/bibtex
% \end{verbatim}
% }
% The advantage of using SVN is that you can keep the package up to date, by just giving the command
% \verb|svn update| in the two directories.
% If you already have a \File{bibtex} directory,
% first move it out of the way, then checkout from SVN
% and then move the contents of the old directory back into the \File{bibtex} tree.

% Under Windows, it appears to be better to use \texttt{https} instead of \texttt{svn+ssh}.
% You should therefore checkout:\\
% \verb|https://svn.cern.ch/reps/atlasgroups/pubcom/latex/atlaslatex/trunk|

In the template files, you have to use the command
\texttt{make newpapertexmf} or \texttt{make newnotetexmf} or simply comment out the line
\verb|\RequirePackage{latex/atlaslatexpath}|
% \begin{center}
%   \begin{tabular}{ll}
%     From & To \\
%     \midrule
%     \verb|\newcommand*{\ATLASLATEXPATH}{latex/}|    & \verb|\newcommand*{\ATLASLATEXPATH}{}| \\
%   \end{tabular}
% \end{center}

If you are using traditional \BibTeX\ you also have to change\\
\verb|\bibliographystyle{bib/bst/atlasBibStyleWoTitle}| to\\
\verb|\bibliographystyle{atlasBibStyleWoTitle}|

The \Option{texmf} option in \Package{atlasphysics} is not strictly necessary if you use the class \Package{atlasdoc},
but it does not do any harm.


\appendix
\clearpage
%-------------------------------------------------------------------------------
\section{Makefile}
%-------------------------------------------------------------------------------
\label{sec:makefile}

This section documents what the \File{Makefile} does when it creates a new document
or compiles one.

When a new paper draft is created using the command\\
\texttt{make newpaper BASENAME=GROUP-YYYY-XX-PAPER}\\
the following files are created in the main directory.
If a template filename is given in the table
it is taken from the \texttt{template} directory,
otherwise empty files are created.
\begin{center}
  \begin{tabular}{ll}
    \mcc{\texttt{template}} & \mcc{\texttt{main}} \\
    \midrule
    \texttt{atlas-paper.tex} & \texttt{GROUP-YYYY-XX-PAPER.tex} \\
    \texttt{atlas-paper-metadata.tex} & \texttt{GROUP-YYYY-XX-PAPER-metadata.tex} \\
    \texttt{atlas-auxmat.tex} & \texttt{GROUP-YYYY-XX-PAPER-auxmat.tex} \\
    \texttt{atlas-hepdata.tex} & \texttt{GROUP-YYYY-XX-PAPER-hepdata.tex} \\
    & \texttt{GROUP-YYYY-XX-PAPER-defs.sty} \\
    & \texttt{GROUP-YYYY-XX-PAPER.bib}
  \end{tabular}
\end{center}
The following string substitutions are made in \texttt{GROUP-YYYY-XX-PAPER.tex}:
\begin{center}
  \begin{tabular}{ll}
    \mcc{Old string} & \mcc{New string} \\
    \midrule
    \texttt{atlas-document} & \texttt{GROUP-YYYY-XX-PAPER} \\
    \texttt{texlive=2020} & \texttt{texlive=YYYY} \\
  \end{tabular}
\end{center}
The \TeX\ Live version is changed to \texttt{YYYY} (if given). Otherwise it is set to 2020.

The same thing is done for an ATLAS supporting note made with the command\\
\texttt{make newnote BASENAME=GROUP-YYYY-XX-INT1},\\
except that the main file template is taken from
\texttt{atlas-note.tex},
the metadata template is taken from \texttt{atlas-note-metadata.tex},
and the auxiliary material and HEPData files are not created.

The standard sequence of commands to compile a document is
\texttt{pdflatex, biber, pdflatex, pdflatex}.
You can change the \texttt{\%.pdf} target if necessary.
Better is to use \texttt{latexmk} via the target \texttt{run\_latexmk}.
I recommend you set this as the default command.

%-------------------------------------------------------------------------------
\section{Journal templates}
%-------------------------------------------------------------------------------
\label{sec:journal}

This section contains some information on where the \LaTeX\ templates for the different journals can be found and how to use them.
With the advent of the ATLAS preprint style and its use for ATLAS publications, 
it should no longer be necessary to format papers in the style used by the journals.
However, for papers that are written by a limited number of authors
the journal may require that the paper be submitted using its style.

The directory \File{journal} contains a very basic paper outline with the preamble needed for different journals.
So far the \Package{atlaslatex} package has been tested with the classes for Elsevier and APS journals and the style file used for JHEP and JINST.
The journal templates turn off the use of \Package{biblatex}
by adding the option \Option{biblatex=false} to \Package{atlaspackage}.
I have not tested if it is possible to use \Package{biblatex}.

\begin{description}
\item[Elsevier]Elsevier uses the \texttt{elsarticle} class which should be already installed if you have a standard 
  \TeX\ Live distribution. 
  It can also be found at \url{http://www.elsevier.com/locate/latex}.
  
\item[APS]APS journals use REV\TeX. This is also usually installed.
  It can also be found at \url{https://journals.aps.org/revtex}.
  Note that you have to specify the author after \verb|\begin{document}| with this class.
  Hence you should comment out the definition in your metadata file,\\
  e.g.\ \File{mydocument-metadata.tex}.
  If you want line numbers in a document typeset using REV\TeX, it is best to use the class option \Option{linenumbers}.
  In addition you should include \Package{atlaspackage} with the option \Option{lineno=false}.
  
\item[JHEP]The package can be downloaded from \url{http://jhep.sissa.it/jhep/help/JHEP_TeXclass.jsp}.
  It contains a style file \File{jheppub.sty} as well as a \BibTeX\ style file \File{JHEP.bst}. 
  If the author of the paper is not the the ATLAS Collaboration,
  you should use the macros \Macro{author} and \Macro{affiliation} to specify the names and their instiutions (see the documentation)
  and should NOT include the \Package{authblk} package.

\item[JINST]The package can be downloaded from \url{https://jinst.sissa.it/jinst/help/helpLoader.jsp?pgType=author}.
  It contains a style file \File{jinstpub.sty} as well as a \BibTeX\ style file \File{JHEP.bst}.
  The information on authors is the same as for JHEP.
\end{description}


%-------------------------------------------------------------------------------
\section{From \texttt{atlasnote} to \texttt{atlasdoc}}
\label{sec:oldnote}
%-------------------------------------------------------------------------------

The \texttt{atlasdoc} class replaces and supersedes \texttt{atlasnote}.
The decision was taken to give the class a new name, as it is supposed to be
able to be used for (almost) all ATLAS documents.
Some small changes in the user setup are necessary to use the new
class, style files and templates.

All style files are collected in the \texttt{latex} subdirectory.
It is assumed that this directory is a direct subdirectory of you main \LaTeX\ file.
If you want to keep the style files in a central place you can either put them in
\verb|${HOME}/texmf/tex/latex| or create a link from your main directory to the location of
your \texttt{latex} directory.

The main changes the user has to make are:
\begin{itemize}
\item Change the class name from \texttt{atlasnote} to \texttt{latex/atlasdoc};
\item Specify the document language as an option: UKenglish or USenglish;
\item Add \verb|\usepackage{latex/atlaspackage}| at the beginning of the document;
\item Change \verb|\usepackage{atlasphysics}| to \verb|\usepackage{latex/atlasphysics}|; 
\item Use the macro \Macro{AtlasTitle} instead of \Macro{title}.
\end{itemize}

The language specification means that dates etc.\ are also formatted according to 
the document language. 
If you use the package \Macro{csquotes}, quotation symbols are also consistently and properly set
when you use \Macro{enquote}.

All the documentation uses \texttt{biblatex} and \texttt{biber} instead of traditional \BibTeX.
The templates provide information on how to make the change in your own document.
The default document settings also use \texttt{biblatex} and \texttt{biber}.

\ADOCnew{01-00-00} The same macro names are used in both \Package{atlasdoc} and
\Package{atlascover} so that title, journal, version number and abstract only need to be specified once.
This means that if you start from an old preamble the following changes should be made:
\begin{center}
  \begin{tabular}{ll}
    Old	& New\\
    \midrule
    \Macro{title} & \Macro{AtlasTitle}\\
    \Macro{draftversion} & \Macro{AtlasVersion}\\
    \Macro{atlasnote} & \Macro{AtlasNote}\\
    \Macro{journal} & \Macro{AtlasJournal}\\
    \Macro{abstracttext} & \Macro{AtlasAbstract}
  \end{tabular}
\end{center}
If you use the old macro names 
\Macro{draftversion}, \Macro{journal}, \Macro{abstracttext},
they will continue to work in the document itself, but not on the cover page.

When you want to circulate a draft with cover pages, 
you also need to set the macro \Macro{AtlasRefCode}.
This replaces \Macro{AtlasCoverNumber} as it is used in several places.

The class and style files have been cleaned up and things 
that were thought to no longer be necessary have been removed.
% These pieces have been collected in \texttt{obsolete/atlasnote-obsolete.sty} in case they are needed.
% If something important has got lost, please let me know.

The \Package{subfigure} package has been replaced with \Package{subfig}, as \Package{subfigure} is now deprecated.
If you use \Package{subfig}, then you have to use \Macro{subfloat} instead of \Macro{subfigure}.
If you want to continue to use \Package{subfigure} include \Package{atlaspackage} with the option
\Option{subfigure=true}. 
You should also comment out the \Macro{usepackage\{subfigure\}}.

Similarly, if you do not want to include \Package{siunitx} set
the option \Option{siunitx=false}.

The option \verb|\skipbeforetitle{<length>}| used to set the distance between
the title page header and the note title. 
Given that stretchable space is now used, such an option is no longer appropriate.
It can be given, but will be ignored.
%The default value should be fine for most notes, but in case you have a long list of
%authors or a lengthy abstract you can use this command to buy
%some extra space. Note that \verb|<length>| can also be negative
%(use it at your own risk!).

%-------------------------------------------------------------------------------
\section{History}
%-------------------------------------------------------------------------------

Quite a lot of people have contributed to the ATLAS \LaTeX\ templates over time.
Marco Delmastro set them up in the first place and added a number of improvements over time.
Mike Vetterli implemented several changes to the cover pages, including switching to two pages.
Cristina Oropeza, Vasia Mitsou, Chris Hays and Mike Vetterli all made contributions to the preprint cover page.

Sven Menke provided the code so that bold math works in titles correctly.
Thorsten Kuhl had the idea of defining \Macro{ATLASLATEXPATH}, which makes things much more flexible.
Some problems occurred with this scheme \TeX{} Live 2020.
As a result the use of \Macro{ATLASLATEXPATH} was replaced with the \File{atlaslatexpath.sty} style file.

Juan Pedro Araque has done most of the work setting up the PO-GitLab project.
This resulted in a much smoother submission process for papers and
an improved handling of auxiliary material.

Knut Zoch provided the code that fixed the line numbering problems with AMS Math \LaTeX\ environments.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-10.0.0}}
\label{sec:atlaslatex10}
%-------------------------------------------------------------------------------

\ADOCnew{10.0.0} switches to Semantic Versioning.

The major change in this version is in the way that the class and style files are included.
This had to be changed as the result of a bug introduced in the October 2020 update of \LaTeX.
The \LaTeX{} update led to options being ignored when passed to a document class or a style file,
if the filename contained a directory.
While this bug will probably be fixed at some point,
it in general appears to be better to adjust the macro \Macro{input@path}
to specify the directory that should be searched for the ATLAS \LaTeX{} packages.
Hence a new style file \File{atlaslatexpath.sty} has been introduced and should be loaded using
\begin{tcblisting}{listing only}
\RequirePackage{latex/atlaslatexpath}
\end{tcblisting}
before the \Macro{documentclass}.

This change implies that all main files have to be updated.
A script \File{scripts/atlaslatex\_2020.sh} is provided that should make the necessary changes.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-05-00-00}}
\label{sec:atlaslatex5}
%-------------------------------------------------------------------------------

\ADOCnew{05-00-00} is the first version set up
to be fully compatible with the PO-GitLab scheme for papers.

Separate (dummy) files for auxiliary material and HEPData tables are created for new papers.
The \verb|make auxmat| command has been renamed to \verb|make newdata|,
as the auxiliary material for the webpage is now separated
from a separate file for tables etc.\ for HEPData.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-04-00-00}}
\label{sec:atlaslatex4}
%-------------------------------------------------------------------------------

\ADOCnew{04-00-00} The \File{Makefile} for \Package{atlaslatex}
has been restructured to reduce duplications and make separate commands for a new paper and a new note.
\texttt{biber} is now the default backend for \Package{biblatex},
as this allows the use of the \enquote{related} field for Errata.
Errata are included in the ATLAS bibliography file.
Metadata for notes and papers are now separate templates to prepare for them being created directly from Glance.
This is the first version that is designed for the Glance/Git integration.
As the above changes are quite major, there is a jump in the main version number.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlaslatex-02-00-00}}
\label{sec:atlaslatex2}
%-------------------------------------------------------------------------------

\ADOCnew{02-00-00} Only the \KOMAScript\ classes are supported.
At the same time, the option BOOK was introduced, which uses \Package{scrbook} as the base class.
This is more suitable for long documents such as a TDR.

Several options, which make maintenance more difficult have been removed:
\Option{maketitle}, \Option{nomaketitle}, \Option{koma}.
In addition, support for \TeX\ Live versions older than 2009 has been removed.
% A version of the class with these options, which should still work with \TeX\ Live 2007,
% but without the \Option{BOOK} option is available as \File{atlasdoc1.cls}.
% However, the class (\Package{atlasdoc1}) will not be actively maintained or developed any more.
% If you want to explicitly load the \Package{atlascover} package,
% you should load \Package{atlascover1} when using \Package{atlasdoc1}.

The options \Option{cernpreprint}, \Option{preprint} and \Option{auxmat} are no longer available
in \Package{atlascover}.
You should pass these to \Package{atlasdoc} instead, as the title pages are now part of the main class.


%-------------------------------------------------------------------------------
\subsection{Changes in \texttt{atlascover-01-00-00}}
\label{sec:oldcover}
%-------------------------------------------------------------------------------

\ADOCnew{01-00-00} The same macro names are used in both \Package{atlasdoc} and
\Package{atlascover} so that title, journal and version number only need to be specified once.
This means that if you start from an old cover page the following changes have to be made:
\begin{center}
  \begin{tabular}{ll}
    Old                            & New                   \\
    \midrule
    \Macro{AtlasCoverPaperTitle}   & \Macro{AtlasTitle}    \\
    \Macro{AtlasCoverNumber}       & \Macro{AtlasRefCode}  \\
    \Macro{AtlasCoverPaperVersion} & \Macro{AtlasVersion}  \\
    \Macro{AtlasCoverJournal}      & \Macro{AtlasJournal}  \\
    \Macro{AtlasCoverAbstract}     & \Macro{AtlasAbstract}
  \end{tabular}
\end{center}

Note that \Package{atlaspreprint} is integrated into \Package{atlascover} and not maintained as a separate style file.
To get the CERN preprint front page, you have to include the option \Option{cernpreprint} when you invoke \Package{atlasdoc}.
If you start from an old preprint front page the following changes have to be made:
\begin{center}
  \begin{tabular}{ll}
    Old                              & New                   \\
    \midrule
    \Macro{PreprintCoverPaperTitle} & \Macro{AtlasTitle}    \\
    \Macro{PreprintJournalName}     & \Macro{AtlasJournal}  \\
    \Macro{PreprintCoverAbstract}   & \Macro{AtlasAbstract}
  \end{tabular}
\end{center}
The following changes are needed for the macros:
\begin{itemize}
\item The macro \Macro{AtlasCoverEdBoardMember} only has one argument, as a generic email list now exists for every EdBoard.
\end{itemize}


==> bib/doc/atlas_physics/Makefile <==
#------------------------------------------------------------------------------
# Makefile to make atlas_physics documentation
#------------------------------------------------------------------------------

BASENAME1 = atlas_physics
BASENAME2 = atlas_hepphysics
TEXLIVE = 2020

.PHONY: clean cleanpdf

atlas_physics:
	make -f ../Makefile run_latexmk BASENAME=$(BASENAME1)

atlas_hepphysics:
	if [ $(TEXLIVE) -ge 2013 ]; then \
		make -f ../Makefile BASENAME=$(BASENAME2); \
	fi

texlive:
	make -f ../Makefile texlive BASENAME=$(BASENAME1) TEXLIVE=$(TEXLIVE)
	make -f ../Makefile texlive BASENAME=$(BASENAME2) TEXLIVE=$(TEXLIVE)

clean:
	make -f ../Makefile clean

cleanpdf:
	-rm $(BASENAME1).pdf
	-rm $(BASENAME2).pdf

cleanall: clean cleanpdf


==> bib/doc/atlas_physics/atlas_physics_body.tex <==
%-------------------------------------------------------------------------------
\section{\File{atlasphysics.sty} style file}
\label{sec:atlasphysics}
%-------------------------------------------------------------------------------

The \File{atlasphysics.sty} style file implements a series of useful
shortcuts to typeset a physics paper, such as particle
symbols.

Options are parsed with the \Package{kvoptions} package, which is included by default.
The style file can included in the preamble of your paper with the usual
syntax:
%
\begin{tcblisting}{listing only}
\usepackage{atlasphysics}
\end{tcblisting}
%
The file is actually split into smaller files,
which can be included or not using options.
The following options are available, where the default setting is given in parentheses:
\begin{description}
\item[BSM](false) BSM and SUSY particles.
\item[hion](false) Useful macros for heavy ion physics.
\item[jetetmiss](false) Useful macros for Jet/Etmiss publications.
\item[journal](true) Journal abbreviations and a few other definitions for references.
\item[math](false) A few extra maths definitions.
\item[misc](true) Miscellaneous definitions that are often used.
\item[other](false) Definitions that used to be in \File{atlasphysics.sty},
  but are probably too specialised to be needed by most people.
\item[particle](true) Standard Model particles and some combinations.
\item[hepparticle](false) Standard Model particles and some combinations using the \Package{hepparticle} package.
  This option will supersede \Option{particle} at some time.
\item[process](false) Some example processes.
  These are not included by default as the current choice is rather arbitrary
  and certainly not complete.
\item[hepprocess](false) Some example processes using the \Package{hepparticle} package.
  These are not included by default as the current choice is rather arbitrary
  and certainly not complete.
  This option will supersede \Option{process} at some time.
\item[unit](true) Units that used to be defined -- not needed if you use \Package{siunitx} or \Package{hepunits}.
\item[xref](true) Useful abbreviations for cross-references.
\item[texlive=YYYY](2020) Set if you use an older version of \TeX\ Live like 2013.
\item[texmf](true) Use the syntax \Macro{usepackage\{package\}}
  instead of \Macro{usepackage\{\textbackslash ATLASLATEXPATH package\}} to include packages.
  This is needed if you install \Package{atlaslatex} centrally,
  rather than in a \File{latex} subdirectory.
\end{description}
Note that \Option{BSM} and \Option{BSM=true} are equivalent.
Use the syntax \Option{option=false} to turn off an option.
\ADOCnew{10.0.0} \Macro{ATLASLATEXPATH} is no longer used,
so the option \Option{texmf} has been set to \Option{true}.

If the  option \Option{texmf} is included, the subfiles are included using the command:
\verb|\RequirePackage{atlasparticle}| etc. instead of \verb|\RequirePackage{\ATLASLATEXPATH atlasparticle}|.
\ADOCnew{10.0.0} This is now the default option.

All definitions are done in a consistent way using \verb|\newcommand*|.
All definitions use \verb|\ensuremath| where appropriate and are terminated with
\verb|\xspace|, so you can simply write {\verb|\ttbar production| instead of
\verb|\ttbar\ production| or \verb|\ttbar{} production| to get \enquote{\ttbar production}.

The \Package{hepparticles}~\cite{hepparticles} package has uniform definitions for many Standard Model and BSM particles.
In fact you should use the package \Package{heppennames} and/or \Package{hepnicenames},
which contain many predefined particles.
These packages load \Package{hepparticles}, which can then be used to define more particles if you need them.
One very nice feature of these packages is that you can switch between italic and upright symbols via an option.

See \cref{sec:old}} for details on changes that were introduced when
when going from version 00-04-05 of \Package{atlasnote}
to version 01-00-00 of \Package{atlaslatex}.
Let me know if you spot some other changes that are not documented here!

Changes to the contents that might affect existing documents are given in \cref{sec:change}.

The following sections list the macros defined in the various files.


==> bib/doc/atlas_physics/atlas_physics_changes.tex <==
\onecolumn
%-------------------------------------------------------------------------------
\section{Changes}
\label{sec:change}
%-------------------------------------------------------------------------------

\textbf{Version 05-08-00} of \Package{atlaslatex} includes a new \File{atlassnippets.sty} style file.
This is supposed to contain snippets of text that are useful in many papers and/or notes.

\textbf{Version 01-08-01} of \Package{atlaslatex} includes quite a few definitions from the Jet/Etmiss group.
A new style file has been created \File{atlasjetetmiss.sty} that is not included by default.
Some of the definitions from the Jet/ETmiss group are of more general use and so have been merged into existing style files:
\begin{description}
\item[atlasmisc.sty] List of Monte Carlo generators expanded:
  \Macro{POWHEGBOX}, \Macro{POWPYTHIA}.
  Add MC macros with suffix \enquote{V} for version number.
  \Macro{kt}, \Macro{antikt}, \Macro{Antikt}, \Macro{LO}, \Macro{NLO}, \Macro{NLL}, \Macro{NNLO},
  \Macro{muF}, \Macro{muR}.
  Added macros \Macro{Runone}, \Macro{Runtwo}, \Macro{Runthr},
  Added \Macro{radlength} and \Macro{StoB}.
  Added some standard \(b\)-tagging terms:
  \Macro{btag}, \Macro{btagged}, \Macro{bquark}, \Macro{bquarks}, \Macro{bjet}, \Macro{bjets}.
\item[atlasparticle.sty] Now includes \Macro{pp}, \Macro{enu}, \Macro{munu},
\item[atlasprocess.sty] Added \Macro{Zbb}, \Macro{Ztt},
  \Macro{Zlplm}, \Macro{Zepem}, \Macro{Zmpmm}, \Macro{Ztptm},
  \Macro{tWb}, \Macro{Wqqbar},
  \Macro{Wlnu}, \Macro{Wenu}, \Macro{Wmunu},
  \Macro{Wjets}, \Macro{Zjets}.
  The definition of \Macro{Hllll} was corrected.
\item[atlasheavyion.sty] \Macro{pp} moved to \File{atlasparticle.sty}.
\end{description}

This version also introduced the (optional) use of the \Package{heppennames} package.
The style files \File{atlashepparticle.sty} and \File{atlashepprocess.sty}
are intended to replace \File{atlasparticle.sty} and \File{atlasprocess.sty}.
Several particle definitions were removed from the \Package{atlasparticle} package,
as they just enable a few Greek letters: \(\pi\), \(\eta\) and \(\psi\) to be used directly in text mode.
In addition, the primed \(\Upsilon\) resonances, e.g.\ \(\Upsilon''\),
as well as \(D^{**}\) were removed.
as the official names are \Ups{3} etc.,

The definitions of \MeV, \GeV\ etc.\ in \texttt{atlasunit.sty} were updated in order to remove the \texttt{if} tests in them.
The \texttt{if} tests caused a problem in a paper draft, although the reason was not understood.
The new definitions do not introduce extra space before the unit in math mode.


%-------------------------------------------------------------------------------
\section{Old macros}
\label{sec:old}
%-------------------------------------------------------------------------------

With the introduction of \Package{atlaslatex} several macro names have been changed to make them more consistent.
A few have been removed. The changes include:
\begin{itemize}
\item Kaons now have a capital \enquote{K} in the macro name, e.g.\ \verb|\Kplus| for \Kplus;
\item \verb|\Ztau|, \verb|\Wtau|, \verb|\Htau| \verb|\Atau| have been replaced by
  \verb|\Ztautau|, \verb|\Wtautau|, \verb|\Htautau| \verb|\Atautau|;
\item \verb|\Ups| replaces \verb|\ups|;
  the use of \verb|\ups| to produce \(\Upsilon\) in text mode has been removed;
\item \verb|\cm| has been removed, as it was the only length unit defined for text and math mode;
\item \verb|\mass| has been removed, as \verb|\twomass| can do the same thing and the name is more intuitive;
\item \verb|\mA| has been removed as it conflicts with \Package{siunitx} Version 1, which uses the name
  for milliamp.
\item \Macro{mathcal} rather than \Macro{mathscr} is recommended for luminosity and aplanarity.
\end{itemize}

Quite a few macros are more related to \Zboson physics than they are to LHC physics and have
been moved to the \File{atlasother.sty} file, which is not included by default.
There are also macros for various decay processes, \File{atlasprocess.sty} which are not included by default,
but may be useful for how you can define your favourite process.

It used to be the case that you had to use \verb|\MET{}| rather than just \verb|\MET| to get the spacing right,
as somehow \Package{xspace} did not do a good job for \met.
However, with the latest version of the packages both forms work fine.
You can compare \MET and \MET\ and see that the spacing is correct in both cases.


==> bib/doc/atlas_physics/atlas_physics_defs.tex <==
% Files with references in BibTeX format and biblatex style options
\addbibresource{../../bib/ATLAS.bib}
\addbibresource{atlas_physics.bib}

\graphicspath{{../../logos/}}

% Useful macros for documentation
% \newcommand{\File}[1]{\texttt{#1}\xspace}
% \newcommand{\Macro}[1]{\texttt{\textbackslash #1}\xspace}
% \newcommand{\Option}[1]{\textsf{#1}\xspace}
% \newcommand{\Package}[1]{\texttt{#1}\xspace}

%-------------------------------------------------------------------------------
% Generic document information
%-------------------------------------------------------------------------------
% Set author and title for the PDF file
\hypersetup{pdftitle={ATLAS LaTeX guide},pdfauthor={Ian Brock}}

\AtlasTitle{Symbols defined in \File{atlasphysics.sty}}

\author{Ian C. Brock}
\affil{University of Bonn}

\AtlasAbstract{%
  This note lists the symbols defined in \File{atlasphysics.sty}.
  These provide examples of how to define your own symbols, as well as many symbols
  that are often used in ATLAS documents.

  This document was generated using version \ATPackageVersion\ of the ATLAS \LaTeX\ package.
  The \TeX\ Live version is set to \AtlasTeXLiveVersion.
  It uses the option \Option{atlasstyle}, which implies that the standard ATLAS preprint style is used.
  The language is set to \languagename.
}


==> bib/doc/atlas_physics/atlas_physics_list1.tex <==
\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasjournal.sty}}

Turn on including these definitions with the option \Option{journal=true} and off with the option \Option{journal=false}.

\input{atlasjournal}


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasmisc.sty}}

Turn on including these definitions with the option \Option{misc=true} and off with the option \Option{misc=false}.

\input{atlasmisc}

\noindent A length \Macro{figwidth} is defined that is \SI{2}{\cm} smaller than \Macro{textwidth}.

\noindent Monte Carlo generators and PDFs have an optional argument
that allows you to include the version, e.g.\
\verb|\PYTHIA[8]| to produce \PYTHIA[8] or\\
\verb|\PYTHIA[(v8.160)]| to produce \PYTHIA[(v8.160)].

\noindent A macro \Macro{pTX} is included that allows you to add an extra subscript and/or a superscript to \pT.
e.g.\\
\verb|\pTX| to produce \pTX;\\
\verb|\pTX[2]| to produce \pTX[2];\\
\verb|\pTX[][\text{had}]| to produce \pTX[][\text{had}];\\
\verb|\pTX[3][\text{had}]| to produce \pTX[3][\text{had}].

\noindent A generic macro \verb|\twomass| is defined, so that for example
\verb|\twomass{\mu}{\mu}| produces \twomass{\mu}{\mu} and \verb|\twomass{\mu}{e}| produces \twomass{\mu}{e}.

A macro \verb|\dk| is also defined which makes it easier to write down decay chains.
For example
\begin{verbatim}
\[\eqalign{a \to & b+c\\
   & \dk & e+f \\
   && \dk g+h}
\]
\end{verbatim}
produces
\[\eqalign{a \to & b+c\cr
   & \dk & e+f \cr
   && \dk g+h}
\]
Note that \Macro{eqalign} is also redefined in this package so that \Macro{dk} works.

The following macro names have been changed:\\
\verb|\ptsq| \(\to\) \verb|\pTsq|.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasxref.sty}}

Turn on including these definitions with the option \Option{xref=true} and off with the option \Option{xref=false}.

\input{atlasxref}

\noindent The following macros with arguments are also defined:
\begin{xtabular}{ll}
\verb|\App{1}|  & \App{1}\\
\verb|\Eqn{1}|  & \Eqn{1}\\
\verb|\Fig{1}|  & \Fig{1}\\
\verb|\Refn{1}|  & \Refn{1}\\
\verb|\Sect{1}| & \Sect{1}\\
\verb|\Tab{1}|  & \Tab{1}\\
\verb|\Apps{1}{4}| & \Apps{1}{4} \\
\verb|\Eqns{1}{4}| & \Eqns{1}{4} \\
\verb|\Figs{1}{4}| & \Figs{1}{4} \\
\verb|\Refns{1}{4}| & \Refns{1}{4} \\
\verb|\Sects{1}{4}| & \Sects{1}{4} \\
\verb|\Tabs{1}{4}| & \Tabs{1}{4} \\
\verb|\Apprange{1}{4}| & \Apprange{1}{4} \\
\verb|\Eqnrange{1}{4}| & \Eqnrange{1}{4} \\
\verb|\Figrange{1}{4}| & \Figrange{1}{4} \\
\verb|\Refrange{1}{4}| & \Refrange{1}{4} \\
\verb|\Sectrange{1}{4}| & \Sectrange{1}{4} \\
\verb|\Tabrange{1}{4}| & \Tabrange{1}{4}
\end{xtabular}

The idea is that you can adapt these definitions according to your own preferences (or those of a journal).
Note that the macros \Macro{Ref} and \Macro{Refs} were renamed to \Macro{Refn} and \Macro{Refns}
in \Package{atlaslatex} 08-00-00, as \Macro{Ref} is now defined in the \Package{hyperref} package.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasbsm.sty}}

Turn on including these definitions with the option \Option{BSM} and off with the option \Option{BSM=false}.

The macro \Macro{susy} simply puts a tilde (\(\tilde{\ }\)) over its argument,
e.g.\ \verb|\susy{q}| produces \susy{q}.

For \susy{q}, \susy{t}, \susy{b}, \slepton, \sel, \smu and
\stau, L and R states are defined; for stop, sbottom and stau also the
light (1) and heavy (2) states.
There are four neutralinos and two charginos defined,
the index number unfortunately needs to be written out completely.
For the charginos the last letter(s) indicate(s) the charge:
\enquote{p} for \(+\), \enquote{m} for \(-\), and \enquote{pm} for \(\pm\).

\input{atlasbsm}


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasheavyion.sty}}

Turn on including these definitions with the option \Option{hion=true} and off with the option \Option{hion=false}.
The heavy ion definitions use the package \Package{mhchem} to help with the formatting of chemical elements.
This package is included by \File{atlasheavyion.sty}.

\input{atlasheavyion}

%The following symbols were removed or modified with respect to the original submission
%\input{atlasheavyion-mod}


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasjetetmiss.sty}}

Turn on including these definitions with the option \Option{jetetmiss=true} and off with the option \Option{jetetmiss=false}.

\input{atlasjetetmiss}

\noindent The macro \Macro{etaRange} produces what you would expect:
\verb|\etaRange{-2.5}{+2.5}| produces \etaRange{-2.5}{+2.5} while
\verb|\AetaRange{1.0}| produces \AetaRange{1.0}.
The macro \Macro{avg} can be used for average values:
\verb|\avg{\mu}| produces \avg{\mu}.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasmath.sty}}

Turn on including these definitions with the option \Option{math=true} and off with the option \Option{math=false}.

\input{atlasmath}

\noindent The macro \Macro{spinor} is also defined.
\verb|\spinor{u}| produces \spinor{u}.


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasother.sty}}

Turn on including these definitions with the option \Option{other} and off with the option \Option{other=false}.

\input{atlasother}


==> bib/doc/atlas_physics/atlas_physics_list2.tex <==
\newpage
\onecolumn
%-------------------------------------------------------------------------------
\section{\File{atlassnippets.sty}}

Turn on including these definitions with the option \Option{snippets} and off with the option \Option{snippets=false}.

\input{atlassnippets}
\twocolumn


\newpage
%-------------------------------------------------------------------------------
\section{\File{atlasunit.sty}}

Turn on including these definitions with the option \Option{unit} and off with the option \Option{unit=false}.

\input{atlasunit}

\noindent Lower case versions of the units also exist, e.g.\ \verb|\tev|, \verb|\gev|, \verb|\mev|, \verb|\kev|, and
\verb|\ev|.

As mentioned above, it is highly recommended to use a units package instead of
these definitions. \Package{siunitx} is the preferred package; a good alternative is \Package{hepunits}.
If either of these packages are used \File{atlasunit.sty} is not needed.

Most units that are needed in ATLAS documents are already defined by \Package{siunitx} or
are defined in \File{atlaspackage.sty}.
A selection of them is given below.
In order to use them in your document the unit should be included in
\verb|\si| or \verb|\SI|:\\
\begin{xtabular}{ll}
\verb|\si{\TeV}| & \si{\TeV} \\
\verb|\si{\GeV}| & \si{\GeV} \\
\verb|\si{\MeV}| & \si{\MeV} \\
\verb|\si{\keV}| & \si{\keV} \\
\verb|\si{\eV}|  & \si{\eV} \\
\verb|\si{\TeVc}| & \si{\TeVc} \\
\verb|\si{\GeVc}| & \si{\GeVc} \\
\verb|\si{\MeVc}| & \si{\MeVc} \\
\verb|\si{\keVc}| & \si{\keVc} \\
\verb|\si{\eVc}|  & \si{\eVc} \\
\verb|\si{\TeVcc}| & \si{\TeVcc} \\
\verb|\si{\GeVcc}| & \si{\GeVcc} \\
\verb|\si{\MeVcc}| & \si{\MeVcc} \\
\verb|\si{\keVcc}| & \si{\keVcc} \\
\verb|\si{\eVcc}|  & \si{\eVcc} \\
\verb|\si{\nb}| & \si{\nb} \\
\verb|\si{\pb}| & \si{\pb} \\
\verb|\si{\fb}| & \si{\fb} \\
\verb|\si{\per\fb}| & \si{\per\fb} \\
\verb|\si{\per\pb}| & \si{\per\pb} \\
\verb|\si{\per\nb}| & \si{\per\nb} \\
\verb|\si{\ifb}| & \si{\ifb} \\
\verb|\si{\ipb}| & \si{\ipb} \\
\verb|\si{\inb}| & \si{\inb} \\
\verb|\si{\Hz}|  & \si{\Hz} \\
\verb|\si{\kHz}| & \si{\kHz} \\
\verb|\si{\MHz}| & \si{\MHz} \\
\verb|\si{\GHz}| & \si{\GHz} \\
\verb|\si{\degr}| & \si{\degr} \\
\verb|\si{\m}| & \si{\m} \\
\verb|\si{\cm}| & \si{\cm} \\
\verb|\si{\mm}| & \si{\mm} \\
\verb|\si{\um}| & \si{\um} \\
\verb|\si{\micron}| & \si{\micron} \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasbsm.tex <==
\begin{xtabular}{ll}
\verb|\Azero| & \Azero \\
\verb|\hzero| & \hzero \\
\verb|\Hzero| & \Hzero \\
\verb|\Hboson| & \Hboson \\
\verb|\Hplus| & \Hplus \\
\verb|\Hminus| & \Hminus \\
\verb|\Hpm| & \Hpm \\
\verb|\Hmp| & \Hmp \\
\verb|\ggino| & \ggino \\
\verb|\chinop| & \chinop \\
\verb|\chinom| & \chinom \\
\verb|\chinopm| & \chinopm \\
\verb|\chinomp| & \chinomp \\
\verb|\chinoonep| & \chinoonep \\
\verb|\chinoonem| & \chinoonem \\
\verb|\chinoonepm| & \chinoonepm \\
\verb|\chinotwop| & \chinotwop \\
\verb|\chinotwom| & \chinotwom \\
\verb|\chinotwopm| & \chinotwopm \\
\verb|\nino| & \nino \\
\verb|\ninoone| & \ninoone \\
\verb|\ninotwo| & \ninotwo \\
\verb|\ninothree| & \ninothree \\
\verb|\ninofour| & \ninofour \\
\verb|\gravino| & \gravino \\
\verb|\Zprime| & \Zprime \\
\verb|\Zstar| & \Zstar \\
\verb|\squark| & \squark \\
\verb|\squarkL| & \squarkL \\
\verb|\squarkR| & \squarkR \\
\verb|\gluino| & \gluino \\
\verb|\stop| & \stop \\
\verb|\stopone| & \stopone \\
\verb|\stoptwo| & \stoptwo \\
\verb|\stopL| & \stopL \\
\verb|\stopR| & \stopR \\
\verb|\sbottom| & \sbottom \\
\verb|\sbottomone| & \sbottomone \\
\verb|\sbottomtwo| & \sbottomtwo \\
\verb|\sbottomL| & \sbottomL \\
\verb|\sbottomR| & \sbottomR \\
\verb|\slepton| & \slepton \\
\verb|\sleptonL| & \sleptonL \\
\verb|\sleptonR| & \sleptonR \\
\verb|\sel| & \sel \\
\verb|\selL| & \selL \\
\verb|\selR| & \selR \\
\verb|\smu| & \smu \\
\verb|\smuL| & \smuL \\
\verb|\smuR| & \smuR \\
\verb|\stau| & \stau \\
\verb|\stauL| & \stauL \\
\verb|\stauR| & \stauR \\
\verb|\stauone| & \stauone \\
\verb|\stautwo| & \stautwo \\
\verb|\snu| & \snu \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasheavyion.tex <==
\begin{xtabular}{ll}
\verb|\NucNuc| & \NucNuc \\
\verb|\nn| & \nn \\
\verb|\pn| & \pn \\
\verb|\np| & \np \\
\verb|\PbPb| & \PbPb \\
\verb|\AuAu| & \AuAu \\
\verb|\CuCu| & \CuCu \\
\verb|\pNuc| & \pNuc \\
\verb|\pdA| & \pdA \\
\verb|\dAu| & \dAu \\
\verb|\pPb| & \pPb \\
\verb|\Npart| & \Npart \\
\verb|\avgNpart| & \avgNpart \\
\verb|\Ncoll| & \Ncoll \\
\verb|\avgNcoll| & \avgNcoll \\
\verb|\TA| & \TA \\
\verb|\avgTA| & \avgTA \\
\verb|\TPb| & \TPb \\
\verb|\avgTPb| & \avgTPb \\
\verb|\TAA| & \TAA \\
\verb|\avgTAA| & \avgTAA \\
\verb|\TAB| & \TAB \\
\verb|\avgTAB| & \avgTAB \\
\verb|\TpPb| & \TpPb \\
\verb|\avgTpPb| & \avgTpPb \\
\verb|\Gl| & \Gl \\
\verb|\GG| & \GG \\
\verb|\sqn| & \sqn \\
\verb|\lns| & \lns \\
\verb|\sumETPb| & \sumETPb \\
\verb|\sumETp| & \sumETp \\
\verb|\sumETA| & \sumETA \\
\verb|\RAA| & \RAA \\
\verb|\RCP| & \RCP \\
\verb|\RpA| & \RpA \\
\verb|\RpPb| & \RpPb \\
\verb|\dNchdeta| & \dNchdeta \\
\verb|\dNevtdET| & \dNevtdET \\
\verb|\ystar| & \ystar \\
\verb|\ycms| & \ycms \\
\verb|\ygappb| & \ygappb \\
\verb|\ygapp| & \ygapp \\
\verb|\fgap| & \fgap \\
\end{xtabular}


==> bib/doc/atlas_physics/atlashepparticle.tex <==
\begin{xtabular}{ll}
\verb|\pp| & \pp \\
\verb|\pbar| & \pbar \\
\verb|\ppbar| & \ppbar \\
\verb|\tbar| & \tbar \\
\verb|\ttbar| & \ttbar \\
\verb|\bbar| & \bbar \\
\verb|\bbbar| & \bbbar \\
\verb|\cbar| & \cbar \\
\verb|\ccbar| & \ccbar \\
\verb|\sbar| & \sbar \\
\verb|\ssbar| & \ssbar \\
\verb|\ubar| & \ubar \\
\verb|\uubar| & \uubar \\
\verb|\dbar| & \dbar \\
\verb|\ddbar| & \ddbar \\
\verb|\fbar| & \fbar \\
\verb|\ffbar| & \ffbar \\
\verb|\qbar| & \qbar \\
\verb|\qqbar| & \qqbar \\
\verb|\nbar| & \nbar \\
\verb|\nnbar| & \nnbar \\
\verb|\ee| & \ee \\
\verb|\epm| & \epm \\
\verb|\epem| & \epem \\
\verb|\mumu| & \mumu \\
\verb|\tautau| & \tautau \\
\verb|\leplep| & \leplep \\
\verb|\ellell| & \ellell \\
\verb|\enu| & \enu \\
\verb|\munu| & \munu \\
\verb|\lnu| & \lnu \\
\verb|\Zzero| & \Zzero \\
\verb|\Zboson| & \Zboson \\
\verb|\Wplus| & \Wplus \\
\verb|\Wminus| & \Wminus \\
\verb|\Wboson| & \Wboson \\
\verb|\Wpm| & \Wpm \\
\verb|\Wmp| & \Wmp \\
\verb|\taulep| & \taulep \\
\verb|\tauhad| & \tauhad \\
\verb|\tauhadvis| & \tauhadvis \\
\verb|\pizero| & \pizero \\
\verb|\piplus| & \piplus \\
\verb|\piminus| & \piminus \\
\verb|\pipm| & \pipm \\
\verb|\pimp| & \pimp \\
\verb|\etaprime| & \etaprime \\
\verb|\Kzero| & \Kzero \\
\verb|\Kzerobar| & \Kzerobar \\
\verb|\kaon| & \kaon \\
\verb|\Kplus| & \Kplus \\
\verb|\Kminus| & \Kminus \\
\verb|\KzeroL| & \KzeroL \\
\verb|\Kzerol| & \Kzerol \\
\verb|\Klong| & \Klong \\
\verb|\KzeroS| & \KzeroS \\
\verb|\Kzeros| & \Kzeros \\
\verb|\Kshort| & \Kshort \\
\verb|\Kstar| & \Kstar \\
\verb|\jpsi| & \jpsi \\
\verb|\Jpsi| & \Jpsi \\
\verb|\psip| & \psip \\
\verb|\chic| & \chic \\
\verb|\UoneS| & \UoneS \\
\verb|\chib| & \chib \\
\verb|\Dstar| & \Dstar \\
\verb|\Bd| & \Bd \\
\verb|\Bs| & \Bs \\
\verb|\Bu| & \Bu \\
\verb|\Bc| & \Bc \\
\verb|\Lb| & \Lb \\
\verb|\Bstar| & \Bstar \\
\verb|\BoBo| & \BoBo \\
\verb|\BodBod| & \BodBod \\
\verb|\BosBos| & \BosBos \\
\end{xtabular}


==> bib/doc/atlas_physics/atlashepprocess.tex <==
\begin{xtabular}{ll}
\verb|\btol| & \btol \\
\verb|\ctol| & \ctol \\
\verb|\btoctol| & \btoctol \\
\verb|\Jee| & \Jee \\
\verb|\Jmm| & \Jmm \\
\verb|\Jmumu| & \Jmumu \\
\verb|\Wjj| & \Wjj \\
\verb|\tjjb| & \tjjb \\
\verb|\Hbb| & \Hbb \\
\verb|\Hgg| & \Hgg \\
\verb|\Hll| & \Hll \\
\verb|\Hllll| & \Hllll \\
\verb|\Hmmmm| & \Hmmmm \\
\verb|\Heeee| & \Heeee \\
\verb|\Zll| & \Zll \\
\verb|\Zlplm| & \Zlplm \\
\verb|\Zee| & \Zee \\
\verb|\Zepem| & \Zepem \\
\verb|\Zmm| & \Zmm \\
\verb|\Zmpmm| & \Zmpmm \\
\verb|\Ztt| & \Ztt \\
\verb|\Ztptm| & \Ztptm \\
\verb|\Zbb| & \Zbb \\
\verb|\Wln| & \Wln \\
\verb|\Wen| & \Wen \\
\verb|\Wmn| & \Wmn \\
\verb|\Wlnu| & \Wlnu \\
\verb|\Wenu| & \Wenu \\
\verb|\Wmunu| & \Wmunu \\
\verb|\Wqqbar| & \Wqqbar \\
\verb|\Amm| & \Amm \\
\verb|\Ztautau| & \Ztautau \\
\verb|\Wtaunu| & \Wtaunu \\
\verb|\Atautau| & \Atautau \\
\verb|\Htautau| & \Htautau \\
\verb|\tWb| & \tWb \\
\verb|\Wjets| & \Wjets \\
\verb|\Zjets| & \Zjets \\
\verb|\Brjl| & \Brjl \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasjetetmiss.tex <==
\begin{xtabular}{ll}
\verb|\topo| & \topo \\
\verb|\Topo| & \Topo \\
\verb|\topos| & \topos \\
\verb|\Topos| & \Topos \\
\verb|\insitu| & \insitu \\
\verb|\Insitu| & \Insitu \\
\verb|\LS| & \LS \\
\verb|\NLOjet| & \NLOjet \\
\verb|\Fastjet| & \Fastjet \\
\verb|\TwoToTwo| & \TwoToTwo \\
\verb|\largeR| & \largeR \\
\verb|\LargeR| & \LargeR \\
\verb|\akt| & \akt \\
\verb|\Akt| & \Akt \\
\verb|\AKT| & \AKT \\
\verb|\AKTFat| & \AKTFat \\
\verb|\AKTPrune| & \AKTPrune \\
\verb|\AKTFilt| & \AKTFilt \\
\verb|\KTSix| & \KTSix \\
\verb|\ca| & \ca \\
\verb|\CamKt| & \CamKt \\
\verb|\CASix| & \CASix \\
\verb|\CAFat| & \CAFat \\
\verb|\CAPrune| & \CAPrune \\
\verb|\CAFilt| & \CAFilt \\
\verb|\htt| & \htt \\
\verb|\mcut| & \mcut \\
\verb|\Nfilt| & \Nfilt \\
\verb|\Rfilt| & \Rfilt \\
\verb|\ymin| & \ymin \\
\verb|\fcut| & \fcut \\
\verb|\Rsub| & \Rsub \\
\verb|\mufrac| & \mufrac \\
\verb|\Rcut| & \Rcut \\
\verb|\zcut| & \zcut \\
\verb|\ftile| & \ftile \\
\verb|\fem| & \fem \\
\verb|\fpres| & \fpres \\
\verb|\fhec| & \fhec \\
\verb|\ffcal| & \ffcal \\
\verb|\central| & \central \\
\verb|\ecap| & \ecap \\
\verb|\forward| & \forward \\
\verb|\Npv| & \Npv \\
\verb|\Nref| & \Nref \\
\verb|\Navg| & \Navg \\
\verb|\avgmu| & \avgmu \\
\verb|\JES| & \JES \\
\verb|\JMS| & \JMS \\
\verb|\EMJES| & \EMJES \\
\verb|\GCWJES| & \GCWJES \\
\verb|\LCWJES| & \LCWJES \\
\verb|\EM| & \EM \\
\verb|\GCW| & \GCW \\
\verb|\LCW| & \LCW \\
\verb|\GSL| & \GSL \\
\verb|\GS| & \GS \\
\verb|\MTF| & \MTF \\
\verb|\MPF| & \MPF \\
\verb|\Njet| & \Njet \\
\verb|\njet| & \njet \\
\verb|\ETjet| & \ETjet \\
\verb|\etjet| & \etjet \\
\verb|\pTavg| & \pTavg \\
\verb|\ptavg| & \ptavg \\
\verb|\pTjet| & \pTjet \\
\verb|\ptjet| & \ptjet \\
\verb|\pTcorr| & \pTcorr \\
\verb|\ptcorr| & \ptcorr \\
\verb|\pTjeti| & \pTjeti \\
\verb|\ptjeti| & \ptjeti \\
\verb|\pTrecoil| & \pTrecoil \\
\verb|\ptrecoil| & \ptrecoil \\
\verb|\pTleading| & \pTleading \\
\verb|\ptleading| & \ptleading \\
\verb|\pTjetEM| & \pTjetEM \\
\verb|\ptjetEM| & \ptjetEM \\
\verb|\pThat| & \pThat \\
\verb|\pthat| & \pthat \\
\verb|\pTprobe| & \pTprobe \\
\verb|\ptprobe| & \ptprobe \\
\verb|\pTref| & \pTref \\
\verb|\ptref| & \ptref \\
\verb|\pToff| & \pToff \\
\verb|\ptoff| & \ptoff \\
\verb|\pToffjet| & \pToffjet \\
\verb|\ptoffjet| & \ptoffjet \\
\verb|\pTZ| & \pTZ \\
\verb|\ptZ| & \ptZ \\
\verb|\pTtrue| & \pTtrue \\
\verb|\pttrue| & \pttrue \\
\verb|\pTtruth| & \pTtruth \\
\verb|\pttruth| & \pttruth \\
\verb|\pTreco| & \pTreco \\
\verb|\ptreco| & \ptreco \\
\verb|\pTtrk| & \pTtrk \\
\verb|\pttrk| & \pttrk \\
\verb|\ptrk| & \ptrk \\
\verb|\pTtrkjet| & \pTtrkjet \\
\verb|\pttrkjet| & \pttrkjet \\
\verb|\ntrk| & \ntrk \\
\verb|\EoverP| & \EoverP \\
\verb|\Etrue| & \Etrue \\
\verb|\Etruth| & \Etruth \\
\verb|\Ecalo| & \Ecalo \\
\verb|\EcaloEM| & \EcaloEM \\
\verb|\asym| & \asym \\
\verb|\Response| & \Response \\
\verb|\Rcalo| & \Rcalo \\
\verb|\Rcalom| & \Rcalom \\
\verb|\RcaloEM| & \RcaloEM \\
\verb|\RMPF| & \RMPF \\
\verb|\EcaloCALIB| & \EcaloCALIB \\
\verb|\RcaloCALIB| & \RcaloCALIB \\
\verb|\EcaloEMJES| & \EcaloEMJES \\
\verb|\RcaloEMJES| & \RcaloEMJES \\
\verb|\EcaloGCWJES| & \EcaloGCWJES \\
\verb|\RcaloGCWJES| & \RcaloGCWJES \\
\verb|\EcaloLCWJES| & \EcaloLCWJES \\
\verb|\RcaloLCWJES| & \RcaloLCWJES \\
\verb|\Rtrack| & \Rtrack \\
\verb|\rtrk| & \rtrk \\
\verb|\Rtrk| & \Rtrk \\
\verb|\rtrackjet| & \rtrackjet \\
\verb|\rtrackjetiso| & \rtrackjetiso \\
\verb|\rtrackjetnoniso| & \rtrackjetnoniso \\
\verb|\rtrackjetisoratio| & \rtrackjetisoratio \\
\verb|\gammajet| & \gammajet \\
\verb|\deltaphijetgamma| & \deltaphijetgamma \\
\verb|\rapjet| & \rapjet \\
\verb|\etajet| & \etajet \\
\verb|\phijet| & \phijet \\
\verb|\etadet| & \etadet \\
\verb|\etatrk| & \etatrk \\
\verb|\Rmin| & \Rmin \\
\verb|\DeltaR| & \DeltaR \\
\verb|\DetaDphi| & \DetaDphi \\
\verb|\Deta| & \Deta \\
\verb|\Drap| & \Drap \\
\verb|\DetaOneTwo| & \DetaOneTwo \\
\verb|\DyDphi| & \DyDphi \\
\verb|\DeltaRdef| & \DeltaRdef \\
\verb|\DeltaRydef| & \DeltaRydef \\
\verb|\DeltaRtrk| & \DeltaRtrk \\
\verb|\JVF| & \JVF \\
\verb|\cJVF| & \cJVF \\
\verb|\RpT| & \RpT \\
\verb|\JVT| & \JVT \\
\verb|\ghostpt| & \ghostpt \\
\verb|\ghostptavg| & \ghostptavg \\
\verb|\ghostfm| & \ghostfm \\
\verb|\ghostfmi| & \ghostfmi \\
\verb|\ghostdensity| & \ghostdensity \\
\verb|\ghostrho| & \ghostrho \\
\verb|\Aghost| & \Aghost \\
\verb|\Amu| & \Amu \\
\verb|\Amui| & \Amui \\
\verb|\jetarea| & \jetarea \\
\verb|\jetareafm| & \jetareafm \\
\verb|\jetareai| & \jetareai \\
\verb|\Rkt| & \Rkt \\
\verb|\pTmuslope| & \pTmuslope \\
\verb|\ptmuslope| & \ptmuslope \\
\verb|\pTnpvslope| & \pTnpvslope \\
\verb|\ptnpvslope| & \ptnpvslope \\
\verb|\pTmuunc| & \pTmuunc \\
\verb|\ptmuunc| & \ptmuunc \\
\verb|\pTnpvunc| & \pTnpvunc \\
\verb|\ptnpvunc| & \ptnpvunc \\
\verb|\sumPt| & \sumPt \\
\verb|\sumpt| & \sumpt \\
\verb|\sumpTtrk| & \sumpTtrk \\
\verb|\sumpttrk| & \sumpttrk \\
\verb|\nPUtrk| & \nPUtrk \\
\verb|\mjet| & \mjet \\
\verb|\mlead| & \mlead \\
\verb|\mleadavg| & \mleadavg \\
\verb|\Mjet| & \Mjet \\
\verb|\massjet| & \massjet \\
\verb|\masscorr| & \masscorr \\
\verb|\mthresh| & \mthresh \\
\verb|\mjetavg| & \mjetavg \\
\verb|\masstrkjet| & \masstrkjet \\
\verb|\width| & \width \\
\verb|\wcalo| & \wcalo \\
\verb|\wtrk| & \wtrk \\
\verb|\shapeV| & \shapeV \\
\verb|\pTsubjet| & \pTsubjet \\
\verb|\ptsubjet| & \ptsubjet \\
\verb|\sjone| & \sjone \\
\verb|\sjtwo| & \sjtwo \\
\verb|\msubjone| & \msubjone \\
\verb|\msubjtwo| & \msubjtwo \\
\verb|\pTsubji| & \pTsubji \\
\verb|\ptsubji| & \ptsubji \\
\verb|\pTsubjone| & \pTsubjone \\
\verb|\ptsubjone| & \ptsubjone \\
\verb|\pTsubjtwo| & \pTsubjtwo \\
\verb|\ptsubjtwo| & \ptsubjtwo \\
\verb|\Rsubjets| & \Rsubjets \\
\verb|\DRsubjets| & \DRsubjets \\
\verb|\yij| & \yij \\
\verb|\dcut| & \dcut \\
\verb|\dmin| & \dmin \\
\verb|\dij| & \dij \\
\verb|\Dij| & \Dij \\
\verb|\Donetwo| & \Donetwo \\
\verb|\Dtwothr| & \Dtwothr \\
\verb|\yonetwo| & \yonetwo \\
\verb|\ytwothr| & \ytwothr \\
\verb|\yonetwoDef| & \yonetwoDef \\
\verb|\ytwothrDef| & \ytwothrDef \\
\verb|\xj| & \xj \\
\verb|\jetFunc| & \jetFunc \\
\verb|\tauone| & \tauone \\
\verb|\tautwo| & \tautwo \\
\verb|\tauthr| & \tauthr \\
\verb|\tauN| & \tauN \\
\verb|\tautwoone| & \tautwoone \\
\verb|\tauthrtwo| & \tauthrtwo \\
\verb|\dip| & \dip \\
\verb|\diponetwo| & \diponetwo \\
\verb|\diptwothr| & \diptwothr \\
\verb|\diponethr| & \diponethr \\
\verb|\mtaSup| & \mtaSup \\
\verb|\mcalo| & \mcalo \\
\verb|\mcomb| & \mcomb \\
\verb|\ECFOne| & \ECFOne \\
\verb|\ECFTwo| & \ECFTwo \\
\verb|\ECFThr| & \ECFThr \\
\verb|\ECFThrNorm| & \ECFThrNorm \\
\verb|\DTwo| & \DTwo \\
\verb|\CTwo| & \CTwo \\
\verb|\FoxWolfRatio| & \FoxWolfRatio \\
\verb|\PlanarFlow| & \PlanarFlow \\
\verb|\Angularity| & \Angularity \\
\verb|\Aplanarity| & \Aplanarity \\
\verb|\KtDR| & \KtDR \\
\verb|\Qw| & \Qw \\
\verb|\NConst| & \NConst \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasjournal.tex <==
\begin{xtabular}{ll}
\verb|\AcPA| & \AcPA \\
\verb|\ARevNS| & \ARevNS \\
\verb|\CPC| & \CPC \\
\verb|\EPJ| & \EPJ \\
\verb|\EPJC| & \EPJC \\
\verb|\FortP| & \FortP \\
\verb|\IJMP| & \IJMP \\
\verb|\JETP| & \JETP \\
\verb|\JETPL| & \JETPL \\
\verb|\JaFi| & \JaFi \\
\verb|\JHEP| & \JHEP \\
\verb|\JMP| & \JMP \\
\verb|\MPL| & \MPL \\
\verb|\NCim| & \NCim \\
\verb|\NIM| & \NIM \\
\verb|\NIMA| & \NIMA \\
\verb|\NP| & \NP \\
\verb|\NPB| & \NPB \\
\verb|\PL| & \PL \\
\verb|\PLB| & \PLB \\
\verb|\PR| & \PR \\
\verb|\PRC| & \PRC \\
\verb|\PRD| & \PRD \\
\verb|\PRL| & \PRL \\
\verb|\PRep| & \PRep \\
\verb|\RMP| & \RMP \\
\verb|\ZfP| & \ZfP \\
\verb|\collab| & \collab \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasmath.tex <==
\begin{xtabular}{ll}
\verb|\boxsq| & \boxsq \\
\verb|\grad| & \grad \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasmisc.tex <==
\begin{xtabular}{ll}
\verb|\pT| & \pT \\
\verb|\pt| & \pt \\
\verb|\pTX| & \pTX \\
\verb|\ET| & \ET \\
\verb|\eT| & \eT \\
\verb|\et| & \et \\
\verb|\HT| & \HT \\
\verb|\pTsq| & \pTsq \\
\verb|\MET| & \MET \\
\verb|\met| & \met \\
\verb|\sumET| & \sumET \\
\verb|\EjetRec| & \EjetRec \\
\verb|\PjetRec| & \PjetRec \\
\verb|\EjetTru| & \EjetTru \\
\verb|\PjetTru| & \PjetTru \\
\verb|\EjetDM| & \EjetDM \\
\verb|\Rcone| & \Rcone \\
\verb|\abseta| & \abseta \\
\verb|\Ecm| & \Ecm \\
\verb|\rts| & \rts \\
\verb|\sqs| & \sqs \\
\verb|\Nevt| & \Nevt \\
\verb|\zvtx| & \zvtx \\
\verb|\dzero| & \dzero \\
\verb|\zzsth| & \zzsth \\
\verb|\RunOne| & \RunOne \\
\verb|\RunTwo| & \RunTwo \\
\verb|\RunThr| & \RunThr \\
\verb|\kt| & \kt \\
\verb|\antikt| & \antikt \\
\verb|\Antikt| & \Antikt \\
\verb|\pileup| & \pileup \\
\verb|\Pileup| & \Pileup \\
\verb|\btag| & \btag \\
\verb|\btagged| & \btagged \\
\verb|\bquark| & \bquark \\
\verb|\bquarks| & \bquarks \\
\verb|\bjet| & \bjet \\
\verb|\bjets| & \bjets \\
\verb|\mh| & \mh \\
\verb|\mW| & \mW \\
\verb|\mZ| & \mZ \\
\verb|\mH| & \mH \\
\verb|\ACERMC| & \ACERMC \\
\verb|\ALPGEN| & \ALPGEN \\
\verb|\AMCatNLO| & \AMCatNLO \\
\verb|\BLACKHAT| & \BLACKHAT \\
\verb|\CALCHEP| & \CALCHEP \\
\verb|\COLLIER| & \COLLIER \\
\verb|\COMPHEP| & \COMPHEP \\
\verb|\EVTGEN| & \EVTGEN \\
\verb|\FEYNRULES| & \FEYNRULES \\
\verb|\GGTOVV| & \GGTOVV \\
\verb|\GOSAM| & \GOSAM \\
\verb|\HATHOR| & \HATHOR \\
\verb|\Herwig| & \Herwig \\
\verb|\HERWIG| & \HERWIG \\
\verb|\HERWIGpp| & \HERWIGpp \\
\verb|\HRES| & \HRES \\
\verb|\JIMMY| & \JIMMY \\
\verb|\MADSPIN| & \MADSPIN \\
\verb|\MADGRAPH| & \MADGRAPH \\
\verb|\MGNLO| & \MGNLO \\
\verb|\MCatNLO| & \MCatNLO \\
\verb|\MCFM| & \MCFM \\
\verb|\METOP| & \METOP \\
\verb|\OPENLOOPS| & \OPENLOOPS \\
\verb|\POWHEG| & \POWHEG \\
\verb|\POWHEGBOX| & \POWHEGBOX \\
\verb|\POWHEGBOXRES| & \POWHEGBOXRES \\
\verb|\PHOTOS| & \PHOTOS \\
\verb|\PHOTOSpp| & \PHOTOSpp \\
\verb|\PROPHECY| & \PROPHECY \\
\verb|\PROTOS| & \PROTOS \\
\verb|\Pythia| & \Pythia \\
\verb|\PYTHIA| & \PYTHIA \\
\verb|\RECOLA| & \RECOLA \\
\verb|\Sherpa| & \Sherpa \\
\verb|\SHERPA| & \SHERPA \\
\verb|\TOPpp| & \TOPpp \\
\verb|\VBFNLO| & \VBFNLO \\
\verb|\MGNLOHER| & \MGNLOHER \\
\verb|\MGNLOPY| & \MGNLOPY \\
\verb|\MGHER| & \MGHER \\
\verb|\MGPY| & \MGPY \\
\verb|\POWHER| & \POWHER \\
\verb|\POWPY| & \POWPY \\
\verb|\SHERPABH| & \SHERPABH \\
\verb|\SHERPAOL| & \SHERPAOL \\
\verb|\ABM| & \ABM \\
\verb|\ABKM| & \ABKM \\
\verb|\CT| & \CT \\
\verb|\CTEQ| & \CTEQ \\
\verb|\GJR| & \GJR \\
\verb|\HERAPDF| & \HERAPDF \\
\verb|\LUXQED| & \LUXQED \\
\verb|\MSTW| & \MSTW \\
\verb|\MMHT| & \MMHT \\
\verb|\MSHT| & \MSHT \\
\verb|\NNPDF| & \NNPDF \\
\verb|\PDFforLHC| & \PDFforLHC \\
\verb|\AUET| & \AUET \\
\verb|\AZNLO| & \AZNLO \\
\verb|\FXFX| & \FXFX \\
\verb|\GEANT| & \GEANT \\
\verb|\MENLOPS| & \MENLOPS \\
\verb|\MEPSatLO| & \MEPSatLO \\
\verb|\MEPSatNLO| & \MEPSatNLO \\
\verb|\MINLO| & \MINLO \\
\verb|\Monash| & \Monash \\
\verb|\Perugia| & \Perugia \\
\verb|\Prospino| & \Prospino \\
\verb|\UEEE| & \UEEE \\
\verb|\LO| & \LO \\
\verb|\NLO| & \NLO \\
\verb|\NLL| & \NLL \\
\verb|\NNLO| & \NNLO \\
\verb|\muF| & \muF \\
\verb|\muQ| & \muQ \\
\verb|\muR| & \muR \\
\verb|\hdamp| & \hdamp \\
\verb|\NLOEWvirt| & \NLOEWvirt \\
\verb|\ra| & \ra \\
\verb|\la| & \la \\
\verb|\rarrow| & \rarrow \\
\verb|\larrow| & \larrow \\
\verb|\lapprox| & \lapprox \\
\verb|\rapprox| & \rapprox \\
\verb|\gam| & \gam \\
\verb|\stat| & \stat \\
\verb|\syst| & \syst \\
\verb|\radlength| & \radlength \\
\verb|\StoB| & \StoB \\
\verb|\alphas| & \alphas \\
\verb|\NF| & \NF \\
\verb|\NC| & \NC \\
\verb|\CF| & \CF \\
\verb|\CA| & \CA \\
\verb|\TF| & \TF \\
\verb|\Lms| & \Lms \\
\verb|\Lmsfive| & \Lmsfive \\
\verb|\kperp| & \kperp \\
\verb|\Vcb| & \Vcb \\
\verb|\Vub| & \Vub \\
\verb|\Vtd| & \Vtd \\
\verb|\Vts| & \Vts \\
\verb|\Vtb| & \Vtb \\
\verb|\Vcs| & \Vcs \\
\verb|\Vud| & \Vud \\
\verb|\Vus| & \Vus \\
\verb|\Vcd| & \Vcd \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasother.tex <==
\begin{xtabular}{ll}
\verb|\etpt| & \etpt \\
\verb|\etptsig| & \etptsig \\
\verb|\begL| & \begL \\
\verb|\lowL| & \lowL \\
\verb|\highL| & \highL \\
\verb|\Epsb| & \Epsb \\
\verb|\Epsc| & \Epsc \\
\verb|\Mtau| & \Mtau \\
\verb|\swsq| & \swsq \\
\verb|\swel| & \swel \\
\verb|\swsqb| & \swsqb \\
\verb|\swsqon| & \swsqon \\
\verb|\gv| & \gv \\
\verb|\ga| & \ga \\
\verb|\gvbar| & \gvbar \\
\verb|\gabar| & \gabar \\
\verb|\Zzv| & \Zzv \\
\verb|\Abb| & \Abb \\
\verb|\Acc| & \Acc \\
\verb|\Aqq| & \Aqq \\
\verb|\Afb| & \Afb \\
\verb|\GZ| & \GZ \\
\verb|\GW| & \GW \\
\verb|\GH| & \GH \\
\verb|\GamHad| & \GamHad \\
\verb|\Gbb| & \Gbb \\
\verb|\Rbb| & \Rbb \\
\verb|\Gcc| & \Gcc \\
\verb|\Gvis| & \Gvis \\
\verb|\Ginv| & \Ginv \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasparticle.tex <==
\begin{xtabular}{ll}
\verb|\pp| & \pp \\
\verb|\pbar| & \pbar \\
\verb|\ppbar| & \ppbar \\
\verb|\tbar| & \tbar \\
\verb|\ttbar| & \ttbar \\
\verb|\bbar| & \bbar \\
\verb|\bbbar| & \bbbar \\
\verb|\cbar| & \cbar \\
\verb|\ccbar| & \ccbar \\
\verb|\sbar| & \sbar \\
\verb|\ssbar| & \ssbar \\
\verb|\ubar| & \ubar \\
\verb|\uubar| & \uubar \\
\verb|\dbar| & \dbar \\
\verb|\ddbar| & \ddbar \\
\verb|\fbar| & \fbar \\
\verb|\ffbar| & \ffbar \\
\verb|\qbar| & \qbar \\
\verb|\qqbar| & \qqbar \\
\verb|\nbar| & \nbar \\
\verb|\nnbar| & \nnbar \\
\verb|\ee| & \ee \\
\verb|\epm| & \epm \\
\verb|\epem| & \epem \\
\verb|\mumu| & \mumu \\
\verb|\tautau| & \tautau \\
\verb|\leplep| & \leplep \\
\verb|\ellell| & \ellell \\
\verb|\enu| & \enu \\
\verb|\munu| & \munu \\
\verb|\lnu| & \lnu \\
\verb|\taulep| & \taulep \\
\verb|\tauhad| & \tauhad \\
\verb|\tauhadvis| & \tauhadvis \\
\verb|\Zzero| & \Zzero \\
\verb|\Zboson| & \Zboson \\
\verb|\Wplus| & \Wplus \\
\verb|\Wminus| & \Wminus \\
\verb|\Wboson| & \Wboson \\
\verb|\Wpm| & \Wpm \\
\verb|\Wmp| & \Wmp \\
\verb|\pizero| & \pizero \\
\verb|\piplus| & \piplus \\
\verb|\piminus| & \piminus \\
\verb|\pipm| & \pipm \\
\verb|\pimp| & \pimp \\
\verb|\etaprime| & \etaprime \\
\verb|\Kzero| & \Kzero \\
\verb|\Kzerobar| & \Kzerobar \\
\verb|\kaon| & \kaon \\
\verb|\Kplus| & \Kplus \\
\verb|\Kminus| & \Kminus \\
\verb|\KzeroL| & \KzeroL \\
\verb|\Kzerol| & \Kzerol \\
\verb|\Klong| & \Klong \\
\verb|\KzeroS| & \KzeroS \\
\verb|\Kzeros| & \Kzeros \\
\verb|\Kshort| & \Kshort \\
\verb|\Kstar| & \Kstar \\
\verb|\jpsi| & \jpsi \\
\verb|\Jpsi| & \Jpsi \\
\verb|\psip| & \psip \\
\verb|\chic| & \chic \\
\verb|\UoneS| & \UoneS \\
\verb|\chib| & \chib \\
\verb|\Dstar| & \Dstar \\
\verb|\Bd| & \Bd \\
\verb|\Bs| & \Bs \\
\verb|\Bu| & \Bu \\
\verb|\Bc| & \Bc \\
\verb|\Lb| & \Lb \\
\verb|\Bstar| & \Bstar \\
\verb|\BoBo| & \BoBo \\
\verb|\BodBod| & \BodBod \\
\verb|\BosBos| & \BosBos \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasprocess.tex <==
\begin{xtabular}{ll}
\verb|\btol| & \btol \\
\verb|\ctol| & \ctol \\
\verb|\btoctol| & \btoctol \\
\verb|\Jee| & \Jee \\
\verb|\Jmm| & \Jmm \\
\verb|\Jmumu| & \Jmumu \\
\verb|\Wjj| & \Wjj \\
\verb|\tjjb| & \tjjb \\
\verb|\Hbb| & \Hbb \\
\verb|\Hgg| & \Hgg \\
\verb|\Hll| & \Hll \\
\verb|\Hllll| & \Hllll \\
\verb|\Hmmmm| & \Hmmmm \\
\verb|\Heeee| & \Heeee \\
\verb|\Zll| & \Zll \\
\verb|\Zlplm| & \Zlplm \\
\verb|\Zee| & \Zee \\
\verb|\Zepem| & \Zepem \\
\verb|\Zmm| & \Zmm \\
\verb|\Zmpmm| & \Zmpmm \\
\verb|\Ztt| & \Ztt \\
\verb|\Ztptm| & \Ztptm \\
\verb|\Zbb| & \Zbb \\
\verb|\Wln| & \Wln \\
\verb|\Wen| & \Wen \\
\verb|\Wmn| & \Wmn \\
\verb|\Wlnu| & \Wlnu \\
\verb|\Wenu| & \Wenu \\
\verb|\Wmunu| & \Wmunu \\
\verb|\Wqqbar| & \Wqqbar \\
\verb|\Amm| & \Amm \\
\verb|\Ztautau| & \Ztautau \\
\verb|\Wtaunu| & \Wtaunu \\
\verb|\Atautau| & \Atautau \\
\verb|\Htautau| & \Htautau \\
\verb|\tWb| & \tWb \\
\verb|\Wjets| & \Wjets \\
\verb|\Zjets| & \Zjets \\
\verb|\Brjl| & \Brjl \\
\end{xtabular}


==> bib/doc/atlas_physics/atlassnippets.tex <==
\begin{xtabular}{lp{10cm}}
\verb|\AntiktSnippet| & \AntiktSnippet \\
\verb|\TopoclusteringSnippet| & \TopoclusteringSnippet \\
\verb|\GroomingSnippet| & \GroomingSnippet \\
\verb|\FastSimSnippet| & \FastSimSnippet \\
\verb|\PileupSnippet| & \PileupSnippet \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasunit.tex <==
\begin{xtabular}{ll}
\verb|\electronvolt| & \electronvolt \\
\verb|\TeV| & \TeV \\
\verb|\GeV| & \GeV \\
\verb|\MeV| & \MeV \\
\verb|\keV| & \keV \\
\verb|\eV| & \eV \\
\verb|\TeVc| & \TeVc \\
\verb|\GeVc| & \GeVc \\
\verb|\MeVc| & \MeVc \\
\verb|\keVc| & \keVc \\
\verb|\eVc| & \eVc \\
\verb|\TeVcc| & \TeVcc \\
\verb|\GeVcc| & \GeVcc \\
\verb|\MeVcc| & \MeVcc \\
\verb|\keVcc| & \keVcc \\
\verb|\eVcc| & \eVcc \\
\verb|\ifb| & \ifb \\
\verb|\ipb| & \ipb \\
\verb|\inb| & \inb \\
\verb|\degr| & \degr \\
\end{xtabular}


==> bib/doc/atlas_physics/atlasxref.tex <==
\begin{xtabular}{ll}
\end{xtabular}


==> bib/doc/atlas_tables/Makefile <==
#------------------------------------------------------------------------------
# Makefile to make atlas_tables documentation
#------------------------------------------------------------------------------

BASENAME = atlas_tables
TEXLIVE = 2020

.PHONY: clean cleanpdf

atlas_tables:
	make -f ../Makefile run_latexmk BASENAME=$(BASENAME); \

texlive:
	make -f ../Makefile texlive BASENAME=$(BASENAME) TEXLIVE=$(TEXLIVE)

clean:
	make -f ../Makefile clean
	
cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf
	

==> bib/doc/atlas_tables/cross-sections_charm-ET1.tex <==
% Charm differential cross sections d sigma / dY in bins of ET
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\begin{tabular}{%
    S[table-format=2.0, table-number-alignment=right,
    round-mode=places, round-precision=0]@{$\,:\,$}
    S[table-format=2.0, table-number-alignment=left,
    round-mode=places, round-precision=0]
    S[table-format=4.2, table-number-alignment=right,
    round-mode=figures, round-precision=3]@{$\,\pm\,$}
    S[table-format=3.2, table-number-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}l}
  \toprule
  \multicolumn{2}{c}{\ET} &
  \multicolumn{3}{c}{$\dif\sigma / \dif\ET$}\\
  \multicolumn{2}{c}{\mbox{}} & \multicolumn{3}{c}{[\si{\pico\barn\per\GeV}]}\\
  \midrule
 4.2 & 8.0  & 3634.06 & 114.491  & \numpmerr{+201.404 }{-181.511}{2}  \\
 8.0 & 11.0 & 719.458 & 21.9334  & \numpmerr{+43.3087 }{-39.7824}{2}  \\
11.0 & 14.0 & 214.572 & 9.71991  & \numpmerr{+20.5413 }{-19.6464}{2}  \\
14.0 & 17.0 & 85.7584 & 6.03401  & \numpmerr{+10.0875 }{-8.99952}{2}  \\
17.0 & 20.0 & 35.4095 & 3.91591  & \numpmerr{+5.5349  }{-5.41347}{2}  \\
20.0 & 25.0 & 14.1253 & 2.72552  & \numpmerr{+3.46528 }{-3.22476}{2}  \\
25.0 & 35.0 & 2.37786 & 0.968562 & \numpmerr{+0.849647}{-0.855525}{2} \\
  \bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-ET2.tex <==
% Charm differential cross sections d sigma / dY in bins of ET
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\begin{tabular}{%
    S[table-format=2.0, table-number-alignment=right,
    round-mode=places, round-precision=0]@{$\,:\,$}
    S[table-format=2.0, table-number-alignment=left,
    round-mode=places, round-precision=0]
    S[table-format=4.1, table-alignment=right,
    round-mode=figures, round-precision=3]@{$\,\pm\,$}
    S[table-format=3.1, table-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}r}
  \toprule
  \multicolumn{2}{c}{\ET} &
  \multicolumn{3}{c}{$\dif\sigma / \dif\ET$}\\
  \multicolumn{2}{c}{[\si{\GeV}]} & \multicolumn{3}{c}{[\si{\pico\barn\per\GeV}]}\\
  \midrule
 4.2 & 8.0  & 3634.06                    & 114.491                    & \numpmRF{+201.404 }{-181.511 }{2}  \\
 8.0 & 11.0 & 719.458                    & 21.9334                    & \numpmerr{+43.3087 }{-39.7824 }{0} \\
11.0 & 14.0 & {\numRF{214.572}{2}\phdo}  & {\numRF{9.71991}{1}\phdo}  & \numpmerr{+20.5413 }{-19.6464 }{0} \\
14.0 & 17.0 & {\numRF{85.7584}{2}\phdo}  & {\numRF{6.03401}{1}\phdo}  & \numpmerr{+10.0875 }{-8.99952 }{0} \\
17.0 & 20.0 & {\numRF{35.4095}{3}}       & {\numRF{3.91591}{2}}       & \numpmerr{+5.5349  }{-5.41347 }{1} \\
20.0 & 25.0 & 14.1253                    & 2.72552                    & \numpmerr{+3.46528 }{-3.22476 }{1} \\
25.0 & 35.0 & {\numRF{2.37786}{2}}       & {\numRF{0.968562}{1}}      & \numpmerr{+0.849647}{-0.855525}{1}  \\
  \bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-eta1.tex <==
\renewcommand{\arraystretch}{1.4}
\sisetup{round-mode = places}
\centering
\begin{tabular}{%
S@{\,:\,}S
r@{\,}@{$\pm$}@{\,}l@{\,}l
}
\toprule
\multicolumn{2}{c}{\etajet} & \multicolumn{3}{c}{\diffetab} \\
\multicolumn{2}{c}{} & \multicolumn{3}{c}{[\si{\pico\barn}]} \\
\midrule
{\num{-1.6}} & -1.1 & \numRP{0.574}{3} & \num[round-precision=3]{0.094} &
$^{\numRP{+0.035}{3}}_{\numRP{-0.031}{3}}$ \\
{\num{-1.1}} & -0.8 & \numRP{1.213}{2} & \num[round-precision=2]{0.211} &
$^{\numRP{+0.162}{2}}_{\numRP{-0.162}{2}}$ \\
{\num{-0.8}} & -0.5 & \numRP{2.141}{2} & \num[round-precision=2]{0.219} &
$^{\numRP{+0.223}{2}}_{\numRP{-0.123}{2}}$ \\
{\num{-0.5}} & -0.2 & \numRP{2.326}{2} & \num[round-precision=2]{0.210} &
$^{\numRP{+0.284}{2}}_{\numRP{-0.214}{2}}$ \\
{\num{-0.2}} & +0.1 & \numRP{2.641}{2} & \num[round-precision=2]{0.220} &
$^{\numRP{+0.283}{2}}_{\numRP{-0.233}{2}}$ \\
{\num{+0.1}} & +0.5 & \numRP{3.160}{2} & \num[round-precision=2]{0.211} &
$^{\numRP{+0.232}{2}}_{\numRP{-0.172}{2}}$ \\
{\num{+0.5}} & +1.4 & \numRP{2.881}{2} & \num[round-precision=2]{0.154} &
$^{\numRP{+0.201}{2}}_{\numRP{-0.301}{2}}$ \\
\bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-eta2.tex <==
\renewcommand{\arraystretch}{1.4}
\sisetup{round-mode = places, round-precision = 2}
\centering
\begin{tabular}{%
    S[table-format=3.2, table-number-alignment = right]@{\,:\,}S
    S[round-mode = places, round-precision = 2,
    table-format = 1.3, table-number-alignment = right]
    @{\(\,\pm\,\)}
    S[round-mode = places, round-precision = 2,
    table-format = 1.3, table-number-alignment = left]
    @{\,}l
    }
\toprule
\multicolumn{2}{c}{\etajet} & \multicolumn{3}{c}{\diffetab} \\
\multicolumn{2}{c}{} & \multicolumn{3}{c}{[\si{\pico\barn}]} \\
\midrule
-1.6 & -1.1 & {\numRP{0.574}{3}} & {\numRP{0.094}{3}} & \(^{\numRP{+0.035}{3}}_{\numRP{-0.031}{3}}\) \\
-1.1 & -0.8 & 1.213 & 0.211 & \(^{\num{+0.162}}_{\num{-0.162}}\) \\
-0.8 & -0.5 & 2.141 & 0.219 & \(^{\num{+0.223}}_{\num{-0.123}}\) \\
-0.5 & -0.2 & 2.326 & 0.210 & \(^{\num{+0.284}}_{\num{-0.214}}\) \\
-0.2 & +0.1 & 2.641 & 0.220 & \(^{\num{+0.283}}_{\num{-0.233}}\) \\
+0.1 & +0.5 & 3.160 & 0.211 & \(^{\num{+0.232}}_{\num{-0.172}}\) \\
+0.5 & +1.4 & 2.881 & 0.154 & \(^{\num{+0.201}}_{\num{-0.301}}\) \\
\bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-x1.tex <==
% Charm differential cross sections d sigma / dY in bins of xda
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\sisetup{scientific-notation=fixed, fixed-exponent=0}
\begin{tabular}{%
    S[table-format=1.5, table-number-alignment=right,
    round-mode=figures, round-precision=1]@{$\,:\,$}
    S[table-format=1.5, table-number-alignment=left,
    round-mode=figures, round-precision=1]
    S[table-format=8.0, table-number-alignment=right,
    round-mode=figures, round-precision=3]@{$\,\pm\,$}
    S[table-format=6.0, table-number-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}r}
  \toprule
  \multicolumn{2}{c}{$x$} &
  \multicolumn{3}{c}{$\dif\sigma / \dif x$}\\
  \multicolumn{2}{c}{\mbox{}} & \multicolumn{3}{c}{[\si{\pico\barn}]}\\
  \midrule
0.00008 & 0.00020 & 1.08474e+07 & 867945  & \numpmerr{+761437 }{-647690 }{2}  \\
0.00020 & 0.00060 & 1.08385e+07 & 388976  & \numpmerr{+567443 }{-441257 }{2}  \\
0.00060 & 0.00160 & 4.974e+06   & 135404  & \numpmerr{+256385 }{-233376 }{2}  \\
0.00160 & 0.00500 & 1.21664e+06 & 31162.1 & \numpmerr{+68948.1}{-62459.6}{2} \\
0.00500 & 0.01000 & 256870      & 12232.7 & \numpmerr{+18363.7}{-16463.7}{2} \\
0.01000 & 0.10000 & 10652.6     &  791.21 & \numpmerr{+913.118}{-815.675}{2} \\
  \bottomrule
\end{tabular}


==> bib/doc/atlas_tables/cross-sections_charm-x2.tex <==
% Charm differential cross sections d sigma / dY in bins of xda
\sisetup{round-mode=figures, round-precision=2,
  group-digits=integer, group-minimum-digits=4}
\sisetup{scientific-notation=fixed, fixed-exponent=0}
\begin{tabular}{%
    S[table-format=1.5, table-number-alignment=right,
    round-mode=figures, round-precision=1]@{$\,:\,$}
    S[table-format=1.5, table-number-alignment=left,
    round-mode=figures, round-precision=1]
    S[table-format=5.1, table-alignment=right,
    round-mode=figures, round-precision=4]@{$\,\pm\,$}
    S[table-format=3.1, table-alignment=right,
    round-mode=figures, round-precision=2]@{$\,$}r}
  \toprule
  \multicolumn{2}{c}{$x$} &
  \multicolumn{3}{c}{$\dif\sigma / \dif x$}\\
  \multicolumn{2}{c}{\mbox{}} & \multicolumn{3}{c}{[\si{\nano\barn}]}\\
  \midrule
0.00008 & 0.00020                 & {\numRF{1.08474e+04}{2}\phdo}  & {\numRF{867945e-3}{1}\phdo}  & \numpmerr{+761437 e-3}{-647690 e-3}{1} \\
0.00020 & 0.00060                 & {\numRF{1.08385e+04}{3}\phdo}  & {\numRF{388976e-3}{1}\phdo}  & \numpmerr{+567443 e-3}{-441257 e-3}{1} \\
0.00060 & {\numRF{0.0016}{2}\pho} & {\numRF{4.974e+03}{3}\phdo}    & 135404e-3                    & \numpmerr{+256385 e-3}{-233376 e-3}{2} \\
{\numRF{0.0016}{2}\pho} & 0.00500 & {\numRF{1.21664e+03}{4}\phdo}  & 31162.1e-3                   & \numpmerr{+68948.1e-3}{-62459.6e-3}{2} \\
0.00500 & 0.01000                 & {\numRF{256870e-03}{3}\phdo}   & 12232.7e-3                   & \numpmerr{+18363.7e-3}{-16463.7e-3}{2} \\
0.01000 & 0.10000                 & {\numRF{10652.6e-03}{3}}       & {\numRF{791.21e-3}{1}}       & \numpmerr{+913.118e-3}{-815.675e-3}{1} \\
  \bottomrule
\end{tabular}


==> foreword/foreword.tex <==
LUXE is going to explore quantum physics in a novel way! What could be more exciting for a physicist? It is rare that we have the opportunity to test fundamental physics in a completely new regime. Julian Schwinger showed in 1951 that at field strengths of $E=m_{e}^{2}/q_{e} \sim 1.32 \times 10^{18}$\,V/m (now known as the Schwinger field) the QED vacuum becomes unstable and decays into electron-positron pairs. Already earlier this effect was proposed by Sauter and Heisenberg and Euler also discussed it but the technology to create such strong fields was not available. 

With the recent advances in laser technology and the high energy electron beam of the European XFEL, LUXE can finally go directly into this regime and measure this effect in detail as a function of the strength of the field. The mission of LUXE is to observe the behaviour of QED in the strong-field regime, and then to also measure it in both Compton scattering and in electron-positron pair production with high precision. LUXE started in 2017 with a coffee meeting of three people, and by now consists of a collaboration of about 100 particle, accelerator and laser physicists. 

A huge thanks goes to all those who have contributed directly to this document, but also to those who gave advice and to the people and agencies who supported the project and its teams. I am excited in seeing LUXE now become a reality at DESY and the European XFEL in Hamburg, and look forward to its breakthrough observations and measurements!

Beate Heinemann\\
LUXE Spokesperson
 


==> journal/Makefile <==
# Makefile for creating an ATLAS paper draft using journal classes

TEXLIVE  = 2020
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
DVIPS    = dvips
DVIPDF   = dvipdf
OPEN     = open

TEXFILES = $(wildcard *.tex)

.PHONY: texlive clean

all: atlas-elsevier atlas-jhep atlas-jinst atlas-revtex

texlive:
	for file in $(TEXFILES); do \
	  if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	    echo "Changing texlive value in $$file"; \
	    sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $$file; \
	  else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \
	done

atlas-elsevier: atlas-elsevier.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jhep: atlas-jhep.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-jinst: atlas-jinst.pdf
	@echo "Made $<"
	# $(OPEN) $<

atlas-revtex: atlas-revtex.pdf
	@echo "Made $<"
	# $(OPEN) $<

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $< and $(basename $<).pdf"

# Standard LaTeX targets
%.pdf: %.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.dvi: $(BASENAME).tex
	$(LATEX)    $<
	$(LATEX)    $<

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf \
	 *.fdb_latexmk *.spl *-revtexNotes.bib *.run.xml *.synctex.gz *~

cleanall: clean
	-rm *.pdf


==> journal/atlas-document-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%% Title
\AtlasTitle{A simple ATLAS paper draft}
%
% Author - this does not work with revtex
% \author{The ATLAS Collaboration}
%
% Date: if not given, uses current date
% \date{\today}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
\AtlasVersion{1.0}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2020-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
% \AtlasNote{ATLAS-CONF-2020-XXX}
% \AtlasNote{ATLAS-PUB-2020-XXX}
\AtlasNote{ATLAS-COM-PHYS-2020-XXX}

% Submission journal
\AtlasJournal{Phys.\ Lett.\ B.}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
	This is a bare bones ATLAS document used to demonstrate how to use journal templates.

	This document is typeset using the \DocumentStyle.
}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% Explicit list of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
\AtlasCoverSupportingNote{A supporting note}{http://cds.cern.ch/record/XXXXXX}
\AtlasCoverSupportingNote{Another supporting note}{http://cds.cern.ch/record/YYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{DD Month 2020}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
\AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-GROUP-2020-XX-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-GROUP-2020-XX-editorial-board@cern.ch}

% CERN preprintnumber
\PreprintIdNumber{CERN-EP-2020-XX}


==> luxetdr-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

%https://indico.cern.ch/event/1439855/page/35202-guidelines

% Title
\AtlasTitle{The LUXE Experiment}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of every other page, 
% and line numbers.
% Comment or remove in the final version.
%\AtlasVersion{0.3}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
  This  Technical Design Report presents a detailed description of all aspects of the LUXE (Laser Und XFEL Experiment),  an experiment that will combine the high-quality and high-energy electron beam of the European XFEL with a high-intensity laser, to explore the uncharted terrain of strong-field quantum electrodynamics characterised by both high energy and high
intensity, reaching the Schwinger field and beyond. The further implications for the search of physics beyond the Standard Model are also discussed.

}

% Author - this does not work with revtex (add it after \begin{document})
% This has to be commented out for TDR etc.
% For PUB notes, add package authblk and use \thanks if an ACE/STA should be added.
% See Section 4.2 of ATLAS LaTeX guide for more details.
% \author{The ATLAS Collaboration}

% ATLAS reference code, to help ATLAS members to locate the paper
%\AtlasRefCode{GROUP-2021-XX}

% CERN preprint number
% \PreprintIdNumber{CERN-EP-2021-XX}

% ATLAS date - arXiv submission; usually filled in by the Physics Office
\AtlasDate{31st March 2025}

% ATLAS heading - heading at top of title page. Set for TDR etc.
% \AtlasHeading{ATLAS ABC TDR}

% arXiv identifier
% \arXivId{21XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
% \AtlasJournal{Phys.\ Lett.\ B.}
% \AtlasJournalRef{\PLB 789 (2021) 123}
% \AtlasDOI{}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
% \AtlasCoverSupportingNote{Short title note 1}{https://cds.cern.ch/record/XXXXXXX}
% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
% \AtlasCoverCommentsDeadline{DD Month 2021}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
% \AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverReaderMember{Reader~2}

% Editors egroup
% \AtlasCoverEgroupEditors{atlas-GROUP-2021-XX-editors@cern.ch}

% EdBoard egroup
% \AtlasCoverEgroupEdBoard{atlas-GROUP-2021-XX-editorial-board@cern.ch}


==> template/EXOT/btagging_selection.tex <==
\subsection{Jet flavor tagging selection}

\begin{table}[ht]
  \caption{\btag selection criteria.}%
  \label{tab:object:btag}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & Criterion \\ 
    \midrule
    & EM Topo Jets / Track jets / VR jets \\
    \midrule
    Jet collection  & \texttt{AntiKt4EMTopo/AntiKt2PV0/AntiKtVR30Rmax4Rmin02} \\
    Jet selection   & \(\pT > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    	            	& \(|\eta| < X\) \\				
                    & JVT cut if applicable \\
    \midrule
    Algorithm 		  & \texttt{MV2c10/MV2c10mu/MV2c10rnn/DL1/DL1mu/DL1rnn} \\
    \midrule
    Operating point & Hybrid /  Fixed \\
                    & Eff = 60 / 70 / 77 / 85 \\
    CDI             & \texttt{2017-21-13TeV-MC16-CDI-2017-12-22\_v1} \\
  \bottomrule
  \end{tabular}
  % }
\end{table}%


==> template/EXOT/egamma_selection.tex <==
\subsection{Electron selection}

\begin{table}[ht]
  \caption{Electron selection criteria.}%
  \label{tab:object:electron}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & \multicolumn{1}{c}{Criterion} \\
    \midrule
    Pseudorapidity range & \(|\eta| <\) X\\
    Energy calibration & \texttt{es2017\_R21\_PRE} (ESModel)\\
    Energy & \(E > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    Transverse energy & \(\ET > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    Transverse momentum & \(\pT > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \midrule
    \multirow{2}{*}{Object quality} & Not from a bad calorimeter cluster (\texttt{BADCLUSELECTRON})\\ %\cline{2-2}
      & Remove clusters from regions with EMEC bad HV (2016 data only) \\
    \midrule
    \multirow{2}{*}{Track to vertex association} & \(|d_{0}^{\text{BL}}(\sigma)| < X\) \\ %\cline{2-2}
    & \(|\Delta z_{0}^{\text{BL}} \sin{\theta}| < \SI[parse-numbers=false]{X}{\mm}\) \\
    \midrule
    Identification & (\texttt{Loose/Medium/Tight}) \\
    Isolation & \texttt{LooseTrackOnly / Loose / Tight / Gradient / \ldots} \\
      \bottomrule
  \end{tabular}
  % }
\end{table}

Notes:
\begin{itemize}
\item Pseudorapidity: when the calorimeter crack is not excluded, the range can be indicated simply as \enquote{\(|\eta| < 2.47\)}, when the crack is excluded: \enquote{\((|\eta| < 1.37) \quad || \quad (1.52 < |\eta| < 2.47)\)}.
\item Usually only one among \enquote{Energy}, \enquote{Transverse energy} and \enquote{Transverse momentum} criteria is applied --- the \SI{30}{\GeV} value is just an example.
  In special cases energy (i.e.\ calorimeter-based measurement) and momentum (i.e.\ tracking-based measurement) criteria can be required in order to constraint different aspects of the reconstruction.
\item Electron ID\@: 3 working points (Loose/Medium/Tight) are evaluated using the Likelihood-based (LH) method, by the
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaIdentificationRun2}{ElectronPhotonSelectorTools}.
\item Energy calibration of electrons is implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/ElectronPhotonFourMomentumCorrection}{ElectronPhotonFourMomentumCorrection} tool.
\item Scale Factors for efficiencies for electrons are implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/XAODElectronEfficiencyCorrectionTool}{ElectronEfficiencyCorrection} tool.
\item Updated configurations for the EGamma CP tools can be found on this \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaRecommendationsR21}{TWiki} page.
\end{itemize}

\newpage

\subsection{Photon selection}

\begin{table}[ht]
  \caption{Photon selection criteria.}%
  \label{tab:object:photon} 
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & \multicolumn{1}{c}{Criterion} \\
    \midrule
    Pseudorapidity range & \(|\eta| <\) X\\
    Energy calibration & \texttt{es2017\_R21\_PRE} (ESModel)\\
    Energy & \(E > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    Transverse energy & \(\ET > \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \midrule
    \multirow{2}{*}{Object quality} & Not from a bad calorimeter cluster (\texttt{BADCLUSELECTRON})\\ %\cline{2-2}
      & Remove clusters from regions with EMEC bad HV (2016 data only) \\
    \midrule
    Photon cleaning & \texttt{passOQquality} \\
    Fudging & Applied for Full sim / not for AtlFastII \\
    \midrule
    Identification & (\texttt{Loose/Tight}) \\
    Isolation &  \texttt{FixedCutTightCaloOnly / FixedCutTight / FixedCutLoose} \\
    \bottomrule
  \end{tabular}
  %  }
\end{table}

Notes:
\begin{itemize}
\item Pseudorapidity: please note that the maximum value for \(|\eta|\) for photon candidates (2.37) is smaller than for electron candidates (2.47). 
  If crack excluded: \enquote{\((|\eta| < 1.37) \quad || \quad (1.52 < |\eta| < 2.37)\)}.
\item Usually only one between \enquote{Energy} and \enquote{Transverse energy} criteria is applied --- the \SI{30}{\GeV} value is just an example.
\item Photon cleaning: a new Photon helper is available to apply the photon cleaning cut 
  (from the \texttt{ElectronPhotonSelectorTools}, tag \(\ge\) 00-02-92-21, release \(\ge\) 2.4.30).
\item Photon ID\@: 2 working points (Loose/Tight) are evaluated using a cut-based method, by the
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaIdentificationRun2}{ElectronPhotonSelectorTools}.
\item Energy calibration of photons is implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/ElectronPhotonFourMomentumCorrection}{ElectronPhotonFourMomentumCorrection} tool.
\item Scale Factors for efficiencies for photons are implemented in the\\
  \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/XAODElectronEfficiencyCorrectionTool}{ElectronEfficiencyCorrection} tool.
\item Updated configurations for the EGamma CP tools can be found on this \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/EGammaRecommendationsR21}{TWiki} page.
\end{itemize}


==> template/EXOT/event_cleaning.tex <==
\subsection{Event cleaning}
Following the \href{https://twiki.cern.ch/twiki/bin/viewauth/Atlas/DataPreparationCheckListForPhysicsAnalysis}{recommendations of the DataPrep group}, the following event-level requirements are made.

We use the official GRL\@:
 \begin{verbatim} FILL IN HERE \end{verbatim}
 
The following event-level vetos are made to reject bad / corrupt events:
 \begin{itemize}
  \item LAr noise burst and data corruption (\verb|xAOD::EventInfo::LAr|),
  \item Tile corrupted events (\verb|xAOD::EventInfo::Tile|),
  \item events affected by the SCT recovery procedure for single event upsets (\verb|xAOD::EventInfo::SCT|),
  \item incomplete events (\verb|xAOD::EventInfo::Core|).
 \end{itemize}
 
 Debug stream events [have/have not] been included.
 
 Checks [have/have not] been done to remove duplicate events.
 
Events are required to have a primary vertex with at least two associated tracks.
The primary vertex is selected as the one with the largest \(\Sigma \pT^2\),
where the sum is over all tracks with transverse momentum \(\pT > \SI{0.4}{\GeV}\) that are associated with the vertex.
 
 

==> template/EXOT/executive_summary.tex <==
\subsection{Target} 

\(\mathcal{O}\)(1 paragraph)
Is this a new analysis? If not, what are the main improvements expected with respect to the previous version?
What is the target publication date / conference?

\subsection{Context and Motivation} 

Motivate this analysis in 1 paragraph: why is this signature interesting? Which kind of models are you probing?

How is the analysis done is 1 paragraph: what are the main BG processes and how do you estimate them (are they MC- or data-driven,
what is the general idea of the control regions, \ldots), general characteristics of the PL fit (which distribution, binned?, \ldots)

\subsection{Milestones}

 Table giving a factual list of who is working on what and what else they do; the idea is to show how the team can / does progress. 
 Including dates for completion of these milestones will help further demonstrate that you are ready for the collaboration
 review, in the form of an editorial board.

%Example : 
The following table summarizes the tasks to be worked on by analysis team.
This is not a complete analysis outline but only an overview of the further steps to be taken as of the time of writing.
Details are not provided here but in the dedicated sections throughout this note.
Tasks which are based on established techniques and straightforward to achieve are marked green in the table.
Tasks which require new work are marked red.
Concerning the involved people, the responsible student supervisors and analysis coordinators are already mentioned in the list of contributions above,
which shall not be repeated here.
A fair overview of all single tasks including past work and of all relevant team members is only given in the list of contributions above!
It is also worth noting that some of the tasks listed below are being worked on in parallel. 

\begin{table}[ht]
  \caption{Milestones in the analysis.}%
  \label{tab:Miles_Ahead} 
  % \resizebox{\textwidth}{!}{
\begin{tabular}{llll} 
  \toprule
  \textbf{Task} & \textbf{Analyzer} & \textbf{Role} & \textbf{Other responsibilities} \\
  \midrule
  \multicolumn{4}{p{\textwidth}}{\textbf{Describe a first milestone.}} \\
  \midrule
  \textcolor{green}{A straightforward task}       & Name         & PhD student, PostDoc/Prof/\ldots & thesis writing \\
  &&& / teaching \\
  &&& / name some CP work \ldots \\ 
  \textcolor{red}{A more involved task}      &    &    &  \\ 
  \bottomrule
  
  \multicolumn{4}{l}{\textbf{Describe a second milestone}} \\
  \midrule
  First task \ldots      &          &  &  \\ 
  \bottomrule
\end{tabular}
%}
\end{table}




==> template/EXOT/jet_selection.tex <==
\subsection{Small-$R$ jet selection}

If you want to use variables such as \verb|\fcut| you need to add the option
\texttt{jetetmiss} to \texttt{atlaspackage}.

\begin{table}[ht]
  \caption{Jet reconstruction criteria.}%
  \label{tab:object:jet1}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
  \toprule
  Feature & Criterion \\
  \midrule
  Algorithm & \Antikt  \\
  \(R\)-parameter & 0.4 \\
  Input constituent & EMTopo \\
  Analysis release number & 21.2.10 \\
  %Calibration tag & JetCalibTools-00-04-76 \\
  \texttt{CalibArea} tag & 00-04-81 \\
  Calibration configuration & \texttt{JES\_data2017\_2016\_2015\_Recommendation\_Feb2018\_rel21.config} \\
  Calibration sequence (Data) & \texttt{JetArea\_Residual\_EtaJES\_GSC\_Insitu} \\
  Calibration sequence (MC) & \texttt{JetArea\_Residual\_EtaJES\_GSC} \\
  %Calibration sequence (AFII) & \texttt{JetArea\_Residual\_EtaJES\_GSC} \\
  \midrule
  \multicolumn{2}{c}{Selection requirements} \\
  \midrule
  Observable & Requirement \\
  \midrule
  Jet cleaning & \texttt{LooseBad} \\
  BatMan cleaning & No \\
  \pT & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
  \(|\eta|\) & \(< X\) \\
  JVT & (\emph{Update if needed}) \(>0.59\) for \(\pT < \SI{60}{\GeV}\), \(|\eta| < 0.4\)\\
  \bottomrule
  \end{tabular}
  % }
\end{table}


\clearpage
\subsection{Large-$R$ jet selection}

\begin{table}[ht]
  \caption{Large-\(R\) jet reconstruction criteria.}%
  \label{tab:object:jet2}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Feature & Criterion \\ 
    \midrule
    Algorithm & \antikt  \\
    R-parameter & 1.0 \\
    Input constituent & \texttt{LCTopo} \\
    Grooming algorithm & Trimming \\ 
    \fcut & 0.05 \\
    \(R_{\text{trim}}\) & 0.2 \\
    Analysis release number & 21.2.10 \\
    %Calibration tag & JetCalibTools-00-04-76 \\
    \texttt{CalibArea} tag & 00-04-81 \\
    Calibration configuration & \texttt{JES\_MC16recommendation\_FatJet\_JMS\_comb\_19Jan2018.config} \\
    Calibration sequence (Data) & \texttt{EtaJES\_JMS\_Insitu} \\
    Calibration sequence (MC) & \texttt{EtaJES\_JMS} \\
    \bottomrule
    \multicolumn{2}{c}{Selection requirements} \\
    \midrule
    Observable & Requirement \\
    \midrule
    \pT  & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \(|\eta|\) & \(< X\) \\
    Mass & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \bottomrule
    \multicolumn{2}{c}{Boosted object tagger} \\
    \midrule
    Object  & Working point \\
    \midrule
    \(W\) / \(Z\) / top & 50\% / 80\% \\
    \(X\rightarrow bb\) & single/double \btag with/without loose/tight mass \\
    \bottomrule
  \end{tabular}
  % }
\end{table}


\subsection{\MET selection}

\begin{table}[ht]
  \caption{\MET reconstruction criteria.}%
  \label{tab:object:met}
  \centering
  \begin{tabular}{ll}
    \toprule
    Parameter & Value \\ 
    \midrule
    Algorithm & Calo-based \\
    Soft term & Track-based (TST) \\ 
    MET operating point & \texttt{Tight} \\
    Analysis release & 21.2.16 \\
    Calibration tag & \texttt{METUtilities-00-02-46} \\
    \bottomrule
    \multicolumn{2}{c}{Selection requirements} \\
    \midrule
    Observable & Requirement \\
    \midrule
    \MET & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \(\sum{\ET} / \MET\)  & \(< X\) \\
    Object-based \MET significance & \(> X\) \\
    \bottomrule
  \end{tabular}
\end{table}




==> template/EXOT/muon_selection.tex <==
\subsection{Muon selection}

\begin{table}[ht]
  \caption{Muon selection criteria.}%
  \label{tab:object:muon}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}[ht]{ll}
    \toprule
    Feature & Criterion \\
    \midrule
    Selection working point & \texttt{Loose/Medium/Tight /High-pT} \\
    Isolation working point & \texttt{LooseTrackOnly/Loose/Tight/Gradient/\ldots}\\
    Momentum calibration & Sagitta correction [used/not used] \\
    \pT Cut & \SI[parse-numbers=false]{X}{\GeV} \\
    \(|\eta|\) cut & \(< X\) \\
    \dzero significance cut & X \\
    \(z_{0}\) cut & \SI[parse-numbers=false]{X}{\mm} \\
    \bottomrule
  \end{tabular}
  % }
\end{table}

The selection criteria are implemented in the \texttt{MuonSelectorTools-XX-XX-XX}\\
with \texttt{MuonMomentumCorrections-XX-XX-XX}, 
isolation in \texttt{IsolationSelection-XX-XX-XX} and \dzero and \(z_{0}\) cuts in \texttt{xAODTracking-XX-XX-XX}.
The muon recommendations can be found in 
\href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/MCPAnalysisGuidelinesMC16}{MCPAnalysisGuidelinesMC16}.


==> template/EXOT/overlap_removal.tex <==
\subsection{Overlap removal}

The reconstruction of the same energy deposits as multiple objects is resolved using the standard overlap removal tools, \texttt{AssociationUtils}, documented \href{https://gitlab.cern.ch/atlas/athena/blob/21.2/PhysicsAnalysis/AnalysisCommon/AssociationUtils/README.rst}{here}

The (Standard/Heavy-flavor/Boosted/Boosted+Heavy-flavor/lepton-favored) working point is used corresponding to:

\begin{table}[ht]
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{lll}
    \toprule
    Reject & Against & Criteria \\
    \midrule
    Electron & Electron & shared track, \(\pTX[][1] < \pTX[][2]\) \\
    Tau      & Electron & \(\Delta R <\) 0.2 \\
    Tau      & Muon     & \(\Delta R <\) 0.2 \\
    Muon     & Electron & is Calo-Muon and shared ID track \\
    Electron & Muon     & shared ID track \\
    Photon   & Electron & \(\Delta R < 0.4\) \\
    Photon   & Muon     & \(\Delta R < 0.4\) \\
    Jet      & Electron & [\(\Delta R < 0.2\) / Not a \bjet and \(\Delta R <\) 0.2] \\
    Electron & Jet      & [\(\Delta R < 0.4\) / \(\Delta R < \min(0.4, 0.04 + \SI{10}{\GeV}/\pT(e))\)/None] \\
    Jet      & Muon     & [\(\texttt{NumTrack} < 3\) and (ghost-associated or \(\Delta R < 0.2\)) / \\
                       && not a \bjet and \(\texttt{NumTrack} < 3\) and (ghost-associated or \(\Delta R < 0.2\))] \\
    Muon     & Jet      & [\(\Delta R < 0.4\) / \(\Delta R < \min(0.4, 0.04 + \SI{10}{\GeV}/\pT(\mu))\)/None] \\
    Jet      & Tau      & \(\Delta R < 0.2\) \\
    Photon   & Jet      & \(\Delta R < 0.4\) \\
    Fat-jet  & Electron & \(\Delta R < 1.0\) \\
    Jet      & Fat-jet  & \(\Delta R < 1.0\) \\
    \bottomrule
  \end{tabular}
  % }
\end{table}

\(\Delta R\) is calculated using rapidity by default.




==> template/EXOT/systematics.tex <==
Systematic uncertainties arise from the reconstruction of the various physics objects and 
from theoretical and/or modelling uncertainties affecting the predictions for both the backgrounds and signals. 
These uncertainties manifest themselves as uncertainties both in the overall yield and 
shape of the final observable.

\subsection{Experimental}

A summary of the experimental systematic uncertainties taken into account in this analysis is given in
Table~\ref{tab:syst_summary_sources}, along with the shorthand name of the uncertainty used throughout 
the analysis. 

\textit{Include also subsections for each of the individual descriptions of the uncertainty groups and the
source where they come from.  If the recommendation is not available at this time, state that in the section.}

\begin{table}[h]
	\centering
	\scriptsize
	\begin{center}
		\begin{tabular}{ll}
			\toprule \midrule
			Systematic uncertainty        & Short description                                                                          \\ \midrule
			\multicolumn{2}{c}{\textbf{Event}}  \\ \midrule
			Luminosity  & uncertainty on the total integrated luminosity  \\ \midrule
			\multicolumn{2}{c}{\textbf{Electrons}}  \\ \midrule
			EL\_EFF\_Trigger\_TOTAL\_1NPCOR\_PLUS\_UNCOR   & trigger efficiency uncertainty    \\
			EL\_EFF\_Reco\_TOTAL\_1NPCOR\_PLUS\_UNCOR    & reconstruction efficiency uncertainty          \\ 
			EL\_EFF\_ID\_TOTAL\_1NPCOR\_PLUS\_UNCOR    & ID efficiency uncertainty               \\ 
			EL\_EFF\_Iso\_TOTAL\_1NPCOR\_PLUS\_UNCOR    & isolation efficiency uncertainty       \\
			EG\_SCALE\_ALL & energy scale uncertainty  \\ 
			EG\_RESOLUTION\_ALL & energy resolution uncertainty  \\ \midrule
			\multicolumn{2}{c}{\textbf{Muons}}  \\ \midrule
			mu20\_iloose\_L1MU15\_OR\_HLT\_mu40\_MUON\_EFF\_Trig   & \multirow{ 2}{*}{trigger efficiency uncertainties (2 muon selection)}       \\ 
			mu24\_ivarmed\_OR\_HLT\_mu40\_MU\_EFF\_TrigStat        &         \\ 
			mu24\_ivarmed\_OR\_HLT\_mu50\_MU\_EFF\_TrigStat        &         \\ 
			mu26\_ivarmed\_OR\_HLT\_mu50\_MU\_EFF\_TrigStat        &         \\ 
			MUON\_EFF\_RECO\_STAT        & \multirow{ 2}{*}{reconstruction uncertainty for \pt > 15 GeV}        \\ % todo: guess that includes the ID uncertainty? PR.
			MUON\_EFF\_RECO\_SYS        &        \\ 
			MUON\_EFF\_RECO\_STAT\_LOWPT        & \multirow{ 2}{*}{reconstruction and ID efficiency uncertainty for \pt < 15 GeV}        \\ 
			MUON\_EFF\_RECO\_SYS \_LOWPT       &        \\ 
			MUON\_ISO\_STAT        & \multirow{ 2}{*}{isolation efficiency uncertainty}        \\ 
			MUON\_ISO\_SYS        &        \\ 
			MUON\_TTVA\_STAT        & \multirow{ 2}{*}{track-to-vertex association efficiency uncertainty}        \\ 
			MUON\_TTVA\_SYS        &        \\ 
			MUONS\_SCALE        & energy scale uncertainty                                                           \\ 
			MUONS\_SAGITTA\_RHO        & variations in the scale of the momentum (charge dependent)                  \\ 
			MUONS\_SAGITTA\_RESBIAS        & variations in the scale of the momentum (charge dependent)              \\ 
			MUONS\_ID        & energy resolution uncertainty from inner detector                              \\ 
			MUONS\_MS & energy resolution uncertainty from muon system  \\ \midrule
			\multicolumn{2}{c}{\textbf{Small-R Jets}}  \\ \midrule
			JET\_GroupedNP  & energy scale uncertainty split into 3 components              \\ 
			JET\_SR1\_JET\_EtaIntercalibration\_NonClosure & non-closure in the jet response at $2.4<|\eta|<2.5$   \\
			JET\_SR1\_JER\_SINGLE\_NP  & energy resolution uncertainty  \\
			JvtEfficiency & JVT efficiency uncertainty  \\
			%
			%
			% todo: decide on b-tagging EV prescription. So far we only have the simplest prescription, but we should switch.
			%
			%
			FT\_EFF\_EIGEN\_B & $b$-tagging efficiency uncertainties ("BTAG\_MEDIUM):   \\
			FT\_EFF\_EIGEN\_C & \\ % \multirow{2}{*}{3 components for $b$-jets, 4 for $c$-jets and 5 for light jets} \\
			FT\_EFF\_EIGEN\_L &   \\ 
			FT\_EFF\_EIGEN\_extrapolation &  $b$-tagging efficiency uncertainty on the extrapolation on high \pt-jets  \\ 
			FT\_EFF\_EIGEN\_extrapolation\_from\_charm & $b$-tagging efficiency uncertainty on $\tau$-jets   \\ \midrule
			\multicolumn{2}{c}{\textbf{Large-R Jets}}  \\ \midrule
			%
			%
			%
			FATJET\_JMR   & mass resolution uncertainty                                                                 \\ 
			FATJET\_JER    & energy resolution uncertainty                                                               \\ 
			JET\_Comb\_Baseline\_Kin &  \multirow{4}{*}{energy scale uncertainties (\pt and mass scales fully correlated)}  \\
			JET\_Comb\_Modelling\_Kin &  \\
			JET\_Comb\_TotalStat\_Kin &  \\
			JET\_Comb\_Tracking\_Kin   &  \\ 
			\midrule % TODO: which uncertainties do we need for large-R jets?
			% calo mass 
			%JET\_Medium\_JET\_Rtrk\_Baseline\_Kin &  \multirow{4}{*}{energy scale uncertainties (\pt and mass scales fully correlated)}  \\
			%JET\_Medium\_JET\_Rtrk\_Modelling\_Kin &  \\
			%JET\_Medium\_JET\_Rtrk\_TotalStat\_Kin &  \\
			%JET\_Medium\_JET\_Rtrk\_Tracking\_Kin   &  \\ \midrule
			%
			%
			% todo: decide on b-tagging EV prescription also for track jets. So far we only have the simplest prescription, but we should switch.
			%
			%
			\multicolumn{2}{c}{\textbf{Track-Jets}}  \\ \midrule
			FT\_EFF\_EIGEN\_B & $b$-tagging efficiency uncertainties ("BTAG\_MEDIUM):   \\
			FT\_EFF\_EIGEN\_C & \\ % \multirow{2}{*}{3 components for $b$-jets, 4 for $c$-jets and 5 for light jets} \\
			FT\_EFF\_EIGEN\_L &   \\ 
			FT\_EFF\_EIGEN\_extrapolation &  $b$-tagging efficiency uncertainty on the extrapolation on high \pt-jets  \\ 
			FT\_EFF\_EIGEN\_extrapolation\_from\_charm & $b$-tagging efficiency uncertainty on $\tau$-jets   \\ \midrule
			\multicolumn{2}{c}{\textbf{\MET-Trigger and \MET-Terms}}  \\ \midrule
			METTrigStat    & \multirow{2}{*}{trigger efficiency uncertainty} -  \\
			METTrigSyst &    \\
			MET\_SoftTrk\_ResoPerp           & track-based soft term related to transversal resolution uncertainty                  \\ 
			MET\_SoftTrk\_ResoPara           & track-based soft term related to longitudinal resolution uncertainty                  \\ 
			MET\_SoftTrk\_Scale                  & track-based soft term related to longitudinal scale uncertainty                          \\ 
			MET\_JetTrk\_Scale                   & track MET scale uncertainty due to tracks in jets                                            \\ \midrule
			PRW\_DATASF         & uncertainty on data SF used for the computation of pileup reweighting      \\
			
			\bottomrule
		\end{tabular}
	\end{center}
	\caption{ Qualitative summary of the experimental systematic uncertainties considered in this analysis.}
	\label{tab:syst_summary_sources}
\end{table}


\subsection{Theory/Modelling}

\textit{Modelling uncertainties can be analysis specific in the case of the background.  However, you should 
have a clear idea for your analysis how you will estimate these uncertainties.  If you are doing 
an MC-based background estimation, describe the sources of these uncertainties and the comparisons that
you will make.  If you are doing a data driven estimation, describe the sources.}

\textit{For signal yield uncertainties, these uncertainties are evaluated in a standard way and should 
include PDF variations and renormalization/factorization scale variations.  There is more information
provided on the PMG TWiki pages for this.}


\clearpage


==> template/EXOT/tau_selection.tex <==
\subsection{Tau selection}

\begin{table}[ht]
  \caption{Tau selection criteria.}%
  \label{tab:object:tau}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
  \toprule
  Feature & Criterion \\
  \midrule
  Pseudorapidity range & \(|\eta| < X\) \\
  Track selection & 1 or 3 tracks \\\
  Charge & \(|Q| = 1\) \\
  Tau energy scale & \texttt{MVA TES}\\
  Transverse momentum & \(\pT > \SI[parse-numbers=false]{XX}{\GeV}\) \\
  Jet rejection & BDT-based (\texttt{Loose/Medium/Tight}) \\
  Electron rejection & BDT-based\\
  Muon rejection & Via overlap removal in \(\Delta R < 0.2\) and \(\pT > \SI{2}{\GeV}\).
    Muons must not be Calo-tagged\\
  \bottomrule
  \end{tabular}
  % }
\end{table}

If the crack is excluded: \((|\eta| < 1.37) || (1.52 < |\eta| < 2.5)\)

The selection criteria are all implemented in the \texttt{TauSelectionTool} as part of the \texttt{TauAnalysisTools}.
Documentation can be found in the \href{https://gitlab.cern.ch/atlas/athena/blob/21.2/PhysicsAnalysis/TauID/TauAnalysisTools/doc/README-TauSelectionTool.rst}{README-TauSelectionTool.rst}.


==> template/EXOT/tracks_selection.tex <==
\subsection{Track selection}

If you use tracks as particular objects on which you cut in your analysis.

\begin{table}[ht]
  \caption{\texttt{TrackParticle} object selection criteria.}%
  \label{tab:object:track}
  \centering
  % \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
    \toprule
    Tracking algorithm								    & Primary / Large Radius Tracking / Custom \\
    Track quality selection (official)    & \texttt{Loose/Tight} \\
    \pT                                   & \(> \SI[parse-numbers=false]{XX}{\GeV}\) \\
    \(|\eta|\)                            & \(< X\) \\
    Track-vertex association criteria     & \texttt{Loose/Tight} \\
    Track-to-tet association method       & Ghost Matched / \(\Delta R\) \\
    \bottomrule
  \end{tabular}
  % }
\end{table}


==> template/MC_snippets/BJ.tex <==
% !TEX root = MC_snippets.tex

\chapter{Single-boson processes}
%\label{sec:VJ}

In the following paragraphs, the set-up of the current ATLAS single-boson baseline samples is described.
Details of the full process configuration are given in the PUB note~\cite{ATL-PHYS-PUB-2017-006}. In the case of \SHERPA samples,
a minimal description of built-in systematic uncertainties is also given.

%In addition, \SHERPA[2.1.1] is still used for cross checks and in the evaluation of theoretical uncertainties.
%Samples using this version have been generated with the \CT[10nlo] set of PDFs~\cite{Lai:2010vv}, in conjunction
%with the dedicated set of tuned parton-shower parameters developed by the \SHERPA authors for this generator version.

\section[Sherpa MEPS@NLO]{\SHERPA (\MEPSatNLO)}
%\label{sec:vjets-sherpa}

\subsection{QCD \(V+\)jets}
%\label{sec:vjets-sherpa-vjets}

\subsection*{Samples}
%\label{sec:vjets-sherpa-samples}

The descriptions below correspond to the samples in \cref{tab:vjets-sherpa}.

\begin{table}[!htbp]
  \caption{\(V\)+jets samples with \SHERPA.}%
  \label{tab:vjets-sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364100--364113    & \(Z\to\mu\mu\)   \\
    364198--364203    & \(Z\to \mu\mu\) (\(\SI{10}{\GeV} < m_{\ell\ell} < \SI{40}{\GeV}\)) \\
    364359, 364362, 364281  &  \(Z\to\mu\mu\) (very low mass)   \\
    364114--364127    & \(Z\to ee\)    \\
    364204--364209    & \(Z\to ee\) (\(\SI{10}{\GeV} < m_{\ell\ell} < \SI{40}{\GeV}\)) \\
    364358, 364361, 364282 & \(Z\to ee\) (very low mass) \\
    364128--364141    & \(Z\to \tau\tau\)    \\
    364210--364215    & \(Z\to \tau\tau\) (\(\SI{10}{\GeV} < m_{\ell\ell} < \SI{40}{\GeV}\)) \\
    364282, 364360, 364363 &  \(Z\to \tau\tau\) \\
    364142--364155    & \(Z\to \nu\nu\)   \\
    364156--364169    & \(W\to \mu\nu\)   \\
    364170--364183    & \(W\to e\nu\)    \\
    364184--364197    & \(W\to \tau\nu\)  \\
    364216--364229    & \(Z\to\ell\ell,W\to\ell\nu\) (high \pT)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \(V+\)jets was simulated with the
\SHERPA[2.2.1]~\cite{Bothmann:2019yzt}
generator using next-to-leading-order (NLO) matrix elements (ME) for up to two partons, and leading-order (LO) matrix elements
for up to four partons calculated with the Comix~\cite{Gleisberg:2008fv}
and \OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They
were matched with the \SHERPA parton shower~\cite{Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
using the set of tuned parameters developed by the \SHERPA authors.
The \NNPDF[3.0nnlo] set of PDFs~\cite{Ball:2014uwa} was used and the samples
were normalised to a next-to-next-to-leading-order (NNLO)
prediction~\cite{Anastasiou:2003ds}.


\paragraph{Long description:}

The production of \(V+\)jets was simulated with the \SHERPA[2.2.1]~\cite{Bothmann:2019yzt}
generator. In this set-up, NLO-accurate matrix elements for up to two partons, and LO-accurate matrix elements for up
to four partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries.
The default \SHERPA parton shower~\cite{Schumann:2007mg} based on
Catani--Seymour dipole factorisation and the cluster hadronisation model~\cite{Winter:2003tt}
were used. They employed the dedicated set of tuned parameters developed by the
\SHERPA authors and the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}.

The NLO matrix elements for a given jet multiplicity were matched to the parton
shower (PS) using a colour-exact variant of the MC@NLO
algorithm~\cite{Hoeche:2011fd}. Different jet multiplicities were then merged
into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}. The merging threshold
was set to \SI{20}{\GeV}.

\input{sherpa_scale_pdf.tex}

The \(V\)+jets samples were normalised to a next-to-next-to-leading-order (NNLO)
prediction~\cite{Anastasiou:2003ds}.


\subsection{Electroweak \(Vjj\) (VBF)}
%\label{sec:vjets-sherpa-vjj}

The descriptions below correspond to the samples in
\cref{tab:ewkvjets-sherpa}.  Samples include the VBF and \(V\)-strahlung diagrams, but
they do not include semileptonic \(VV\) diagrams and do not overlap with QCD \(V+\)jets samples.

\begin{table}[!htbp]
  \caption{Electroweak \(Vjj\) samples with \SHERPA.}%
  \label{tab:ewkvjets-sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    308092--308096 & EWK \(Vjj\) \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Electroweak production of \(\ell\ell jj\), \(\ell\nu jj\) and \(\nu\nu jj\) final states
was simulated with \SHERPA[2.2.1]~\cite{Bothmann:2019yzt} using
leading-order (LO) matrix elements with up to two additional parton emissions.
The matrix elements were merged with the \SHERPA parton
shower~\cite{Schumann:2007mg} following the \MEPSatLO
prescription~\cite{Catani:2001cc} and using the set of tuned
parameters developed by the \SHERPA authors.  The \NNPDF[3.0nnlo] set of
PDFs~\cite{Ball:2014uwa} was employed. The samples were produced
using the VBF approximation, which avoids overlap  with semileptonic
diboson topologies by requiring a \(t\)-channel colour-singlet exchange.

%These samples are generated in the \(G_\mu\) scheme using, ensuring an
%optimal description of pure electroweak interactions at the
%electroweak scale.


\section[MadGraph5 (CKKW-L)]{\MADGRAPH (CKKW-L)}
%\label{sec:vjets-mg5py8_ckkwl}

\subsection*{Samples}
%\label{sec:vjets-mg5py8_ckkwl-samples}

The descriptions below correspond to the samples in
\cref{tab:vjets-mg5py8_ckkwl}. The set-ups of \(N_\text{parton}\)- and
\HT-sliced samples differ slightly between the two slicing schemes
with regard to the matrix element PDF, the jet-clustering radius parameter
and the scale used in the evaluation of  \alphas to determine the weight of
each splitting. The short description merges the two set-ups and requires
the paper editors to select the appropriate PDF set (or gracefully describe
both); the long description is left unmerged.

\begin{table}[!htbp]
  \caption{\(V\)+jets samples with \MGPY[8] using CKKW-L merging.}%
  \label{tab:vjets-mg5py8_ckkwl}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    363123--363146 & \HT-sliced \(Z\to\mu\mu\)   \\
    363147--363170 & \HT-sliced \(Z\to ee\)     \\
    361510--361514 & \(N_\text{parton}\)-sliced \(Z\to\tau\tau\) \\
    361515--361519 & \(N_\text{parton}\)-sliced \(Z\to\nu\nu\)   \\
    363624--363647 & \HT-sliced \(W\to \mu\nu\)   \\
    363600--363623 & \HT-sliced \(W\to e\nu\)    \\
    363648--363671 & \HT-sliced \(W\to\tau\nu\)  \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description for \HT-sliced and \(N_\text{parton}\)-sliced \(V\)+jets:}

QCD \(V\)+jets production was simulated with \MGNLO[2.2.2]~\cite{Alwall:2014hca},
using LO-accurate matrix elements (ME) with up to four final-state partons.
The ME calculation employed the \NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa}
(\HT-sliced) / \NNPDF[2.3lo] set of PDFs~\cite{Ball:2012cx} (\(N_\text{parton}\)-sliced).
Events were interfaced to \PYTHIA[8.186]~\cite{Sjostrand:2007gs} for the modelling
of the parton shower, hadronisation, and  underlying event. The overlap between
matrix element and parton shower emissions was removed using the CKKW-L
merging procedure~\cite{Lonnblad:2001iq,Lonnblad:2011xx}. The A14
tune~\cite{ATL-PHYS-PUB-2014-021} of \PYTHIA[8] was used with the
\NNPDF[2.3lo] PDF set~\cite{Ball:2012cx}.
The decays of bottom and charm
hadrons were performed by \EVTGEN[1.2.0]~\cite{Lange:2001uf}.
The \(V\)+jets samples were normalised to a next-to-next-to-leading-order (NNLO)
prediction~\cite{Anastasiou:2003ds}.


\paragraph{\HT-sliced long description:}

QCD \(V\)+jets production was simulated with LO-accurate matrix elements (ME)
for up to four partons with \MGNLO[2.2.2]~\cite{Alwall:2014hca}. The ME calculation was interfaced with
\PYTHIA[8.186]~\cite{Sjostrand:2007gs} for the modelling of the parton
shower, hadronisation, and underlying event. To remove overlap between the matrix
element and the parton shower the CKKW-L merging
procedure~\cite{Lonnblad:2001iq,Lonnblad:2011xx} was applied with a
merging scale of \SI{30}{\GeV} and a jet-clustering radius parameter of
\(0.2\). In order to better model the region of large jet \pT, the
strong coupling constant \alphas was evaluated at the scale of each splitting to
determine the weight. The matrix element calculation was performed with
the \NNPDF[3.0nlo] PDF set~\cite{Ball:2014uwa} with \(\alphas= 0.118\). The calculation was done
in the five-flavour number scheme with massless \(b\)- and
\(c\)-quarks. Quark masses were reinstated in the \PYTHIA[8] parton shower.
The renormalisation and factorisation scales were set to the \MADGRAPH default
values, based on a clustering of the event. The A14
tune~\cite{ATL-PHYS-PUB-2014-021} of \PYTHIA[8] was used with the
\NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} with \(\alphas=0.13\).
The decays of bottom and charm hadrons were performed by \EVTGEN[1.2.0]~\cite{Lange:2001uf}.


\paragraph{\(N_\text{parton}\)-sliced long description:}

QCD \(V\)+jets production was simulated with LO-accurate matrix elements (ME) for up to four partons with
\MGNLO[2.2.2]~\cite{Alwall:2014hca}. The ME calculation was interfaced
with \PYTHIA[8.186]~\cite{Sjostrand:2007gs} for the modelling of the parton
shower and underlying event. To remove overlap between the matrix
element and the parton shower the CKKW-L merging
procedure~\cite{Lonnblad:2001iq,Lonnblad:2011xx} was applied with a
merging scale of \SI{30}{\GeV} and a jet-clustering radius parameter of
\(0.4\). In order to better model the region of large jet \pT, the
strong coupling constant \alphas was evaluated at the scale of each splitting to
determine the weight. The matrix element calculation was performed with
the \NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} with \(\alphas= 0.13\). The calculation was done
in the five-flavour number scheme with massless \(b\)- and
\(c\)-quarks. Quark masses were reinstated in the \PYTHIA[8] parton shower.
The renormalisation and factorisation scales were set to the \MADGRAPH default
values, based on a clustering of the event. The A14 tune~\cite{ATL-PHYS-PUB-2014-021}
of \PYTHIA[8] was used with the \NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} with \(\alphas=0.13\).
The decays of bottom and charm hadrons were performed by \EVTGEN[1.2.0]~\cite{Lange:2001uf}.

% No usable aMC@NLO \FXFX samples exist in ATLAS central production, therefore
% the description is commented out to avoid confusion

%% \section{\MGNLO (\FXFX)}
%% \label{sec:vjets-mg5-fxfx}

%% \begin{table}[!htbp]
%% \caption{Samples with \MGNLOPYTHIA[8] using CKKW-L merging.}%
%% \label{tab:mg5-fxfx}
%% \centering
%% \begin{tabular}{l l}
%% \toprule
%% DSID range & Description \\
%% \midrule
%% 999999-888888 & V+jets HT-sliced\\
%% \bottomrule
%% \end{tabular}
%% \end{center}
%% \end{table}

%% Samples have also been generated using the \MGNLO program to
%% generate matrix elements for \(V\) + 0, 1 and 2 partons at NLO accuracy.
%% The showering and subsequent hadronisation has been performed using \PYTHIA[8.210] with the A14 tune, using the \NNPDF[2.3lo]
%% PDF set with \(\alphas = 0.13\).
%% The different jet multiplicities are merged using the
%% \FXFX prescription~\cite{Frederix:2012ps} implemented in the \MGNLO program
%% (version 2.3.3 is used here).

%% \MGNLO performs a 5FNS calculation with massless \(b\)- and \(c\)-quarks in the matrix element, and massive quarks in the
%% \PYTHIA shower.
%% The PDF input set in use for event generation is \NNPDF[2.3nlo] PDF set with \(\alphas = 0.119\)
%% and the samples have been generated with additional weights for the PDF replicas as well as scale variations of
%% the renormalisation and the factorisation scales~\cite{Frederix:2011ss}.

%% The impact of various merging scales (\muQ) has been studied,
%% analysing three different values: \SI{20}{\GeV} (down variation), \SI{25}{\GeV} (nominal value) and \SI{50}{\GeV} (up variation).
%% At the event-generation level, the minimum jet transverse momentum, \(\pT^j\) is required to be at least
%% \SI{8}{\GeV} with no restriction on the absolute value of the jet pseudorapidity (jet \(|\eta|\)).
%% %The cut on the \(\pT^j\) should be at least half the value used for the merging scale,
%% %in order to not introduce any bias in the MC generation.
%% The samples have been generated using LHAPDF-6.1.5~\cite{Butterworth:2014efa} and FastJet-3.1.0~\cite{Cacciari:2006sm}.


\section[Inclusive Powheg \(V\)]{Inclusive \POWHEG \(V\)}
%\label{sec:v-powheg}

The descriptions below correspond to the samples in \cref{tab:v-powheg}.

\begin{table}[!htbp]
  \caption{Inclusive \(V\) samples with \POWHEG.}%
  \label{tab:v-powheg}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361100--361108    & \(W^+,W^-,Z/\gamma^\ast\) with \(e,\mu,\tau\) decays\\
    301000--301178, 344722    & high-mass slices: \(W^+,W^-,Z\) with \(e,\mu,\tau\) decays \\
    361664--361669 & \(Z/\gamma^\ast\) low-mass slices (\(m=6\)--10--60\,\si{\GeV})\\
    426335--426336 & \(Z/\gamma^\ast\) high-\(\pTX[][\ell\ell] > \SI{150}{\GeV}\) slices \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The \POWHEGBOX[v1] MC generator~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Alioli:2008gx}
was used for the simulation at NLO accuracy of the hard-scattering processes of \(W\)
and \(Z\) boson production and decay in the electron, muon, and \(\tau\)-lepton
channels. It was interfaced to \PYTHIA[8.186]~\cite{Sjostrand:2007gs}
for the modelling of the parton shower, hadronisation, and underlying
event, with parameters set according to the \AZNLO
tune~\cite{STDM-2012-23}. The \CT[10nlo] PDF set~\cite{Lai:2010vv} was used
for the hard-scattering processes, whereas the \CTEQ[6L1] PDF
set~\cite{Pumplin:2002vw} was used for the parton shower. The effect of
QED final-state radiation was simulated with \PHOTOSpp[3.52]~\cite{Golonka:2005pn,Davidson:2010ew}.
The \EVTGEN[1.2.0] program~\cite{Lange:2001uf} was used to decay bottom and charm hadrons.

% No usable \POWHEG \MINLO samples exist in ATLAS central production, therefore
% the description is commented out to avoid confusion

%% \section{\POWHEG \MINLO}
%% \label{sec:vjets-minlo}

%% Predictions from \POWHEG \MINLO~\cite{Alioli:2010xd,Hamilton:2012np,Hamilton:2012rf}
%% interfaced to \PYTHIA[8.210]~\cite{Sjostrand:2007gs} with the
%% AZNLO tune~\cite{STDM-2012-23} are obtained to produce
%% \(V\)+jets events, and will be referred to in the remainder of the note
%% as \POWHEG \MINLO+\PYTHIA[8]. The \EVTGEN[1.2.0] program~\cite{Lange:2001uf}
%% is used as an afterburner to better simulate the decays of bottom and charm hadrons.
%% The \PHOTOSpp[3.61] program~\cite{Golonka:2005pn,Davidson:2010ew} is interfaced to \PYTHIA to accurately
%% describe the QED final state radiation, and the emission of lepton pairs is activated in this setup.
%% The PDF set used in \POWHEG is \CT[14nnlo]~\cite{Dulat:2015mca} whereas the PDF set used in the parton shower
%% is the \CTEQ[6L1]~\cite{Pumplin:2002vw} leading order set.

%% \POWHEG \MINLO is an improvement of the CKKW matching procedure to reach NLO accuracy for
%% boson production in association one jet, and smoothly
%% merges to NLO single boson production at low boson \pT, using no external merging scale.
%% NLO contributions from the CKKW Sudakov form factors are subtracted to the virtual corrections provided by \POWHEGBOX.
%% Thanks to the optimal scale and to the Sudakov form factors, the
%% \POWHEG \MINLO samples do not need any Born suppression cut, and their cross-sections are well-behaved at small boson \pT,
%% contrary to fixed order predictions that diverge in this kinematic phase space.


==> template/MC_snippets/GJ.tex <==
\chapter{Photon processes}
%\label{sec:GJ}

The following paragraphs describe the set-up of the current ATLAS \(\gamma\)+jets and \(\gamma\gamma\)+jets baseline samples.

\section[Sherpa (MEPS@NLO)]{\SHERPA (\MEPSatNLO)}
%\label{sec:gammajets-sherpa-nlo}

\subsection*{Samples}
%\label{sec:gammajets-sherpa-nlo-samples}

The descriptions below correspond to the samples in \cref{tab:gammajets-sherpa-nlo}.

\begin{table}[!htbp]
  \caption{\(\gamma\)+jets and \(\gamma\gamma\)+jets samples with \SHERPA NLO\@.}%
  \label{tab:gammajets-sherpa-nlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364541--364547 & single photon \\
    364350--364354 & diphoton  \\
    \bottomrule
  \end{tabular}
\end{table}


%same description as in~\cref{sec:vjets-sherpa-vjets}
\subsection{\(\gamma\)+jets}
%\label{sec:gammajets-sherpa-nlo-singlephoton}

\paragraph{Short description:}

Prompt single-photon production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} generator. In this set-up, NLO-accurate
matrix elements for up to two partons, and LO-accurate matrix elements for up
to four partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They were matched
with the \SHERPA parton shower~\cite{Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
with a dynamic merging cut~\cite{Siegert:2016bre} of \SI{20}{\GeV}.
Photons were required to be isolated according to
a smooth-cone isolation criterion~\cite{Frixione:1998jh}. Samples were generated using the
\NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}, along with the dedicated set of
tuned parton-shower parameters developed by the \SHERPA authors.


\paragraph{Long description:}

Prompt single-photon production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} parton shower Monte Carlo
generator. In this set-up, NLO-accurate
matrix elements for up to two partons, and LO-accurate matrix elements for up
to four partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries.
The default \SHERPA parton shower~\cite{Schumann:2007mg} based on
Catani--Seymour dipole factorisation and the cluster hadronisation model~\cite{Winter:2003tt}
were used. They employed the dedicated set of tuned parameters developed by the
\SHERPA authors for this generator version and the \NNPDF[3.0nnlo] PDF
set~\cite{Ball:2014uwa}.

The NLO matrix elements for a given jet multiplicity were matched to the parton
shower using a colour-exact variant of the MC@NLO
algorithm~\cite{Hoeche:2011fd}. Different jet multiplicities were then merged
into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.
The merging cut was set dynamically at a scale of \SI{20}{\GeV}
according to the prescription in Ref.~\cite{Siegert:2016bre}.

The renormalisation and factorisation scales for the photon-plus-jet core
process were set to the transverse energy of the photon, \(E_\text{T}^\gamma\).
The strong coupling constant was set to \(\alphas (m_Z)= 0.118\) and the QED coupling
constant was evaluated in the Thomson limit. Photons from the matrix elements were required
to be central, by being within the rapidity range \(|y_{\gamma}|<2.7\), and isolated according to a
smooth-cone isolation criterion~\cite{Frixione:1998jh} with \(\delta_0=0.1\), \(\epsilon_{\gamma}=0.1\) and \(n=2\).

The effects of QCD scale uncertainties were evaluated~\cite{Bothmann:2016nao} using
seven-point variations of the factorisation and renormalisation scales in the matrix elements.
The scales were varied independently by factors of \(0.5\) and \(2\), avoiding variations in opposite directions.

PDF uncertainties for the nominal PDF set were
evaluated using the 100 variation replicas, as well as \(\pm 0.001\) shifts
of \alphas. Additionally, the results were cross-checked using the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa}
PDF sets.

%\textcolor{red}{ Several Monte Carlo slices were generated to ensure good statistics over the whole phase space. In each of them, the photon was required to fall within a \(E_{T}^{\gamma}\) range that depends on the slice avoiding any double-counting when the different slices are combined.}


\subsection[yy+jets]{ \(\gamma\gamma\)+jets}
%\label{sec:gammajets-sherpa-nlo-diphoton}

\paragraph{Short description:}

Prompt diphoton production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} generator. In this set-up, NLO-accurate
matrix elements for up to one parton, and LO-accurate matrix elements for up
to three partons were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They were matched
with the \SHERPA parton shower~\cite{Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
with a dynamic merging cut~\cite{Siegert:2016bre} of \SI{10}{\GeV}.
Photons were required to be isolated according to a smooth-cone isolation
criterion~\cite{Frixione:1998jh}. Samples were generated using the
\NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}, along with the dedicated set of tuned
parton-shower parameters developed by the \SHERPA authors.


\paragraph{Long description:}

Prompt diphoton production was simulated with the
\SHERPA[2.2]~\cite{Bothmann:2019yzt} parton shower Monte Carlo
generator. In this set-up, NLO and LO-accurate
matrix elements were calculated with the Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries.
The default \SHERPA parton shower~\cite{Schumann:2007mg} based on
Catani--Seymour dipole factorisation and the cluster hadronisation model~\cite{Winter:2003tt}
were used. They employed the dedicated set of tuned parameters developed by the
\SHERPA authors for this generator version and the \NNPDF[3.0nnlo]
PDF set~\cite{Ball:2014uwa}.

The NLO matrix elements for a given jet multiplicity were matched to the parton
shower using a colour-exact variant of the MC@NLO algorithm~\cite{Hoeche:2011fd}.
Different jet multiplicities were then merged
into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.
The merging cut was set dynamically to a scale of \SI{20}{\GeV},
according to the prescription in Ref.~\cite{Siegert:2016bre}.

The renormalisation and factorisation scales for the diphoton core process
were set to the invariant mass of the photon pair, \(m_{\gamma\gamma}\).
The strong coupling constant was set to \(\alphas (m_Z)= 0.118\) and the QED coupling
constant was evaluated in the Thomson limit. Photons from the matrix elements were required to be central,
by being within the rapidity range \(|y_{\gamma}|<2.7\), and isolated according to a smooth-cone isolation
criterion~\cite{Frixione:1998jh} with \(\delta_0=0.1\), \(\epsilon_{\gamma}=0.1\) and \(n=2\).
Additionally, the photons were required to be separated by \(\Delta R(\gamma_1,\gamma_2) > 0.2\).


The effects of QCD scale uncertainties were evaluated~\cite{Bothmann:2016nao} using
seven-point variations of the factorisation and renormalisation scales in the matrix elements.
The scales were varied independently by factors of \(0.5\) and \(2\), avoiding variations in opposite directions.

PDF uncertainties for the nominal PDF set were
evaluated using the 100 variation replicas, as well as \(\pm 0.001\) shifts
of \alphas. Additionally, the results were cross-checked using the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa}
PDF sets.
%\textcolor{red}{ Several Monte Carlo slices were generated to ensure good statistics over the whole phase space. In each of them, the photon pair was required to fall within a \(m_{\gamma\gamma}\) range that depends on the slice avoiding any double-counting when the different slices are combined.}


\section[Sherpa (MEPS@NLO)]{\SHERPA (\MEPSatNLO)}
%\label{sec:gammajets-sherpa-lo}

\subsection*{Samples}
%\label{sec:gammajets-sherpa-lo-samples}

The descriptions below correspond to the samples in \cref{tab:gammajets-sherpa-lo}.

\begin{table}[!htbp]
  \caption{\(\gamma\)+jets and  \(\gamma\gamma\)+jets samples with \SHERPA LO\@.}%
  \label{tab:gammajets-sherpa-lo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361039--361062 & single photon \\
    303727--303742 & diphoton \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection[y+jets]{\(\gamma\)+jets}
%\label{sec:gammajets-sherpa-lo-singlephoton}

\paragraph{Description:}

Prompt single-photon production was simulated using the \SHERPA[2.1]~\cite{Bothmann:2019yzt}
generator. The tree-level matrix elements, generated for up to three
additional partons, were merged with the initial- and final-state parton showers using the
\MEPSatLO prescription~\cite{Hoeche:2009rj}. The \CT[10nlo] set of PDFs~\cite{Lai:2010vv} was
used to parameterise the proton structure in conjunction with the dedicated set of tuned
parton-shower parameters developed by the \SHERPA authors for this generator version. A
modified version of the cluster model~\cite{Winter:2003tt} was used
for the description of the fragmentation into hadrons. Photons from the matrix elements were
required to be isolated according to a smooth-cone hadronic isolation criterion~\cite{Frixione:1998jh}
with \(\delta_0=0.3\), \(\epsilon_{\gamma}=0.025\) and \(n=2\).


\subsection[yy+jets]{ \(\gamma\gamma\)+jets}
%\label{sec:gammajets-sherpa-lo-diphoton}

\paragraph{Description:}

Prompt diphoton production was simulated using the \SHERPA[2.1]~\cite{Bothmann:2019yzt}
generator. The tree-level matrix elements, generated for up to two
additional partons, were merged with the initial- and final-state parton showers using the
\MEPSatLO prescription~\cite{Hoeche:2009rj}. The \CT[10nlo] set of PDFs~\cite{Lai:2010vv} was
used to parameterise the proton structure in conjunction with the dedicated set of tuned
parton-shower parameters developed by the \SHERPA authors for this generator version. A
modified version of the cluster model~\cite{Winter:2003tt} was used
for the description of the fragmentation into hadrons. Photons from the matrix elements were
required to be isolated according to a smooth-cone hadronic isolation criterion~\cite{Frixione:1998jh}
with \(\delta_0=0.3\), \(\epsilon_{\gamma}=0.025\) and \(n=2\). Additionally, the photons were
required to be separated by \(\Delta R(\gamma_1,\gamma_2) > 0.2\).


\section[Pythia (LO)]{\PYTHIA (LO)}
%\label{sec:gammajets-pythia-lo}

The descriptions below correspond to the samples in \cref{tab:gammajets-pythia-lo}.

\begin{table}[!htbp]
  \caption{\(\gamma\)+jets and  \(\gamma\gamma\)+jets samples with \PYTHIA.}%
  \label{tab:gammajets-pythia-lo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    423099--423112 & single photon \\
    344008, 302520--34, 364423 & diphoton \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection[y+jets]{\(\gamma\)+jets}
%\label{sec:gammajets-pythia-lo-singlephoton}

\paragraph{Description:}

Prompt single-photon production was simulated using the \PYTHIA[8.186]~\cite{Sjostrand:2007gs} generator.
Events were generated using tree-level matrix elements for photon-plus-jet final
states as well as LO QCD dijet events, with the inclusion of initial-
and final-state parton showers. The fragmentation component was
modelled by final-state QED radiation arising from calculations of all
\(2\rightarrow 2\) QCD processes. The \NNPDF[2.3lo]~\cite{Ball:2012cx} PDF
set was used in the matrix element calculation, the parton shower, and
the simulation of the multi-parton interactions. The samples
include a simulation of the underlying event with parameters set
according to the A14 tune~\cite{ATL-PHYS-PUB-2014-021}. The Lund
string model~\cite{Andersson:1983ia,Sjostrand:1984ic} was used for the
description of the fragmentation into hadrons.


\subsection[yy+jets]{ \(\gamma\gamma\)+jets}
%\label{sec:gammajets-pythia-lo-diphoton}

\paragraph{Description:}

Prompt diphoton production was simulated using the
\PYTHIA[8.186]~\cite{Sjostrand:2007gs} generator. Events were
generated using tree-level matrix elements for diphoton final states,
with the inclusion of initial- and final-state parton showers.  The
fragmentation component was modelled by final-state QED radiation
arising from calculations of photon-plus-jet processes in dedicated
samples. The \NNPDF[2.3lo]~\cite{Ball:2012cx} PDF set was used in the
matrix element calculation, the parton shower, and in the simulation of the
multi-parton interactions. The samples include a simulation of the
underlying event with parameters set according to the A14
tune~\cite{ATL-PHYS-PUB-2014-021}. The Lund string
model~\cite{Andersson:1983ia,Sjostrand:1984ic} was used for the
description of the fragmentation into hadrons.


==> template/MC_snippets/Higgs.tex <==
% !TEX root = MC_snippets.tex

\chapter{Higgs boson processes}
%\label{sec:higgs}

In this chapter, the set-up of the current ATLAS samples for Higgs boson production in gluon--gluon fusion,
vector-boson fusion and Higgs-strahlung processes is described.

\section{\(H\) via gluon--gluon fusion}
%\label{sec:higgs-ggH}

\subsection*{\texorpdfstring{\POWPY[8]}{Powheg+Pythia8} samples}
%\label{sec:higgs-ggH-samples}

%HGam: https://twiki.cern.ch/twiki/bin/view/Sandbox/RuggeroTurraSandbox
%ZZ: https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HZZllllRun2MCSamplesMC16#mc16
%WW: https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HWWMC
%Hlep:https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HSG4MCrequests2015
%Hbb: https://twiki.cern.ch/twiki/bin/view/AtlasProtected/HbbMC

The descriptions below correspond to the samples in \cref{tab:higgs-ggH-samples}.

\begin{table}[!htbp]
  \caption{\POWHEG Higgs gluon--gluon fusion samples with \POWPY[8] for different Higgs boson decay channels.}%
  \label{tab:higgs-ggH-samples}
  \centering
  \begin{tabular}{ l | l | l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    343981 & \(H\to\gamma\gamma\)&   \\
    345316 & \(H\to Z\gamma\) & \\
    345060 & \(H\to ZZ^{*} \to 4\ell \) & \(\ell=e,\mu,\tau\)   \\
    345324 & \(H\to WW^{*} \to 2\ell2\nu \) &  \(\pTX[][\ell1] > \SI{15}{\GeV}\) and \(\pTX[][\ell2] > \SI{5}{\GeV}\) \\
    308284 & \(H\to ZZ^{*}\to 4\nu\) & \(\MET > \SI{75}{\GeV}\)\\
    345342 & \(H\to b \bar{b}\) & \\
    345097 & \(H\to\mu\mu\)      &     \\
    345120 & \(H\to\tau\tau\to \ell^{+}\ell^{-}\) & \(\pTX[][\ell1] > \SI{13}{\GeV}\) and \(\pTX[][\ell2] > \SI{7}{\GeV}\) \\
    345121 & \(H\to\tau\tau\to h^{+}\ell^{-}\)    & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    345122 & \(H\to\tau\tau\to \ell^{+}h^{-}\)    & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    345123 & \(H\to\tau\tau\to h^{+}h^{-}\)       & \(\pTX[][h1]    > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\) \\
    345124 & \(H\to\tau\tau\to \mu\tau\)          & \\ %\(\pTX[][h1] > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\)
    345125 & \(H\to\tau\tau\to e \tau\)           & \\ %\(\pTX[][h1] > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\)
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Higgs boson production via gluon--gluon fusion was simulated at next-to-next-to-leading-order (NNLO) accuracy in
QCD using \POWHEGBOX[v2]~\cite{Hamilton:2013fea,Hamilton:2015nsa,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}.
The simulation achieved NNLO accuracy for arbitrary inclusive \(gg\to H\) observables by reweighting the Higgs boson
rapidity spectrum in \textsc{Hj}-\MINLO~\cite{Hamilton:2012np,Campbell:2012am,Hamilton:2012rf} to that of HNNLO~\cite{Catani:2007vq}.
%The transverse momentum spectrum of the Higgs boson obtained with this sample was found to be compatible with the fixed-order HNNLO calculation and the Hres2.3 calculation~\cite{Bozzi:2005wk,deFlorian:2011xf} performing resummation at next-to-next-to- leading-logarithm accuracy matched to a NNLO fixed-order calculation (NNLL+NNLO).
The \PDFforLHC[15nnlo] PDF set~\cite{Butterworth:2015oua} and the \AZNLO tune~\cite{STDM-2012-23}
of \PYTHIA[8]~\cite{Sjostrand:2014zea} were used.

The gluon--gluon fusion prediction from the Monte Carlo samples was normalised to the
next-to-next-to-next-to-leading-order cross-section in QCD plus electroweak corrections
at next-to-leading order
(NLO)~\cite{deFlorian:2016spz,Anastasiou:2016cez,Anastasiou:2015ema,Dulat:2018rbf,Harlander:2009mq,Harlander:2009bw,Harlander:2009my,Pak:2009dg,Actis:2008ug,Actis:2008ts,Bonetti:2018ukf,Bonetti:2018ukf}. The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}.
The normalisation of all Higgs boson
samples accounts for the decay branching ratio calculated with HDECAY~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz}
and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\paragraph{Long description:}

Higgs boson production via gluon--gluon fusion was simulated at next-to-next-to-leading-order (NNLO) accuracy in QCD using
\POWHEGBOX[v2]~\cite{Hamilton:2013fea,Hamilton:2015nsa,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}. The simulation achieved NNLO
accuracy for arbitrary inclusive \(gg\to H\) observables by reweighting the Higgs boson rapidity spectrum
in \textsc{Hj}-\MINLO~\cite{Hamilton:2012np,Campbell:2012am,Hamilton:2012rf} to that of HNNLO~\cite{Catani:2007vq}. The transverse momentum
spectrum of the Higgs boson obtained with this sample was found to be compatible with the fixed-order HNNLO calculation and the
\HRES[2.3] calculation~\cite{Bozzi:2005wk,deFlorian:2011xf} performing resummation at next-to-next-to-leading-logarithm accuracy
matched to a NNLO fixed-order calculation (NNLL+NNLO).
Top- and bottom-quark mass effects were included up to next-to-leading order (NLO).

The renormalisation and factorisation scales were set to half of the Higgs boson mass and the \PDFforLHC[15nnlo] PDF
set~\cite{Butterworth:2015oua} was used. The matrix elements were matched to the parton shower of \PYTHIA[8]~\cite{Sjostrand:2014zea}
which uses the AZNLO tune~\cite{STDM-2012-23}. The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}.

The QCD scale uncertainties were obtained using nine-point scale variations of the NLO renormalisation and factorisation scales and applying the NNLO reweighting to those variations, including up and down variations of \(\muR=\muF\) around the central value for the NNLO part, yielding a total of 27 scale variations.
PDF and \alphas uncertainties were estimated using the \PDFforLHC[15nlo] set of eigenvectors.
The envelope of the resulting 27 scale variations was taken to estimate the QCD scale uncertainty.
Uncertainties were also provided for switching off bottom- and top-quark mass effects.
%From YR4

The prediction from the Monte Carlo samples was normalised to the next-to-next-to-next-to-leading-order
cross-section in QCD in the infinite top-quark mass
limit~\cite{deFlorian:2016spz,Anastasiou:2016cez,Anastasiou:2015ema,Dulat:2018rbf,Aglietti:2004nj} and including exact
corrections for all finite quark-mass effects at NLO in QCD as well as NLO electroweak
effects~\cite{Actis:2008ug,Bonetti:2018ukf}. Additionally, corrections to the inverse of the top-quark mass were taken
into account at NNLO~\cite{Harlander:2009mq,Harlander:2009bw,Harlander:2009my,Pak:2009dg}.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated with
HDECAY~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz}
and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\section{\(H\) via vector-boson fusion}
%\label{sec:higgs-VBF}

\subsection*{\texorpdfstring{\POWPY[8]}{Powheg+Pythia8} samples}
%\label{sec:higgs-VBF-samples}

The descriptions below correspond to the samples in \cref{tab:higgs-VBF-samples}.

\begin{table}[!htbp]
  \caption{\POWPY[8] Higgs vector-boson fusion samples for different Higgs boson decay channels.}%
  \label{tab:higgs-VBF-samples}
  \centering
  \begin{tabular}{ l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    346317 & \(H\to\) all  & \\
    346214 & \(H\to\gamma\gamma\)& \\
    345833 & \(H\to Z\gamma\) & \(Z\to \ell^{+}\ell^{-}\) \\
    345834 & \(H\to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\) \\
    346228 & \(H\to ZZ^{*} \to 4\ell \) & \(\ell=e,\mu\) \\
    450576 & \(H\to ZZ^{*} \to 2\ell2b \) &  \\
    345948 & \(H\to WW^{*} \to 2\ell2\nu \) &  \(\pTX[][\ell1] > \SI{15}{\GeV}\) and \(\pTX[][\ell2] > \SI{5}{\GeV}\) \\
    346600 & \(H\to ZZ^{*}\to 4\nu\) & \(\MET > \SI{75}{\GeV}\) \\
    345949 & \(H\to b \bar{b}\) & \\
    % & \(H\to\mu\mu\)      &     \\
    346190& \(H\to\tau\tau\to \ell^{+}\ell^{-}\) & \(\pTX[][\ell1] > \SI{13}{\GeV}\) and \(\pTX[][\ell2] > \SI{7}{\GeV}\) \\
    346191 & \(H\to\tau\tau\to h^{+}\ell^{-}\)   & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    346192 & \(H\to\tau\tau\to \ell^{+}h^{-}\)   & \(\pTX[][\ell]  > \SI{15}{\GeV}\) and \(\pTX[][h]     > \SI{20}{\GeV}\) \\
    346193 & \(H\to\tau\tau\to h^{+}h^{-}\)      & \(\pTX[][h1]    > \SI{30}{\GeV}\) and \(\pTX[][h2]    > \SI{20}{\GeV}\) \\
    346194 & \(H\to\tau\tau\to e\tau\)           & \\%\(\pTX[][l1] > \SI{10}{\GeV}\) and \(\pTX[][h1]    > \SI{20}{\GeV}\) \\
    346195 & \(H\to\tau\tau\to \mu\tau\)         & \\%\(\pTX[][l1] > \SI{10}{\GeV}\) and \(\pTX[][h1]    > \SI{20}{\GeV}\) \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Higgs boson production via vector-boson fusion was simulated with
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}
and interfaced with \PYTHIA[8]~\cite{Sjostrand:2014zea} for parton shower and non-perturbative effects,
with parameters set according to the \AZNLO tune~\cite{STDM-2012-23}.
The \POWHEGBOX prediction is accurate to next-to-leading order (NLO) and uses
the \PDFforLHC[15nlo] PDF set~\cite{Butterworth:2015oua}.
%It was tuned to match calculations with effects due to finite heavy-quark masses
%and soft-gluon resummation up to NNLL.
It was normalised to an approximate-NNLO QCD cross-section
with NLO electroweak corrections~\cite{Ciccolini:2007jr,Ciccolini:2007ec,Bolzoni:2010xr}.
The decays of bottom and charm hadrons were performed by \EVTGEN~\cite{Lange:2001uf}.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated
with \textsc{HDECAY}~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz}
and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\paragraph{Long description:}

Higgs boson production via vector-boson fusion was simulated with
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}. A factorised approximation, where cross-talk between the
fermion lines is neglected, was used. The implementation is based on the respective NLO QCD calculations for genuine \(W/Z\) vector-boson
fusion topologies (VBF approximation). Quark--antiquark annihilation and interference contributions
between \(t\)- and \(u\)-channel contributions were disregarded.
%External fermion masses are neglected throughout.  For the choice of renormalisation and factorisation scales, various options are available.  For this report, fixed scales,μF=μR=MW, are used, and contributions from external bottom and top quarks are entirely disregarded.

The renormalisation and factorisation scales were set to the \(W\) boson mass and the \PDFforLHC[15nlo] PDF set~\cite{Butterworth:2015oua}
was used. The matrix elements were matched to the parton shower of \PYTHIA[8]~\cite{Sjostrand:2014zea} which uses the \AZNLO
tune~\cite{STDM-2012-23}. A dipole-recoil strategy was used for the parton shower.The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}.%, which provides a better agreement than other recoil schemes with the NNLO predictions of proVBFH (not included in the HiggsReference twiki). % cite https://arxiv.org/pdf/1710.00391.pdf ?,

%The samples include weight variations evaluated on-the-fly for the estimation of QCD scale, PDF- and \alphas-induced uncertainties.
The QCD scales \muR and \muF were varied independently by factors of 0.5 and 2.0, both in the matrix element
and in the parton shower.

The prediction from the \POWHEGBOX sample was normalised to the next-to-next-to-leading-order cross-section in QCD
using the VBF approximation~\cite{Ciccolini:2007jr,Ciccolini:2007ec,Bolzoni:2010xr}. Relative
next-to-leading-order electroweak corrections were also taken into account for the \(t\)- and \(u\)-channel contribution
considered in the VBF approximation. The normalisation of all Higgs boson samples accounts for the decay branching
ratio calculated with \textsc{HDECAY}~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz} and
\PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\section{\(VH\)}
%\label{sec:higgs-VH}

This section describes the generation details of nominal samples for Higgs-strahlung production.

\subsection*{\texorpdfstring{\POWPY[8]}{Powheg+Pythia8} samples}
%\label{sec:higgs-VH-samples}

The descriptions below correspond to the samples in \crefrange{tab:higgs-ZH-samples}{tab:higgs-ggZH-samples}.

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of Higgs boson production in association with a \(Z\) boson for different Higgs boson decay channels.}%
  \label{tab:higgs-ZH-samples}
  \centering
  \begin{tabular}{ l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345038 & \(H \to ZZ^{*} \to 4\ell\) & \(Z\to\) all\\
    345319 & \(H \to \gamma\gamma\) & \(Z\to\) all\\
    345322 & \(H \to Z\gamma\) & \(Z\to\) all\\
    345103 & \(H \to\mu\mu\) & \(Z\to\) all\\
    345217 & \(H \to\tau\tau\)& \(Z\to\) all\\
    345218 & \(H \to e\tau\) &\(Z\to\) all\\
    345219 & \(H \to \mu\tau\)&\(Z\to\) all\\
    345445 & \(H \to WW^{*} \to 2\ell2\nu \) & \(Z\to\) all \\
    345876 & \(H\ to ee\) &\(Z\to\) all \\
    345965 & \(H \to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\); \(Z\to\) all\\
    346310 & \(H \to\) all&\(Z\to\) all\\
    346607 & \(H \to ZZ^{*} \to 4\nu \) &\(Z\to \ell^{+}\ell^{-}\) \\
    345055 & \(H \to b\bar{b}\)              & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    345111 & \(H \to c\bar{c}\)              & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    345337 & \(H \to WW^{*} \to 2\ell2\nu \) & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    346326 & \(H \to\tau\tau\)               & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    346693 & \(H \to ZZ^{*} \to 4\nu \)      & \pTX[][Z] enhancement; \(Z\to \ell^{+}\ell^{-}\)\\
    345056 & \(H \to b\bar{b}\)              & \pTX[][Z] enhancement; \(Z\to \nu\bar{\nu}\)\\
    345112 & \(H \to c\bar{c}\)              & \pTX[][Z] enhancement; \(Z\to \nu\bar{\nu}\)\\
    345445 & \(H \to WW^{*} \to 2\ell2\nu\)  & \pTX[][Z] enhancement; \(Z\to \nu\bar{\nu}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of Higgs boson production in association with a \(W^{+}\) boson for different Higgs boson decay channels.}
  \label{tab:higgs-WpH-samples}
  \centering
  \begin{tabular}{l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345039 & \(H \to ZZ^{*} \to 4\ell\) & \(W^{+}\to\) all\\
    345318 & \(H \to \gamma\gamma\) & \(W^{+}\to\) all\\
    345104 & \(H \to \mu\mu\) &  \(W^{+}\to\) all\\
    345212 & \(H \to \tau\tau\) &  \(W^{+}\to\) all\\
    345214 & \(H \to e \tau \) & \(W^{+}\to\) all\\
    345216 & \(H \to \mu \tau \) & \(W^{+}\to\) all\\
    345321 & \(H \to Z\gamma\) & \(W^{+}\to\) all\\
    345325 & \(H \to WW^{*} \to 2\ell2\nu \) & \(W^{+} \to q\bar{q}\) \\
    345877 & \(H \to e^{+}e^{-}\) & \(W^{+}\to\) all\\
    345964 & \(H \to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\); \(W^{+}\to\) all\\
    346311 & \(H \to\) all & \(W^{+}\to\) all\\
    346605 & \(H \to ZZ^{*} \to 4\nu \) & \(W^{+}\to\) all\\
    346699 & \(H \to 4\ell\) & interfaced to PROPHECY4F \\
    346705 & \(H \to 4\ell\) & interfaced to Hto4l \\
    345054 & \(H \to b\bar{b}\)                   & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    345110 & \(H \to c\bar{c}\)                   & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    345327 & \(H \to WW^{*} \to 2\ell2\nu\)       & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    346561 & \(H \to WW^{*} \to q\bar{q}\ell\nu\) & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    346325 & \(H \to \tau\tau\)                   & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    346729 & \(H \to ZZ^{*} \to 4\nu\)            & \pTX[][W] enhancement; \(W^{+}\to \ell^{+}\nu\) \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of Higgs boson production in association with a \(W^{-}\) boson for different Higgs boson decay channels.}
  \label{tab:higgs-WmH-samples}
  \centering
  \begin{tabular}{l l l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345040 & \(H \to ZZ^{*} \to 4\ell\) & \(W^{-}\to\) all\\
    345317 & \(H \to \gamma\gamma\) & \(W^{-}\to\) all\\
    345105 & \(H \to \mu\mu\) &  \(W^{-}\to\) all\\
    345211 & \(H \to \tau\tau\) &  \(W^{-}\to\) all\\
    345213 & \(H \to e \tau \) & \(W^{-}\to\) all\\
    345215 & \(H \to \mu \tau \) & \(W^{-}\to\) all\\
    345320 & \(H \to Z\gamma\) & \(W^{-}\to\) all\\
    345333 & \(H \to WW^{*} \to 2\ell2\nu \) & \(W^{-} \to q\bar{q}\) \\
    345878 & \(H \to e^{+}e^{-}\) & \(W^{-}\to\) all\\
    345963 & \(H \to \gamma\gamma^{*}\) & \(\gamma^{*}\to \ell^{+}\ell^{-}\); \(W^{-}\to\) all\\
    346312 & \(H \to\) all & \(W^{-}\to\) all\\
    346606 & \(H \to ZZ^{*} \to 4\nu \) & \(W^{-}\to\) all\\
    346700 & \(H \to 4\ell\) & interfaced to PROPHECY4F \\
    346706 & \(H \to 4\ell\) & interfaced to Hto4l \\
    345053 & \(H \to b\bar{b}\)                   & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    345109 & \(H \to c\bar{c}\)                   & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\)  \\
    345326 & \(H \to WW^{*} \to 2\ell2\nu\)       & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    346560 & \(H \to WW^{*} \to q\bar{q}\ell\nu\) & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    346324 & \(H \to \tau\tau\)                   & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    346730 & \(H \to ZZ^{*} \to 4\nu\)            & \pTX[][W] enhancement; \(W^{-}\to \ell^{-}\bar{\nu}\) \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[!htbp]
  \caption{\POWPY[8] samples of loop-induced Higgs boson production in association with a \(Z\) boson for different
  Higgs boson decay channels.}%
  \label{tab:higgs-ggZH-samples}
  \centering
  \begin{tabular}{ l | l | l}
    \toprule
    DSID   & Decay channel & Additional comment \\
    \midrule
    345061 & \(H \to \gamma\gamma\) & \(Z\to\) all \\
    345066 & \(H \to ZZ^{*} \to 4\ell\) & \(Z\to\) all \\
    345098 & \(H \to \mu\mu\) & \(Z\to\) all \\
    345596 & \(H \to ZZ^{*} \to 4\nu\) & \(Z\to\) all \\
    346524 & \(H \to WW^{*} \to 2\ell2\nu \) & \(Z\to\) all \\
    346697 & \(H \to ZZ^{*} \to 4\nu\) & interfaced to PROPHECY4F \\
    346703 & \(H \to ZZ^{*} \to 4\nu\) & interfaced to Hto4l \\
    345057 & \(H \to b\bar{b}\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    345113 & \(H \to c\bar{c}\) & \(Z\to \ell^{+}\ell^{-}\)\\
    345446 & \(H \to WW^{*} \to 2\ell2\nu\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    346329 & \(H \to \tau\tau\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    346694 & \(H \to ZZ^{*} \to 4\nu\) &  \(Z\to \ell^{+}\ell^{-}\)\\
    345058 & \(H \to b\bar{b}\) & \(Z\to \nu\bar{\nu}\)\\
    345114 & \(H \to c\bar{c}\) & \(Z\to \nu\bar{\nu}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Higgs boson production in association with a vector boson was simulated using
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw} and interfaced with \PYTHIA[8]~\cite{Sjostrand:2014zea} for
parton shower and non-perturbative effects. The \POWHEGBOX prediction is accurate to next-to-leading order for \(VH\) boson plus one-jet production.
The loop-induced \(gg\to ZH\) process was generated separately at leading order. The \PDFforLHC[15nlo] PDF
set~\cite{Butterworth:2015oua} and the \AZNLO tune~\cite{STDM-2012-23} of \PYTHIA[8]~\cite{Sjostrand:2014zea} were used. The decays of bottom and charm hadrons
were performed by \EVTGEN~\cite{Lange:2001uf}. The Monte Carlo
prediction was normalised to cross-sections calculated at NNLO in QCD with NLO electroweak corrections for \(q\bar{q}/qg \to VH\) and at NLO
and next-to-leading-logarithm accuracy in QCD for
\(gg \to ZH\)~\cite{Ciccolini:2003jy,Brein:2003wg,Brein:2011vx,Altenkamp:2012sx,Denner:2014cla,Brein:2012ne,Harlander:2014wda}.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated with
HDECAY~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz} and \PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


\paragraph{Long description:}

Higgs boson production in association with a vector boson was simulated using
\POWHEGBOX[v2]~\cite{Nason:2009ai,Alioli:2010xd,Nason:2004rx,Frixione:2007vw}. The computation was carried out using the
\MINLO~\cite{Luisoni:2013cuh} prescription, which achieves NLO accuracy for the \(VH\) and \(VH\) boson plus one-jet production
inclusive distributions and dictates the choice of renormalisation and factorisation scales. Virtual amplitudes were constructed
through the interface to the \GOSAM package~\cite{Cullen:2011ac}. The loop-induced \(gg\to ZH\) process was generated separately at
leading order with \POWHEGBOX. In all cases, the \PDFforLHC[15nlo] PDF set~\cite{Butterworth:2015oua} was used.

The matrix elements were matched to the parton shower of \PYTHIA[8]~\cite{Sjostrand:2014zea} which uses the \AZNLO
tune~\cite{STDM-2012-23}. The decays of bottom and charm hadrons were performed by \EVTGEN~\cite{Lange:2001uf}.
%The samples include weight variations evaluated on-the-fly for the estimation of QCD scale, PDF- and \alphas-induced uncertainties.
The QCD scales \muR and \muF were varied independently by factors of 0.5 and 2.0 to account for their uncertainties.

The predictions from \POWHEGBOX were normalised to the best available theoretical prediction. The  \(q\bar{q}/qg \to VH\) cross-sections
were calculated at NNLO in QCD with NLO electroweak corrections and the \(gg \to ZH\) cross-sections were calculated at NLO and
next-to-leading-logarithm accuracy~\cite{Ciccolini:2003jy,Brein:2003wg,Brein:2011vx,Altenkamp:2012sx,Denner:2014cla,Brein:2012ne,Harlander:2014wda}.
The normalisation of the \(q\bar{q}\to ZH\) samples was extracted from the subtraction of the latter from the former.
Differential NLO EW corrections were available from the \textsc{HAWK} program~\cite{Denner:2014cla} to be applied to
\(q\bar{q}\)-initiated \(VH\) production as a function of the vector boson's transverse momentum.
The normalisation of all Higgs boson samples accounts for the decay branching ratio calculated with
\textsc{HDECAY}~\cite{Djouadi:1997yw,Spira:1997dg,Djouadi:2006bz} and
\PROPHECY~\cite{Bredenstein:2006ha,Bredenstein:2006rh,Bredenstein:2006nk}.


==> template/MC_snippets/MB.tex <==
% !TEX root = MC_snippets.tex

\chapter{Multiboson processes}
%\label{sec:MB}

In the following paragraphs, the set-ups of the current ATLAS multiboson baseline samples are described.
Details of the full process configuration are given in the PUB note~\cite{ATL-PHYS-PUB-2017-005}.


\section[Inclusive Powheg]{Inclusive \POWHEG}
%\label{sec:MB-powheg}

The descriptions below correspond to the samples in \cref{tab:MB-powheg}.

\begin{table}[htbp]
  \caption{Inclusive \(VV\) samples with \POWHEG.}%
  \label{tab:MB-powheg}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361600--361605 & inclusive \(WW(2\ell 2\nu), WZ(3\ell\nu), ZZ(4\ell), ZZ(4\nu), ZZ(2\ell 2\nu)\) (all lepton flavours)\\
    361606--361611 & inclusive \(WW/WZ/ZZ\) semileptonic decays (\(\ell\ell qq\), \(\ell\nu qq\), \(\nu\nu qq\), all lepton flavours)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The \POWHEGBOX[v2]~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd} generator
was used to simulate the \(WW\), \(WZ\) and \(ZZ\)~\cite{Nason:2013ydw} production
processes at NLO accuracy in QCD. The effect of singly resonant
amplitudes and interference effects due to \(Z/\gamma^*\) and
same-flavour lepton combinations in the final state were included, where appropriate.
Interference effects between \(WW\) and \(ZZ\) for same-flavour charged leptons and
neutrinos were ignored.
Events were interfaced to \PYTHIA[8.210]~\cite{Sjostrand:2014zea}
for the modelling of the parton shower, hadronisation, and underlying
event, with parameters set according to the \AZNLO
tune~\cite{STDM-2012-23}. The \CT[10] PDF set~\cite{Lai:2010vv} was used
for the hard-scattering processes, whereas the \CTEQ[6L1] PDF
set~\cite{Pumplin:2002vw} was used for the parton shower. The \EVTGEN[1.2.0]
program~\cite{Lange:2001uf} was used to decay bottom and charm hadrons.

The factorisation and renormalisation scales were set to the invariant mass of
the boson pair. An invariant mass of \(m_{\ell\ell} > \SI{4}{\GeV}\) was required
at matrix-element level for any pair of same-flavour charged leptons.


\section[Sherpa]{\SHERPA}
%\label{sec:MB-sherpa}

\subsection{Fully leptonic, semileptonic and loop-induced \texorpdfstring{\(VV\)}{VV}}
%\label{sec:MB-sherpa-fully}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa}. They describe the almost
identical set-ups of fully leptonic (including loop-induced \(VV\) production)
and semileptonic \(VV\) decays. For loop-induced processes \(gg\to VV\),
the description below assumes that the `nominal' samples with
Higgs contributions are used. If you are using specialised set-ups that
exclude the Higgs component, the description should be modified appropriately.
(Get in touch with the PMG Weak Boson Processes subgroup if you are unsure.)

\begin{table}[htbp]
  \caption{\(VV\) samples with \SHERPA: fully leptonic, semileptonic,
    loop-induced fully leptonic, loop-induced semileptonic. SFOS stands for
    \enquote{same flavour opposite-charge sign}.}%
  \label{tab:MB-sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364250--364255, 363494   & \(4\ell, 3\ell\nu, 2\ell 2\nu, 4\nu\) with \(m_{\ell\ell}\mathrm{(SFOS)} > \SI{4}{\GeV}\), \(\pTX[\ell](1,2) > \SI{5}{\GeV}\)\\
    364288--364290 & fully leptonic low \(m_{\ell\ell}\) and \(\pTX[\ell]\) complement\\
    \midrule
    345705--345727   & loop-induced leptonic\\
    \midrule
    363355-363360, 363489   & semileptonic, on-shell diboson production with factorised decays\\
    \midrule
    364302-364305   & loop-induced semileptonic, using factorised on-shell decays)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples of diboson final states (\(VV\)) were simulated with the
\SHERPA[2.2.1] or 2.2.2~\cite{Bothmann:2019yzt} generator depending on the process,
%~\footnote{This is an admixture of 2.2.1 and above versions, so the version should be kept generic to avoid confusions. As an
%alternative, the sentence can be modified indicating that samples are simulated with the \SHERPA[2.2.1] or 2.2.2 depending on the process.}
including off-shell effects and Higgs boson contributions, where appropriate.
Fully leptonic final states and semileptonic final states, where one boson
decays leptonically and the other hadronically, were generated using
matrix elements at NLO accuracy in QCD for up to one additional parton
and at LO accuracy for up to three additional parton
emissions. Samples for the loop-induced processes \(gg \to VV\) were
generated using LO-accurate matrix elements for up to one
additional parton emission for both the cases of fully leptonic and
semileptonic final states. The matrix element calculations were matched
and merged with the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the MEPS@NLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections were provided by the
\OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}. The
\NNPDF[3.0nnlo] set of PDFs was used~\cite{Ball:2014uwa}, along with the
dedicated set of tuned parton-shower parameters developed by the
\SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample using an
improved CKKW matching procedure~\cite{Catani:2001cc,Hoeche:2009rj}
which is extended to NLO accuracy using the MEPS@NLO
prescription~\cite{Hoeche:2012yf}. The virtual QCD corrections for
matrix elements at NLO accuracy were provided by the
\OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}. The
calculation was performed in the \(G_\mu\) scheme, ensuring an
optimal description of pure electroweak interactions at the
electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Electroweak VVjj]{Electroweak \(VVjj\)}
%\label{sec:MB-sherpa-vvjj}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vvjj}.

\begin{table}[htbp]
  \caption{Electroweak \(VVjj\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vvjj}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364283--364284   & \(\ell\ell\ell\ell jj\), \(\ell\ell\ell\nu jj\)\\
    364285   &  \(\ell\ell\nu\nu jj\) opposite-sign\\
    364287   &  \(\ell\ell\nu\nu jj\) same-sign\\
    366086--366089   &  \(\ell\ell\ell\ell jj\), \(\ell\ell\ell\nu jj\), \(\ell\ell\nu\nu jj\), with the triboson contributions removed\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Electroweak production of a diboson in association with two jets
(\(VVjj\)) was simulated with the \SHERPA[2.2.2]~\cite{Bothmann:2019yzt}
generator. The LO-accurate matrix elements were matched to a parton
shower based on Catani--Seymour dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the MEPS@LO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa},
along with the dedicated set of tuned parton-shower parameters
developed by the \SHERPA authors.

\paragraph{Additional description:} The calculation was performed in the
\(G_\mu\) scheme, ensuring an optimal description of pure
electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Vgamma (NLO, biased)]{\(V\gamma\) (NLO, biased)}
%\label{sec:MB-sherpa-vgamma-nlo-biased}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vynlo-ew}.

\begin{table}[htbp]
  \caption{NLO \(V\gamma\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vynlo-ew}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    700011--700017 & biased in \(\log_{10}(\max[\pT(V), \pT(\gamma)])\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of \(V\gamma\) final states was simulated with the
\SHERPA[2.2.8]~\cite{Bothmann:2019yzt} generator.  Matrix elements at
NLO QCD accuracy for up to one additional parton and LO accuracy for
up to three additional parton emissions were matched and merged with
the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the MEPS@NLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections for matrix elements at NLO accuracy were provided by
the \OPENLOOPS[2] library~\cite{Buccioni:2019sur,Cascioli:2011va,Buccioni:2017yxi,Denner:2016kdg}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa}, along with
the dedicated set of tuned parton-shower parameters developed by the \SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the MEPS@NLO prescription~\cite{Hoeche:2012yf}.
The virtual QCD corrections for matrix elements at NLO accuracy were provided by
the \OPENLOOPS[2] library~\cite{Buccioni:2019sur,Cascioli:2011va,Buccioni:2017yxi,Denner:2016kdg}.
Multijet merging at NLO accuracy in the electroweak coupling was based on
the \NLOEWvirt approach~\cite{Kallweit:2014xda,Kallweit:2015dum}.
The calculation was performed in the \(G_\mu\) scheme, ensuring an optimal
description of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Vgamma (NLO, sliced)]{\(V\gamma\) (NLO, sliced)}
%\label{sec:MB-sherpa-vgamma-nlo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vynlo}.

\begin{table}[htbp]
  \caption{NLO \(V\gamma\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vynlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364500--364535   & sliced in \pTX[\gamma]\\
    345887--345900   & sliced in \(m_{\ell\ell}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of \(V\gamma\) final states was simulated with the
\SHERPA[2.2.2]~\cite{Bothmann:2019yzt} generator.  Matrix elements at
NLO QCD accuracy for up to one additional parton and LO accuracy for
up to three additional parton emissions were matched and merged with
the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections for matrix elements at NLO accuracy were
provided by the
\OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}. Samples
were generated using the \NNPDF[3.0nnlo] PDFset~\cite{Ball:2014uwa}, along with
the dedicated set of tuned parton-shower parameters developed by the
\SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj} which was extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.
The virtual QCD corrections for matrix elements at NLO accuracy were
provided by the \OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}.
The calculation was performed in the \(G_\mu\) scheme, ensuring an optimal
description of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection[Vgamma (LO)]{\(V\gamma\) (LO)}
%\label{sec:MB-sherpa-vgamma-lo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vylo}.

\begin{table}[htbp]
  \caption{LO \(V\gamma\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vylo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    366140--366154   & \SHERPA[2.2.4], \(Z(\to ee/\mu\mu/\tau\tau)\gamma\), sliced in \pTX[\gamma]\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of \(V\gamma\) final states was simulated with the
\SHERPA[2.2.4]~\cite{Bothmann:2019yzt} generator. Matrix elements at LO
accuracy in QCD for up to three additional parton emissions were
matched and merged with the \SHERPA parton shower based on
Catani--Seymour dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg}
using the \MEPSatLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa},
along with the dedicated set of tuned parton-shower parameters
developed by the \SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj}.
The calculation was performed in the \(G_\mu\) scheme, ensuring an optimal
description of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection{Tribosons (NLO)}
%\label{sec:MB-sherpa-vvv-nlo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vvvnlo}.

\begin{table}[htbp]
  \caption{NLO \(VVV\) samples (factorised decays) with \SHERPA.}%
  \label{tab:MB-sherpa-vvvnlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    363507--363509   & \(3\ell1\nu2j\), \(4\ell2j\)\\
    364242--364249   & fully leptonic decays\\
    364336--364339   & \(WWW\to 2\ell2\nu jj\)\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of triboson (\(VVV\)) events was simulated with the
\SHERPA[2.2.2]~\cite{Bothmann:2019yzt} generator using factorised gauge-boson decays.
Matrix elements, accurate to NLO for the inclusive process and to LO for up to
two additional parton emissions, were matched and merged with the \SHERPA parton
shower based on Catani--Seymour dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg}
using the \MEPSatNLO prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
The virtual QCD corrections for matrix elements at NLO accuracy were
provided by the \OPENLOOPS library~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}.
Samples were generated using the \NNPDF[3.0nnlo] PEF set~\cite{Ball:2014uwa}, along with
the dedicated set of tuned parton-shower parameters developed by the \SHERPA authors.


\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching procedure~\cite{Catani:2001cc,Hoeche:2009rj} which is extended to NLO
accuracy using the \MEPSatNLO prescription~\cite{Hoeche:2012yf}.  The
calculation was performed in the \(G_\mu\) scheme, ensuring an optimal description of pure electroweak interactions at the
electroweak scale.

\input{sherpa_scale_pdf.tex}


\subsection{Tribosons (LO)}
%\label{sec:MB-sherpa-vvv-lo}

The descriptions below correspond to the samples in
\cref{tab:MB-sherpa-vvvlo}.

\begin{table}[htbp]
  \caption{LO \(VVV\) samples with \SHERPA.}%
  \label{tab:MB-sherpa-vvvlo}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    407311--407315   & on- and off-shell contributions to 6-lepton production\\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

The production of triboson (\(VVV\)) events was simulated with the
\SHERPA[2.2.1]~\cite{Bothmann:2019yzt} generator. Matrix elements accurate to LO in QCD
for up to one additional parton emission were matched and merged with the \SHERPA parton shower based on Catani--Seymour
dipole factorisation~\cite{Gleisberg:2008fv,Schumann:2007mg} using the \MEPSatLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}.
Samples were generated using the \NNPDF[3.0nnlo] PDF set~\cite{Ball:2014uwa},
along with the dedicated set of tuned parton-shower parameters
developed by the \SHERPA authors.

\paragraph{Additional description:}

The ME+PS matching~\cite{Hoeche:2011fd} was employed for different jet
multiplicities which were then merged into an inclusive sample
using an improved CKKW matching
procedure~\cite{Catani:2001cc,Hoeche:2009rj}.  The calculation was
performed in the \(G_\mu\) scheme, ensuring an optimal description
of pure electroweak interactions at the electroweak scale.

\input{sherpa_scale_pdf.tex}


==> template/MC_snippets/MJ.tex <==
\chapter{Jet processes}
%\label{sec:MJ}

This section describes the MC samples used for the modelling of multijet production.
\Cref{subsec:jets-pythia} describes the \PYTHIA[8] samples,
\cref{subsec:jets-herwig} describes the \HERWIG[7] samples,
\cref{subsec:jets-powheg} describes the \POWPY[8] samples,
and finally \cref{subsec:jets-sherpa} describes the \SHERPA samples.

\section[Pythia 8]{\PYTHIA[8]}
\label{subsec:jets-pythia}

The descriptions below correspond to the samples in \cref{tab:mj_pythia}.

\begin{table}[!htbp]
  \caption{Nominal multijet samples produced with \PYTHIA.}%
  \label{tab:mj_pythia}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364700--364712 & \PYTHIA with shower weights \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Multijet production was generated using \PYTHIA[8.230]~\cite{Sjostrand:2014zea} with leading-order matrix elements
for dijet production which were matched to the parton shower.
%  supplemented by matrix element corrections (MEC) for the hardest
%  emission.

The renormalisation and factorisation scales were set to the geometric
mean of the squared transverse masses of the two outgoing particles in the matrix element,
\(\pTHatPythia = \sqrt{(\pTX[2][1] + m_1^2) (\pTX[2][2] + m_2^2)}\).
The \NNPDF[2.3lo] PDF set~\cite{Ball:2012cx} was used in
the ME generation, the parton shower, and the simulation of the
multi-parton interactions. The A14~\cite{ATL-PHYS-PUB-2014-021}
set of tuned parameters was used. Perturbative uncertainties were estimated
through event weights~\cite{Mrenna:2016sih} that encompass variations
of the scales at which the strong coupling constant is evaluated in
the initial- and final-state shower as well as the PDF uncertainty in
the shower and the non-singular part of the splitting functions.


\paragraph{Additional description:}

The modelling of fragmentation and
hadronisation was based on the Lund string
model~\cite{Andersson:1983ia,Sjostrand:1984ic}. To populate the
inclusive jet \pT spectrum efficiently, the sample used a biased
phase-space sampling which was compensated for by a continuously decreasing
weight for the event. Specifically, events at a scale
\pTHatPythia scale were oversampled by a factor of
\((\pTHatPythia/\SI{10}{\GeV})^4\).


\section[Herwig 7.1]{\HERWIG[7.1]}
\label{subsec:jets-herwig}

The descriptions below correspond to the samples in \cref{tab:mj_herwig}.

\begin{table}[!htbp]
  \caption{Multijet samples produced with \HERWIG[7].}%
  \label{tab:mj_herwig}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364922--364929 & angular ordering in shower \HERWIG[7] \\
    364902--364909 & dipole shower \HERWIG[7] \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Multijet production at next-to-leading order (NLO) was generated using \HERWIG[7.1.3]~\cite{Bellm:2017jjp}.
The renormalisation and factorisation scales were set to the \pT of the leading jet. The
\MMHT[nlo]~\cite{Harland-Lang:2014zoa} PDF set was used for the matrix element calculation.
Two sets of samples were generated, where one makes use of the default parton shower with angular ordering,
and the other uses the dipole shower as an alternative. The description of
hadronisation was based on the cluster model~\cite{Winter:2003tt} for both of these samples.
Two different samples with the same matrix elements and hadronisation allow the effects of using different
parton shower models to be investigated. These samples include variations from the hard scattering and shower.


\section[Powheg+Pythia8]{\POWPY[8]}
\label{subsec:jets-powheg}

The descriptions below correspond to the samples in \cref{tab:mj_powheg}.

\begin{table}[!htbp]
  \caption{Multijet samples produced with \POWHEGBOX[v2].}%
  \label{tab:mj_powheg}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    361281--361289 & \POWPY[8] \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Alternative samples of multijet production at NLO accuracy were produced with \POWHEGBOX[v2]~\cite{Nason:2004rx, Frixione:2007vw}
interfaced to \PYTHIA[8]. These were generated with the dijet process as implemented in \POWHEGBOX[v2]~\cite{Alioli:2010xd}.
The \pT of the underlying Born configuration was taken as the renormalisation and factorisation scales
and the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function (PDF) was used. \PYTHIA with the A14 tune and the
\NNPDF[2.3lo]~\cite{Ball:2012cx} PDF was used for the shower and multi-parton interactions.
These samples included per-event weight variations for different perturbative scales in the matrix element,
different parton distribution functions and their uncertainties, and the \PYTHIA perturbative
shower uncertainties.


\section[Sherpa 2.2]{\SHERPA[2.2]}
\label{subsec:jets-sherpa}

The descriptions below correspond to the samples in \cref{tab:mj_sherpa}.

\begin{table}[!htbp]
  \caption{Multijet samples produced with \SHERPA.}%
  \label{tab:mj_sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    364677--364685 & \SHERPA AHADIC \\
    364686--364694 & \SHERPA Lund \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Multijet production samples were also generated using the \SHERPA[2.2.5]~\cite{Bothmann:2019yzt} generator.
The matrix element calculation was included for the \(2\rightarrow2\) process at leading order, and the default \SHERPA parton
shower~\cite{Schumann:2007mg} based on Catani--Seymour dipole factorisation was used for the showering with \pT
ordering, using the \CT[14nnlo] PDF set~\cite{Dulat:2015mca}.
The first of these samples made use of the dedicated \SHERPA AHADIC model for hadronisation~\cite{Winter:2003tt},
based on cluster fragmentation ideas. A second sample was generated with the same configuration but using the \SHERPA interface to
the Lund string fragmentation model of \PYTHIA[6]~\cite{Sjostrand:2006za} and its decay tables.
These two sets of samples were used to evaluate uncertainties stemming from the hadronisation modelling.

% need to comment on the slicing of these samples. JZ1 to JZ4 are JZW filtered to improve statistics for and an equal number of simulated events, while slices JZ9-JZ12 have been combined into a single JZ9 plus slice.


==> template/MC_snippets/Pileup.tex <==
\chapter{\Pileup overlay}

\paragraph{Description:}

The effect of multiple interactions in the same and neighbouring bunch
crossings (\pileup) was modelled by overlaying the simulated hard-scattering event with
inelastic proton--proton (\(pp\)) events generated with \PYTHIA[8.186]~\cite{Sjostrand:2007gs}
using the \NNPDF[2.3lo] set of parton distribution functions (PDF)~\cite{Ball:2012cx} and the
A3 set of tuned parameters~\cite{ATL-PHYS-PUB-2016-017}.

\paragraph{Optional description:}

The Monte Carlo (MC) events were weighted to reproduce the
distribution of the average number of interactions per bunch crossing
(\(\left<\mu \right>\)) observed in the data. The \(\left<\mu \right>\)
value in data was rescaled by a factor of \(1.03\pm 0.04\) to improve
agreement between data and simulation in the visible inelastic
proton--proton (\(pp\)) cross-section~\cite{STDM-2015-05}.



==> template/MC_snippets/RT.tex <==
\chapter{Rare top-quark processes}
%\label{sec:RT}

This chapter describes the samples used for rare top-quark processes.
\Cref{subsec:ttH} describes the \ttH\ samples.
\Cref{subsec:ttV} describes the \ttV\ (\(V=W/Z\)) samples.
\Cref{subsec:ttgamma} describes the \ttgamma\ samples.
\Cref{subsec:tHq} describes the \tH\ samples.
\Cref{subsec:tZq} describes the \tZq\ samples.
\Cref{subsec:tWZ} describes the \tWZ\ samples.
%\tgamma\ samples are described in \cref{subsec:tgamma}.
Finally, \cref{subsec:tttt} describes the \tttt\ samples.

\input{ttH}
\input{ttV}
\input{ttgamma}
\input{tHq}
\input{tHW}
\input{tZq}
\input{tWZ}
%\input{tgamma}
\input{tttt}


==> template/MC_snippets/TQ.tex <==
% !TEX root = MC_snippets.tex

\chapter{Top-quark processes}
%\label{sec:TQ}

This chapter describes the samples used for top-quark processes.
The \ttbar\ samples are described in \cref{subsec:ttbar}.
Single-top samples are described in \cref{subsec:tW} for \(tW\) associated production,
in \cref{subsec:tchan} for \(t\)-channel production,
and in \cref{subsec:schan} for \(s\)-channel production.
Finally, \ttHF\ samples are described in \cref{subsec:ttHF}.

\input{ttbar}
\input{sgtop}
\input{ttHF}


==> template/MC_snippets/sgtop.tex <==
% !TEX root = MC_snippets.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tW                     %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Single-top \texorpdfstring{\(tW\)}{tW} associated production}
\label{subsec:tW}

This section describes the MC samples used for the modelling of single-top \(tW\) associated production.
\Cref{subsubsec:tW_PP8} describes the \POWPY[8] samples -- both for the diagram removal (DR) set-ups,
which are used for the nominal prediction as well as uncertainties due to additional radiation and PDFs,
and for the diagram subtraction (DS) set-ups, which are used for the uncertainty due to the treatment
of the overlap with \ttbar production.
\Cref{subsubsec:tW_PH7} describes the \POWHER[7] samples used for the uncertainty
due to parton showering and hadronisation modelling, and \cref{subsubsec:tW_aMCP8} describes the
\MGNLOPY[8] samples used for the uncertainty due to the choice of matching scheme.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGsgtopXsec}.

\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:tW_PP8}

\paragraph{Samples}
%\label{par:tW_PP8_samples}

\Cref{tab:tW_PP8} gives the DSIDs of the \(tW\) \POWPY[8] samples, for both the DR and DS schemes.
Single-top and single-anti-top (\(tW^-\) and \(\bar{t}W^+\)) events were generated in different samples.
The dileptonic samples overlap with the inclusive ones.

\begin{table}[htbp]
  \caption{Single-top \(tW\) associated production samples produced with \POWPY[8].}%
  \label{tab:tW_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    410646 & \(tW^-\) (DR) inclusive \\
    410647 & \(\bar{t}W^+\) (DR) inclusive \\
    410648 & \(tW^-\) (DR) dileptonic \\
    410649 & \(\bar{t}W^+\) (DR) dileptonic \\
    \midrule
    410654 & \(tW^-\) (DS) inclusive \\
    410655 & \(\bar{t}W^+\) (DS) inclusive \\
    410656 & \(tW^-\) (DS) dileptonic \\
    410657 & \(\bar{t}W^+\) (DS) dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The associated production of top quarks with \(W\) bosons (\(tW\)) was
modelled by the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in QCD using the five-flavour scheme and the
\NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa}.
The diagram removal scheme~\cite{Frixione:2008yi} was used to
remove interference and overlap with \ttbar production.
The related uncertainty was estimated by comparison with an alternative sample
generated using the diagram subtraction scheme~\cite{Frixione:2008yi,ATL-PHYS-PUB-2016-020}.\footnote{Analyses which do not use this approach
should obviously not use this sentence in their description.}
The events were interfaced to \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] set of
PDFs~\cite{Ball:2012cx}.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

Single-top \(tW\) associated production was modelled using the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas\ in the five-flavour
scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton
distribution function~(PDF) set.  The functional form of the
renormalisation and factorisation scales was set to the default scale,
which is equal to the top-quark mass (\(\mtop = \SI{172.5}{\GeV}\)).
The diagram removal scheme~\cite{Frixione:2008yi} was employed to handle the interference
with \ttbar production~\cite{ATL-PHYS-PUB-2016-020}.  The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.  The
decays of bottom and charm hadrons were simulated using the
\EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The inclusive cross-section was corrected to the theory prediction
calculated at NLO in QCD with NNLL soft-gluon
corrections~\cite{Kidonakis:2010ux,Kidonakis:2013zqa}.  For proton--proton
collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this
cross-section corresponds to \(\sigma(tW)_{\text{NLO+NNLL}} = 71.7 \pm 3.8\,\si{\pb}\),
using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).  The uncertainty in
the cross-section due to the PDF was calculated using the \MSTW[nnlo] 90\%
CL~\cite{Martin:2009iq,Martin:2009bu} PDF set, and was added in
quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

The nominal \POWPY[8] sample was compared with an alternative
sample generated using the diagram subtraction
scheme~\cite{Frixione:2008yi,ATL-PHYS-PUB-2016-020} to estimate the
uncertainty arising from the interference with \ttbar production.

To evaluate the PDF uncertainties for the nominal PDF, the 100
variations for \NNPDF[3.0nlo] were taken into account.
In addition, the central value of this PDF was compared with the
central values of the \CT[14nnlo]~\cite{Dulat:2015mca} and
\MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7]{\POWHER[7]}
\label{subsubsec:tW_PH7}

\paragraph{Samples}
%\label{par:tW_PH7_samples}

\Cref{tab:tW_PH7} gives the DSIDs of the \(tW\) \POWHER[7] DR samples.
Single-top and single-anti-top (\(tW^-\) and \(\bar{t}W^+\)) events were generated in different samples.
The dileptonic samples overlap with the inclusive ones.

\begin{table}[htbp]
  \caption{Single-top \(tW\) associated production samples produced with \POWHER[7].}%
  \label{tab:tW_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    411036 & \(tW^-\) (DR) inclusive \\
    411037 & \(\bar{t}W^+\) (DR) inclusive \\
    411038 & \(tW^-\) (DR) dileptonic \\
    411039 & \(\bar{t}W^+\) (DR) dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The uncertainty due to the parton shower and hadronisation model was
evaluated by comparing the nominal sample of events with a sample where
events generated with the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator were interfaced to
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \(tW\) sample with another sample produced with the
\POWHEGBOX[v2]~\cite{Re:2010bp,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp},
using the H7UE set of tuned parameters~\cite{Bellm:2015jjp} and the
\MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the
strong coupling constant \alphas in the five-flavour scheme with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to
the default scale, which is equal to the top-quark mass.  The diagram removal
scheme~\cite{Frixione:2008yi} was employed to handle the interference
with \ttbar production~\cite{ATL-PHYS-PUB-2016-020}.  The decays of bottom
and charm hadrons are simulated using the \EVTGEN[1.6.0]
program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tW_aMCP8}

\paragraph{Samples}
%\label{par:tW_aMCP8_samples}

\Cref{tab:tW_aMCP8} gives the DSIDs of the \(tW\) \MGNLOPY[8] samples.
The dileptonic sample overlaps with the inclusive one.

\begin{table}[htbp]
  \caption{Single-top \(tW\) associated production samples produced with \MGNLOPY[8].}%
  \label{tab:tW_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    412002 & \(tW\) inclusive \\
    412003 & \(tW\) dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, the nominal \(tW\) sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO in QCD using the five-flavour
scheme and the \NNPDF[2.3nlo]~\cite{Ball:2014uwa} PDF set. The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14
set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]
PDF.


\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme, the nominal \(tW\) sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the five-flavour scheme, using the \NNPDF[2.3nlo]~\cite{Ball:2014uwa} PDF set.
The functional form of the renormalisation and factorisation scale was set to the default scale, which is equal to the top-quark mass.
The parton-shower starting scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
The diagram removal scheme~\cite{Frixione:2008yi} was employed to handle the interference with \ttbar production~\cite{ATL-PHYS-PUB-2016-020}.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              t-channel              %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Single-top \texorpdfstring{\(t\)}{t}-channel production}
\label{subsec:tchan}

This section describes the MC samples used for the modelling of single-top \(t\)-channel production.
\Cref{subsubsec:tchan_PP8} describes the \POWPY[8] samples used for the nominal prediction
and for the uncertainty from additional radiation and due to PDFs.
\Cref{subsubsec:tchan_PH7} describes the \POWHER[7] samples used for the uncertainty due to the choice of parton shower and hadronisation model,
and \cref{subsubsec:tchan_aMCP8} describes the \MGNLOPY[8] samples used for the uncertainty due to the choice of matching scheme.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGsgtopXsec}.


\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:tchan_PP8}

\paragraph{Samples}
%\label{par:tchan_PP8_samples}

\Cref{tab:tchan_PP8} gives the DSIDs of the \(t\)-channel \POWPY[8] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[!htbp]
  \caption{Single-top \(t\)-channel event samples produced with \POWPY[8].}%
  \label{tab:tchan_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    410658 & \(t\)-channel \(t\) leptonic \\
    410659 & \(t\)-channel \(\bar{t}\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Single-top \(t\)-channel production was modelled using the
\POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in QCD using the four-flavour scheme and the
corresponding \NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa}.  The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] set of
PDFs~\cite{Ball:2012cx}.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

Single-top \(t\)-channel production was modelled using the
\POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading-order~(NLO)
accuracy in the strong coupling constant \alphas\ in the four-flavour
scheme with the corresponding \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton
distribution function~(PDF) set.  The functional form of the
renormalisation and factorisation scales was set to
\(\sqrt{m_b^2 + \pTX[2][b]}\) following the
recommendation of Ref.~\cite{Frederix:2012dh}. Top quarks were decayed at
LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve
all spin correlations.  The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14
tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the
\EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The inclusive cross-section was corrected to the theory prediction calculated at NLO in QCD with
\HATHOR[2.1]~\cite{Aliev:2010zk,Kant:2014oha}.
For proton--proton collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this cross-section corresponds to
\(\sigma(t,t\text{-chan})_\text{NLO}= 136.02^{+5.40}_{-4.57}\)\,pb (\(\sigma(\bar{t},t\text{-chan})_\text{NLO}=80.95^{+4.06}_{-3.61}\)\,pb)
for single-top (single-anti-top) production, using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).
The uncertainties in the cross-section due to the PDF and \alphas were calculated using the \PDFforLHC prescription~\cite{Butterworth:2015oua}
with the \MSTW[nlo] 68\% CL~\cite{Martin:2009iq,Martin:2009bu}, \CT[10nlo]~\cite{Lai:2010vv}
and \NNPDF[2.3nlo]~\cite{Ball:2012cx} PDF sets,
and were added in quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

To evaluate the PDF uncertainties for the nominal PDF, the 100 variations for \NNPDF[3.0nlo] were taken into account.
In addition, the central value of this PDF was compared with the central values of the \CT[14nnlo]~\cite{Dulat:2015mca}
and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7]{\POWHER[7]}
\label{subsubsec:tchan_PH7}

\paragraph{Samples}
%\label{par:tchan_PH7_samples}

\Cref{tab:tchan_PH7} gives the DSIDs of the \(t\)-channel \POWHER[7] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[htbp]
  \caption{Single-top \(t\)-channel event samples produced with \POWHER[7].}%
  \label{tab:tchan_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    411032 & \(t\)-channel \(\bar t\) leptonic \\
    411033 & \(t\)-channel \(t\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The uncertainty due to the parton shower and hadronisation model was
evaluated by comparing the nominal sample of events with a sample where
the events generated with the
\POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator were interfaced to
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set
\cite{Harland-Lang:2014zoa}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated by comparing the nominal sample
with another sample produced with the \POWHEGBOX[v2]~\cite{Frederix:2012dh,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the four-flavour scheme with the corresponding \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to \(\sqrt{m_b^2 + \pTX[2][b]}\)
following the recommendation of Ref.~\cite{Frederix:2012dh}.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tchan_aMCP8}

\paragraph{Samples}
%\label{par:tchan_aMCP8_samples}

\Cref{tab:tchan_aMCP8} gives the DSIDs of the \(t\)-channel \MGNLOPY[8] samples.

\begin{table}[htbp]
  \caption{Single-top \(t\)-channel event samples produced with \MGNLOPY[8].}%
  \label{tab:tchan_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    412004 & \(t\)-channel leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO in QCD using the five-flavour
scheme and the \NNPDF[2.3nlo]~\cite{Ball:2014uwa} PDF set. The events were
interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14
set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.


\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the four-flavour scheme, using the corresponding \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The functional form of the renormalisation and factorisation scales was set to \(\sqrt{m_b^2 + \pTX[2][b]}\)
following the recommendation of Ref.~\cite{Frederix:2012dh}.
The parton-shower starting scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              s-channel              %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Single-top \texorpdfstring{\(s\)}{s}-channel production}
\label{subsec:schan}

This section describes the MC samples used for the modelling of single-top \(s\)-channel production.
\Cref{subsubsec:schan_PP8} describes the \POWPY[8] samples used for the nominal prediction
and for the uncertainty from additional radiation and due to PDFs.
\Cref{subsubsec:schan_PH7} describes the \POWHER[7] samples used for the uncertainty due to the parton shower and hadronisation model,
and \cref{subsubsec:schan_aMCP8} describes the \MGNLOPY[8] samples used for the uncertainty due to the choice of matching scheme.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGsgtopXsec}.

\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:schan_PP8}

\paragraph{Samples}
%\label{par:schan_PP8_samples}

\Cref{tab:schan_PP8} gives the DSIDs of the \(s\)-channel \POWPY[8] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[htbp]
  \caption{Single-top \(s\)-channel event samples produced with \POWPY[8].}%
  \label{tab:schan_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    410644 & \(s\)-channel \(t\) leptonic \\
    410645 & \(s\)-channel \(\bar{t}\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Single-top \(s\)-channel production was modelled using the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in QCD in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) set.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo] PDF set.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

Single-top \(s\)-channel production was modelled using the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas in the
five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) set.
The functional form of the renormalisation and factorisation scales was set to the default scale, which was equal to the top-quark mass.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The inclusive cross-section was corrected to the theory prediction calculated at NLO in QCD with
\HATHOR[2.1]~\cite{Aliev:2010zk,Kant:2014oha}.
For proton--proton collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this cross-section corresponds to
\(\sigma(t,s\text{-chan})_{\text{NLO}} = 6.35^{+0.23}_{-0.20}\,\si{\pb}\)
(\(\sigma(\bar{t},s\text{-chan})_{\text{NLO}} = 3.97^{+0.19}_{-0.17}\,\si{\pb}\))
for single-top (single-anti-top) production, using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).
The uncertainties in the cross-section due to the PDF and \alphas were calculated using the \PDFforLHC prescription~\cite{Butterworth:2015oua}
with the \MSTW[nlo] 68\% CL~\cite{Martin:2009iq,Martin:2009bu}, \CT[10nlo]~\cite{Lai:2010vv} and \NNPDF[2.3nlo]~\cite{Ball:2012cx} PDF sets,
and were added in quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

To evaluate the PDF uncertainties for the nominal PDF, the 100 variations for \NNPDF[3.0nlo] were taken into account.
In addition, the central value of this PDF was compared with the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7]{\POWHER[7]}
\label{subsubsec:schan_PH7}

\paragraph{Samples}
%\label{par:schan_PH7_samples}

\Cref{tab:schan_PH7} gives the DSIDs of the \(s\)-channel \POWHER[7] samples.
Single-top and single-anti-top events were generated in distinct samples.

\begin{table}[htbp]
  \caption{Single-top \(s\)-channel event samples produced with \POWHER[7].}%
  \label{tab:schan_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    411034 & \(s\)-channel \(t\) leptonic \\
    411035 & \(s\)-channel \(\bar{t}\) leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated by comparing the nominal sample
with another sample produced with the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO in the strong coupling constant \alphas in the five-flavour scheme using the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
Events in the latter sample were interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated by comparing the nominal sample
with another sample produced with the \POWHEGBOX[v2]~\cite{Alioli:2009je,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set \cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to the default scale, which is equal to the top-quark mass.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:schan_aMCP8}

\paragraph{Samples}
%\label{par:schan_aMCP8_samples}

\Cref{tab:schan_aMCP8} gives the DSIDs of the \(s\)-channel \MGNLOPY[8] samples.

\begin{table}[htbp]
  \caption{Single-top \(s\)-channel event samples produced with \MGNLOPY[8].}%
  \label{tab:schan_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    412005 & \(s\)-channel leptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

%% the MG5_aMC@NLO version was double checked in the tag collector
To assess the uncertainty due to the choice of matching scheme, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO in the strong coupling constant \alphas in the five-flavour scheme,
using the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF set.


\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme, the nominal sample was compared with a sample generated
with the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to the default scale, which is equal to the top-quark mass.
The parton-shower starting scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo] PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/sherpa_scale_pdf.tex <==
Uncertainties from missing higher orders were
evaluated~\cite{Bothmann:2016nao} using seven variations of the QCD
factorisation and renormalisation scales in the matrix elements by
factors of \(0.5\) and \(2\), avoiding variations in opposite directions.

Uncertainties in the nominal PDF set were evaluated using 100 replica
variations. Additionally, the results were cross-checked using the
central values of the \CT[14nnlo]~\cite{Dulat:2015mca} and
\MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets. The effect of the uncertainty
in the strong coupling constant \(\alphas\) was assessed by variations of \(\pm 0.001\).






==> template/MC_snippets/tHW.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tHW                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tHW]{\tHW}
\label{subsec:tHW}

This section describes the MC samples used for the modelling of \tHW\ production.
\Cref{subsubsec:tHW_aMCP8} describes the \MGNLOPY[8] samples.

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tHW_aMCP8}

\paragraph{Samples}

The descriptions below correspond to the samples in \cref{tab:tHW_aMCP8}.

\begin{table}
  \caption{Nominal \tHW\ samples produced with \MGNLOPY[8].}%
  \label{tab:tHW_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID & Description \\
    \midrule
    346486 & \tHW\, \Hgg\ \\
    346511 & \tHW\, \Hllll \\
    346678 & \tHW\, \(H\rightarrow\) inclusive, UFO model \\
    346759 & \tHW\, \Hgg{}, UFO model \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The \tHW{} production is modelled using the \MGNLO[2.6.2]~\cite{Alwall:2014hca} generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The overlap with the \ttH{} production is removed using the diagram removal scheme~\cite{Frixione:2008yi,Demartin:2016axk}. The events are interfaced with \PYTHIA[8.235]~\cite{Sjostrand:2014zea} using the A14 parameter set~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons are simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The \tHW{} samples were simulated using the \MGNLO[2.6.2]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The events were interfaced with
\PYTHIA[8.235]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The top quark was decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations,
whereas the Higgs boson was decayed by \PYTHIA in the parton shower. The samples
were generated in the five-flavour scheme.
The functional form of the renormalisation and factorisation scales was set to the
default scale \(0.5\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\), where the sum runs over
all the particles generated from the matrix element calculation.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/tHq.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tH                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tHq]{\tHq}
\label{subsec:tHq}

This section describes the MC samples used for the modelling of \tH\ production.
\Cref{subsubsec:tHq_aMCP8} describes the \MGNLOPY[8] samples,

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tHq_aMCP8}

\paragraph{Samples}
%\label{par:tHq_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tHq_aMCP8}.

\begin{table}[htbp]
  \caption{Nominal \tH\ samples produced with \MGNLOPY[8].}%
  \label{tab:tHq_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    346188 & \tHq\, \Hgg\, four flavour \\
    346229 & \tHq\, \Hbb\, four flavour \\
    346230 & \tHq\, \Htautau/\HZZ/\HWW\, four flavour \\
    346414 & \tHq\, \Hllll, four flavour \\
    \midrule
    346676 & \tHq\, \(H\rightarrow\) inclusive, four flavour, UFO model \\
    346677 & \tHq\, \Hgg, four flavour, UFO model \\
    346799 & \tHq\, \Htautau/\HZZ/\HWW\ + Nleptons=2 filter, four flavour, UFO model \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Exceptions:}
If and only if you are using the UFO model sample: the correct version is \MGNLO[2.6.2].

\paragraph{Short description:}

The production of \tHq events was modelled using the \MGNLO[2.6.0]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The \tHq samples were simulated using the \MGNLO[2.6.0]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The top quark was decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations,
whereas the Higgs boson was decayed by \PYTHIA in the parton shower. The samples
were generated in the four-flavour scheme.
The functional form of the renormalisation and factorisation scales was set to the
default scale \(0.5\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\), where the sum runs over
all the particles generated from the matrix element calculation.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/tWZ.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tWZ                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tWZ]{\tWZ}
\label{subsec:tWZ}

This section describes the MC samples used for the modelling of \tWZ\ production.
\Cref{subsubsec:tWZ_aMCP8} describes the \MGNLOPY[8] samples,

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tWZ_aMCP8}

\paragraph{Samples}
%\label{par:tWZ_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tWZ_aMCP8}.

\begin{table}[htbp]
  \caption{Nominal \tWZ\ samples produced with \MGNLOPY[8].}%
  \label{tab:tWZ_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410408 & \tWZ\, DR1 \\
    410409 & \tWZ\, DR2 \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \tWZ\ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.212]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The production of \tWZ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with
\PYTHIA[8.212]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The top quark and the \(Z\) boson were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations.
While the top quark was allowed to decay inclusively, the \(Z\) boson decay was restricted to a pair of charged leptons.
The five-flavour scheme was used, where all the quark masses are set to zero, except the top quark.
The renormalisation and factorisation scales were set to the top-quark mass.
The diagram removal scheme described in Ref.~\cite{Frixione:2008yi} was employed to handle the interference
between \tWZ and \ttZ, and was applied to the \tWZ sample.
A sample with the alternative scheme described in Ref.~\cite{Demartin:2016axk} was produced to assess the associated systematic uncertainty.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.



==> template/MC_snippets/tZq.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tZq                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tZq]{\tZq}
\label{subsec:tZq}

This section describes the MC samples used for the modelling of \tZq production.
\Cref{subsubsec:tZq_aMCP8} describes the \MGNLOPY[8] samples,

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tZq_aMCP8}

\paragraph{Samples}
%\label{par:tZq_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tZq_aMCP8,tab:tZq_aMCP8_addRad}.

\begin{table}[htbp]
  \caption{Nominal \tZq samples produced with \MGNLOPY[8].}%
  \label{tab:tZq_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412063 & \tZq \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\tZq samples produced with \MGNLOPY[8] used to estimate initial-state radiation systematic uncertainties.}%
  \label{tab:tZq_aMCP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412065 & \tZq, A14Var3c up \\
    410064 & \tZq, A14Var3c down \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \tZq events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.

The uncertainty due to initial-state radiation (ISR) was estimated by comparing the nominal \tZq sample with two additional samples,
which had the same settings as the nominal one, but employed the Var3c up and down variations of the A14 tune.


\paragraph{Long description:}

The \tZq sample was simulated using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF). The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021}
and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. Off-resonance events away from the \(Z\) mass peak were included.
The top quark was decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin correlations.
The four-flavour scheme was used, where all the quark masses are set to zero, except for the top and bottom quarks.
Following the discussion in Ref.~\cite{Frederix:2012dh}, the functional form of the renormalisation and factorisation scales
was set to \(4\sqrt{m_b^2+\pTX[2][b]}\), where the \(b\)-quark was the one produced by a gluon splitting in the event.
The decays of bottom and charm hadrons were simulated using the \EVTGEN program~\cite{Lange:2001uf}.

The \tZq total cross-section, calculated at next-to-leading order (NLO) using \MGNLO[2.3.3] with the \NNPDF[3.0nlo] PDF set,
is \(\SI{800}{\fb}\), with an uncertainty of \(^{+6.1}_{-7.4}\)\%. The uncertainty was computed by varying the renormalisation and
factorisation scales by a factor of two and by a factor of 0.5.

The uncertainty due to initial-state radiation (ISR) was estimated by comparing the nominal \tZq sample with two additional samples,
which have the same settings as the nominal one, but employed the Var3c up or down variation of the A14 tune, which
corresponds to the variation of \alphas for ISR in the A14 tune.

To evaluate the effect of renormalisation and factorisation scale uncertainties, the two scales were varied simultaneously by factors 2.0 and 0.5.
To evaluate the PDF uncertainties for the nominal PDF, the 100 variations for \NNPDF[2.3lo] were taken into account.


==> template/MC_snippets/tgamma.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tgamma                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[tgamma production]{\tgamma production}
\label{subsec:tgamma}

This section describes the MC samples used for the modelling of \tgamma production.
For now, it will be empty since the sample is still in production.


==> template/MC_snippets/top_isrfsr_powpy_long.tex <==
The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal \ttbar sample with two additional
samples~\cite{ATL-PHYS-PUB-2017-007}.  To simulate higher parton
radiation, the factorisation and renormalisation scales were reduced by
a factor of 0.5 while simultaneously increasing the \hdamp value to
3.0\,\mtop and using the Var3c up variation from the A14 tune. For
lower parton radiation, \muR and \muF were increased by a factor of two
while keeping the \hdamp value set to 1.5\,\mtop and using the Var3c down
variation in the parton shower.  The Var3c A14 tune
variation~\cite{ATL-PHYS-PUB-2014-021} largely corresponds to the variation of
\alphas for ISR in the A14 tune.
The impact of final-state radiation (FSR) was evaluated by
varying the renormalisation scale for emissions from the
parton shower up and down by a factor of two.


==> template/MC_snippets/top_isrfsr_powpy_short.tex <==
The uncertainty due to initial-state radiation (ISR) was estimated by
simultaneously varying the \hdamp parameter and the \muR and
\muF scales, and choosing the Var3c up/down variants of the A14 tune
as described in Ref.~\cite{ATL-PHYS-PUB-2017-007}. The impact of
final-state radiation (FSR) was evaluated by varying the renormalisation scale
for emissions from the parton shower up or down by a factor two.


==> template/MC_snippets/ttH.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttH                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttH production]{\ttH}
\label{subsec:ttH}

\subsection[Powheg+Pythia8]{\POWPY[8]}
%\label{subsubsec:ttH_PP8}

Nominal \(t\bar{t}H\) samples are produced with \POWPY[8].
The \hdamp value is set to \(\SI{352.5}{\GeV} = 3/4 \cdot (\mH+2\mtop)\).

\paragraph{Samples}
%\label{par:ttH_PP8_samples}
\Cref{tab:ttH_PP8} gives the nominal \ttH samples.

\begin{table}[htbp]
  \caption{Nominal \ttH samples produced with \POWPY[8].}%
  \label{tab:ttH_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    346343 & \ttH, \(H\to\) all, \(\ttbar\to\) all-hadronic \\
    346344 & \ttH, \(H\to\) all, \(\ttbar\to\) semileptonic \\
    346345 & \ttH, \(H\to\) all, \(\ttbar\to\) dileptonic \\
    346525 & \ttH, \(H\to \gamma\gamma\), \(\ttbar\to\) all \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttH events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Hartanto:2015uka}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The events were interfaced to \PYTHIA[8.230]~\cite{Sjostrand:2014zea}~using
the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The decays of bottom and charm hadrons
were performed by \EVTGEN[1.6.0]~\cite{Lange:2001uf}.

\paragraph{Long description:}

The production of \ttH events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd,Hartanto:2015uka}
generator, which provided matrix elements at next-to-leading order (NLO) in the strong coupling
constant \alphas in the five-flavour scheme with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set.
The functional form of the renormalisation and factorisation scales was
set to \(\sqrt[3]{m_\text{T}(t)\cdot m_\text{T}(\bar{t}) \cdot m_\text{T}(H)}\).
The events were interfaced to \PYTHIA[8.230]~\cite{Sjostrand:2014zea}
using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The decays of bottom and charm hadrons
were performed by \EVTGEN[1.6.0]~\cite{Lange:2001uf}.

The cross-section was calculated at NLO QCD and NLO EW accuracy using
\MGNLO as reported in Ref.~\cite{deFlorian:2016spz}.
The predicted value at \(\rts = \SI{13}{\TeV}\) is
\(507^{+35}_{-50}\,\si{\fb}\), where the uncertainties were estimated from
variations of \alphas and the renormalisation and factorisation scales.

The uncertainty in the initial-state radiation (ISR) was estimated using the Var3c
up/down variations of the A14 tune. Uncertainties due to missing
higher-order corrections were evaluated through simultaneous variations of the
renormalisation and factorisation scales by factors of
2.0 and 0.5. Uncertainties in the PDFs were evaluated using the 100
variations of the \NNPDF[3.0nlo] set.


\subsection[Powheg+Herwig7]{\POWHER[7]}
%\label{subsubsec:ttH_PH7}

\paragraph{Samples}
%\label{par:ttH_PH7_samples}

\Cref{tab:ttH_PH7} presents alternative \ttH samples.

\begin{table}[htbp]
  \caption{Alternative \ttH \POWHER[7] samples produced to evaluate systematic uncertainties
  due to different MC models for parton showering and hadronisation.}%
  \label{tab:ttH_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    346346 & \ttH, \(H\to\) all, \(\ttbar\to\) all-hadronic \\
    346347 & \ttH, \(H\to\) all, \(\ttbar\to\) semileptonic \\
    346348 & \ttH, \(H\to\) all, \(\ttbar\to\) dileptonic \\
    346526 & \ttH, \(H\to\gamma\gamma\), \(\ttbar\to\) all \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated by showering the nominal hard-scatter events with
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp} using the H7UE set of tuned parameters~\cite{Bellm:2015jjp} and
the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.

\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal sample with another sample produced with
the \POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the
H7UE set of tuned parameters~\cite{Bellm:2015jjp} and
the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was
set to \(\sqrt[3]{m_\text{T}(t)\cdot m_\text{T}(\bar{t}) \cdot m_\text{T}(H)}\).
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


==> template/MC_snippets/ttHF.tex <==
% !TEX root = MC_snippets.tex

\section[\ttHF]{\ttHF}
\label{subsec:ttHF}

In the following subsections, the set-ups of the current baseline samples for the production of \ttbar quark pairs in association with
\(b\)-quarks (\ttHF) are described. NLO predictions with massive \(b\)-quarks in the matrix element and matched to parton shower
programs are available within the \SHERPAOL, \MGNLO and, more recently, \POWHEGBOX frameworks.

\subsection[Sherpa]{\SHERPA}
%\label{subsubsec:ttHF_sherpa}
The descriptions below refer to the \SHERPA[2.2.1] samples.
Details of the set-up are given in Ref.~\cite{ATL-PHYS-PUB-2016-016} and reported below.

\paragraph{Samples}
%\label{par:ttHF_sherpa_samples}

The descriptions below correspond to the samples in \cref{tab:ttHF_Sh}.

\begin{table}[htbp]
  \caption{Nominal \ttbar+HF samples produced with \SHERPA.
      Variation samples are not explicitly listed.}%
  \label{tab:ttHF_Sh}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410323--4 & \ttbar single lepton \\
    410325 & \ttbar dilepton \\
    410369 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples for \ttHF processes were produced with the \SHERPA[2.2.1]~\cite{Bothmann:2019yzt} generator,
using the MEPS@NLO prescription~\cite{Hoeche:2012yf} and interfaced with \OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}
to provide the virtual corrections for matrix elements at NLO accuracy.
The four-flavour scheme is used with the \(b\)-quark mass set to \SI{4.75}{\GeV}.
The renormalisation scale \muR has the functional form
\(\sqrt[4]{m_\text{T}(t) \cdot m_{\text{T}}(\bar{t}) \cdot m_{\text{T}}(b) \cdot m_{\text{T}}(\bar{b})}\). The
factorisation scale \muF was set to \(\HT/2\), where \HT is the transverse-mass sum of the
partons in the matrix element, and this value was also the resummation scale \muQ of the parton shower.
The \CT[10nlo] PDF set was used in conjunction with a dedicated PS tune developed by the \SHERPA authors.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
%\label{subsubsec:ttHF_aMCP8}
In the following, set-ups are described for \PYTHIA only.
Details of the set-up are given in Ref.~\cite{ATL-PHYS-PUB-2016-016} and reported below.

\paragraph{Samples}
%\label{par:ttHF_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttHF_amc}.

\begin{table}[htbp]
  \caption{Nominal \ttbar+HF samples produced with \MGNLOPY[8].}%
  \label{tab:ttHF_amc}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410265 & \ttbar non-all-hadronic \\
    410266 & \ttbar dileptonic \\
    410267 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples for \ttHF processes were produced with the \MGNLO generator
with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set. It was interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea},
using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF.
The four-flavour scheme was used with the \(b\)-quark mass set to \SI{4.75}{\GeV}.
The renormalisation scale \muR has the functional form
\(\sqrt[4]{m_\text{T}(t) \cdot m_\text{T}(\bar{t}) \cdot m_\text{T}(b) \cdot m_\text{T}(\bar{b})}\). The
factorisation scale \muF was set to \(\HT/2\), where \HT is the transverse-mass sum of the partons in the matrix
element.
The resummation scale \muQ has the form \(\muQ = f_\text{Q} \sqrt{\hat{s}}\), where
the prefactor \(f_\text{Q}\) is an external parameter randomly distributed in the
range \([f^\text{min}_\text{Q}\), \(f^\text{max}_\text{Q}]=[0.1,0.25]\).


\subsection[PowhegBoxRes+Pythia8]{\POWHEGBOXRES+\PYTHIA[8]}
%\label{subsubsec:ttHF_PP8}
In the following, set-ups are described for \PYTHIA[8] only.

\paragraph{Samples}
%\label{par:ttHF_PP8_samples}
The descriptions below correspond to the samples in \cref{tab:ttHF_pp8}.

\begin{table}[htbp]
  \caption{Nominal \ttbar+HF samples produced with \POWHEGBOXRES+\PYTHIA[8].}%
  \label{tab:ttHF_pp8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    411179--80 & \ttbar non-all-hadronic \\
    411178    & \ttbar dileptonic \\
    411275    & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Samples for \ttHF processes were produced with the \POWHEGBOXRES~\cite{Jezo:2018yaf}
generator and \OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg}, using a pre-release
of the implementation of this process in \POWHEGBOXRES provided by the authors~\cite{ttbbPowheg},
with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set. It was interfaced with \PYTHIA[8.240]~\cite{Sjostrand:2014zea},
using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] PDF set.
The four-flavour scheme was used with the \(b\)-quark mass set to \SI{4.95}{\GeV}.
The factorisation scale was set to \(0.5\times\Sigma_{i=t,\bar{t},b,\bar{b},j}m_{\mathrm{T},i}\),
the renormalisation scale was set to \(\sqrt[4]{m_{\text{T}}(t)\cdot m_{\text{T}}(\bar{t})\cdot m_{\text{T}}(b)\cdot m_{\text{T}}(\bar{b})}\),
and the \hdamp parameter was set to \(0.5\times\Sigma_{i=t,\bar{t},b,\bar{b}}m_{\mathrm{T},i}\).


==> template/MC_snippets/ttV.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttV                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttV production]{\ttV production}
\label{subsec:ttV}

This section describes the MC samples used for the modelling of \ttV (\(V=W/Z\)) production.
\Cref{subsubsec:ttV_aMCP8} describes the \MGNLOPY[8] samples,
and \cref{subsubsec:ttV_sherpa} describes the \SHERPA samples.
(NOTE: this section is not frozen as the \SHERPA samples are likely to be updated and become the nominal samples in the near future.)

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:ttV_aMCP8}

\paragraph{Samples}
%\label{par:ttV_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttV_aMCP8,tab:ttV_aMCP8_addRad}.

\begin{table}[htbp]
  \caption{Nominal \ttV samples produced with \MGNLOPY[8].}%
  \label{tab:ttV_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410155 & \ttW \\
    410156 & \ttZnunu \\
    410157 & \ttZqq \\
    410218 & \ttee, \(m_{\ell\ell} > \SI{5}{\GeV}\) \\
    410219 & \ttmumu, \(m_{\ell\ell} > \SI{5}{\GeV}\) \\
    410220 & \tttautau, \(m_{\ell\ell} > \SI{5}{\GeV}\) \\
    410276 & \ttee, \(m_{\ell\ell} \in \SI[parse-numbers=false]{[1,5]}{\GeV}\)\\
    410277 & \ttmumu, \(m_{\ell\ell} \in \SI[parse-numbers=false]{[1,5]}{\GeV}\)\\
    410278 & \tttautau, \(m_{\ell\ell} \in \SI[parse-numbers=false]{[1,5]}{\GeV}\)\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttV samples produced with \MGNLOPY[8] used to estimate initial-state radiation systematic uncertainties.}%
  \label{tab:ttV_aMCP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410376 & \ttW\ A14Var3c up \\
    410377 & \ttW\ A14Var3c down \\
    410378 & \ttZnunu\ A14Var3c up \\
    410379 & \ttZnunu\ A14Var3c down \\
    410380 & \ttZqq\ A14Var3c up \\
    410381 & \ttZqq\ A14Var3c down \\
    410370 & \ttee\ A14Var3c up \\
    410371 & \ttee\ A14Var3c down \\
    410372 & \ttmumu\ A14Var3c up \\
    410373 & \ttmumu\ A14Var3c down \\
    410374 & \tttautau\ A14Var3c up \\
    410375 & \tttautau\ A14Var3c down \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttV\ events was modelled using the
\MGNLO[2.3.3]~\cite{Alwall:2014hca} generator at NLO with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced to \PYTHIA[8.210]~\cite{Sjostrand:2014zea}
using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The decays of bottom and charm
hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.

The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal event sample with two samples where the Var3c
up/down variations of the A14 tune were employed.


\paragraph{Long description:}

The production of \ttV events was modelled using the \MGNLO[2.3.3]
\cite{Alwall:2014hca} generator, which provided matrix elements at
next-to-leading order~(NLO) in the strong coupling constant \alphas
with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution
function~(PDF). The functional form of the renormalisation and
factorisation scales was set to the default of
\(0.5 \times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\),
where the sum runs over all the particles
generated from the matrix element calculation. Top quarks were decayed
at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to
preserve spin correlations. The events were interfaced with
\PYTHIA[8.210]~\cite{Sjostrand:2014zea} for the parton shower and
hadronisation, using the A14 set of tuned
parameters~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.2.0] program~\cite{Lange:2001uf}.

% Note : The cross-section is supplemented with an off-shell (down to \SI{5}{\GeV}) correction calculated in Ref.~\cite{ATLASPMGttVNLOXsec}.
The cross-sections were calculated at NLO QCD and NLO EW accuracy using
\MGNLO as reported in Ref.~\cite{deFlorian:2016spz}.
In the case of \ttll the cross-section was scaled by
an off-shell correction estimated at one-loop level in \alphas.
(\emph{Optionally:})
The predicted values at \(\rts = \SI{13}{\TeV}\) are \(0.88^{+0.09}_{-0.11}\,\si{\pb}\) and
\(0.60^{+0.08}_{-0.07}\,\si{\pb}\) for \ttZ and \ttW, respectively, where the
uncertainties were estimated from variations of \alphas and the renormalisation and
factorisation scales.

The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal \ttV sample with two additional samples, which
have the same settings as the nominal one, but employed the Var3c up or down
variation of the A14 tune, which corresponds
to the variation of \alphas for initial-state radiation
(ISR) in the A14 tune.

Uncertainties due to missing higher-order corrections were evaluated
by simultaneously varying the renormalisation and factorisation scales
by factors of 2.0 and 0.5. Uncertainties in the PDFs
were evaluated using the 100 replicas of the \NNPDF[3.0nlo] set.


\subsection[Sherpa]{\SHERPA}
\label{subsubsec:ttV_sherpa}

\paragraph{Samples}
%\label{par:ttV_sherpa_samples}

The descriptions below correspond to the samples in \cref{tab:ttV_sherpa}.

\begin{table}[htbp]
  \caption{\ttV samples produced with \SHERPA.}%
  \label{tab:ttV_sherpa}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410142 & \ttll \\
    410143 & \ttZqq, \ttZnunu \\
    410144 & \ttW \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Additional \ttV samples were produced with the
\SHERPA[2.2.0]~\cite{Bothmann:2019yzt} generator at LO accuracy, using
the \MEPSatLO set-up~\cite{Catani:2001cc,Hoeche:2009rj} with up to one
additional parton for the \ttll sample and two additional partons for the
others. A dynamic renormalisation scale was used and is defined
similarly to that of the nominal \ttV samples. The CKKW matching
scale of the additional emissions was set to \SI{30}{\GeV}. The default
\SHERPA[2.2.0] parton shower was used along with the
\NNPDF[3.0nnlo]~\cite{Ball:2014uwa} PDF set.


==> template/MC_snippets/ttbar.tex <==
% !TEX root = MC_snippets.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttbar                  %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttbar production]{\ttbar production}
\label{subsec:ttbar}

This section describes the MC samples used for the modelling of \ttbar production.
\Cref{subsubsec:ttbar_PP8} describes the \POWPY[8] samples,
\cref{subsubsec:ttbar_PH7} describes the \POWHER[7] samples,
\cref{subsubsec:ttbar_aMCP8} describes the \MGNLOPY[8] samples,
and finally \cref{subsubsec:ttbar_sherpa} describes the \SHERPA samples.

The reference cross-section values are extracted from Ref.~\cite{LHCTopWGttbarXsec}.
Studies of MC simulation performance including comparisons with unfolded data
are collected in the PUB notes~\cite{ATL-PHYS-PUB-2018-009,ATL-PHYS-PUB-2017-007,ATL-PHYS-PUB-2016-020}.

\subsection[Powheg+Pythia8]{\POWPY[8]}
\label{subsubsec:ttbar_PP8}

\paragraph{Samples}
%\label{par:ttbar_PP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_PP8,tab:ttbar_PP8_addRad,tab:ttbar_PP8_hdampvar}.

\begin{table}[htbp]
  \caption{Nominal \ttbar samples produced with \POWPY[8].
    The \hdamp\ value is set to 1.5\,\mtop.}%
  \label{tab:ttbar_PP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410470 & \ttbar non-all-hadronic \\
    410471 & \ttbar dileptonic \\
    410472 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWPY[8]
    used to estimate initial-state radiation systematic uncertainties.
    The \hdamp value is set to 3.0\,\mtop.}%
  \label{tab:ttbar_PP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410480 & \ttbar single lepton \\
    410481 & \ttbar all-hadronic \\
    410482 & \ttbar dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWPY[8] with alternative \hdamp values
    which can be used to estimate the uncertainty due to the \POWPY[8] matching scheme.}%
  \label{tab:ttbar_PP8_hdampvar}
  \centering
  \begin{tabular}{l l l l}
    \toprule
    DSID (1.3\,\mtop) & DSID (1.8\,\mtop) & DSID (2.0\,\mtop) & Description \\
    \midrule
    411350 & 411353 & 411356 & \ttbar single lepton \\
    411351 & 411354 & 411357 & \ttbar all-hadronic \\
    411352 & 411355 & 411358 & \ttbar dileptonic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttbar events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator at NLO with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set
and the \hdamp parameter\footnote{The
  \hdamp parameter is a resummation damping factor and one of the
  parameters that controls the matching of \POWHEG matrix elements to
  the parton shower and thus effectively regulates the
  high-\pT radiation against which the \ttbar system recoils.} set
to 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.  The events were interfaced
to \PYTHIA[8.230]~\cite{Sjostrand:2014zea} to model the parton shower,
hadronisation, and underlying event, with parameters set according
to the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and using the \NNPDF[2.3lo]
set of PDFs~\cite{Ball:2012cx}. The decays of bottom and charm hadrons
were performed by \EVTGEN[1.6.0]~\cite{Lange:2001uf}.

\input{top_isrfsr_powpy_short}


\paragraph{Long description:}

The production of \ttbar events was modelled using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas, and the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The \hdamp parameter, which controls the matching in \POWHEG and
effectively regulates the high-\pT radiation against which the
\ttbar system recoils, was set to 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pTX[2]}\).
The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea} for the parton shower and
hadronisation, using the A14 set of tuned
parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]
set of PDFs~\cite{Ball:2012cx}.
The decays of bottom and charm hadrons were simulated using the
\EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The \ttbar sample was normalised to the cross-section prediction at next-to-next-to-leading order (NNLO)
in QCD including the resummation of next-to-next-to-leading logarithmic (NNLL) soft-gluon terms calculated using
\TOPpp[2.0]~\cite{Beneke:2011mq,Cacciari:2011hy,Baernreuther:2012ws,Czakon:2012zr,Czakon:2012pz,Czakon:2013goa,Czakon:2011xx}.
For proton--proton collisions at a centre-of-mass energy of \(\rts = \SI{13}{\TeV}\), this cross-section corresponds to
\(\sigma(\ttbar)_{\text{NNLO+NNLL}} = 832 \pm 51\,\si{\fb}\) using a top-quark mass of \(\mtop = \SI{172.5}{\GeV}\).
The uncertainties in the cross-section due to the PDF and \alphas were calculated using the \PDFforLHC[15] prescription~\cite{Butterworth:2015oua}
with the \MSTW[nnlo]~\cite{Martin:2009iq,Martin:2009bu}, \CT[10nnlo]~\cite{Lai:2010vv,Gao:2013xoa}
and \NNPDF[2.3lo]~\cite{Ball:2012cx} PDF sets in the five-flavour scheme, and were added in quadrature to the effect of the scale uncertainty.

\input{top_isrfsr_powpy_long}

The \NNPDF[3.0lo] replicas were used to evaluate the PDF uncertainties for the nominal PDF.
In addition, the central value of this PDF was compared with the central values of the
\CT[14nnlo]~\cite{Dulat:2015mca} and \MMHT[nnlo]~\cite{Harland-Lang:2014zoa} PDF sets.


\subsection[Powheg+Herwig7.04]{\POWHER[7.04]}
\label{subsubsec:ttbar_PH7}

\paragraph{Samples}
%\label{par:ttbar_PH7_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_PH7}.

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWHER[7].}%
  \label{tab:ttbar_PH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410557 & \ttbar single lepton  \\
    410558 & \ttbar dileptonic  \\
    410559 & \ttbar all-hadronic  \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with another event sample produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator using the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
Events in the latter sample were interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp},
using the H7UE set of tuned parameters~\cite{Bellm:2015jjp} and the
\MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with an event sample also produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the H7UE set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading order~(NLO) in the
strong coupling constant \alphas, and used the \NNPDF[3.0nlo]~\cite{Ball:2014uwa}
parton distribution function~(PDF) and an \hdamp parameter value of \(1.5\,\mtop\)~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pT^2}\).
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[Powheg+Herwig7.13]{\POWHER[7.13]}
%\label{subsubsec:ttbar_PH713}

\paragraph{Samples}
%\label{par:ttbar_PH713_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_PH713}.

\begin{table}[htbp]
  \caption{\ttbar samples produced with \POWHER[7.13].}%
  \label{tab:ttbar_PH713}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    411233 & \ttbar single lepton  \\
    411234 & \ttbar dileptonic  \\
    411316 & \ttbar all-hadronic  \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with another event sample produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator using the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
Events in the latter sample were interfaced with \HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp},
using the \HERWIG[7.1] default set of tuned parameters~\cite{Bellm:2015jjp,Bellm:2017jjp}
and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The impact of using a different parton shower and hadronisation model was evaluated
by comparing the nominal \ttbar sample with an event sample also produced with the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator but interfaced with \HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the
\HERWIG[7.1] default set of tuned parameters~\cite{Bellm:2015jjp,Bellm:2017jjp} and the
\MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
\POWHEGBOX provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas, and used the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) and
an \hdamp parameter value of 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pTX[2]}\).
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:ttbar_aMCP8}

\paragraph{Samples}
%\label{par:ttbar_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_aMCP8}.
\begin{table}[htbp]
  \caption{\ttbar samples produced with \MGNLOPY[8].}%
  \label{tab:ttbar_aMCP8}
  \centering
  \begin{tabular}{l l}
  \toprule
  DSID range & Description \\
  \midrule
  410464 & \ttbar single lepton \\
  410465 & \ttbar dileptonic \\
  410466 & \ttbar all-hadronic \\
  \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, the \POWHEG sample was compared with a sample of events
generated with \MGNLO[2.6.0]~\cite{Alwall:2014hca} interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea}. The \MGNLO calculation used the
\NNPDF[3.0nlo] set of PDFs~\cite{Ball:2014uwa} and \PYTHIA[8] used
the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and
the \NNPDF[2.3lo] set of PDFs~\cite{Ball:2012cx}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

\paragraph{Long description:}

To assess the uncertainty due to the choice of matching scheme,
the \POWHEG sample was compared with a sample generated by
\MGNLOPY[8]. For the calculation of the hard-scattering,
\MGNLO[2.6.0]~\cite{Alwall:2014hca} with the \NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set was
used. The events were interfaced with
\PYTHIA[8.230]~\cite{Sjostrand:2014zea}, using the A14 set of tuned
parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo] set of PDFs~\cite{Ball:2012cx}.
Top quarks were decayed at LO using
\MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin
correlations. The decays of bottom and charm hadrons were simulated
using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.  The parton-shower starting
scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined as the scalar sum of the \pT of all outgoing partons.
The renormalisation and factorisation scale choice was the same as for the
\POWHEGBOX set-up.

\subsection[MadGraph5\_aMC@NLO+Herwig7.13]{\MGNLOHER[7.13]}
%\label{subsubsec:ttbar_aMCH713}

\paragraph{Samples}
%\label{par:ttbar_aMCH713_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_aMCH713}.
\begin{table}[htbp]
  \caption{\ttbar samples produced with \MGNLOHER[7.13].}%
  \label{tab:ttbar_aMCH713}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412116 & \ttbar single lepton \\
    412117 & \ttbar dileptonic \\
    412175 & \ttbar all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

To assess the uncertainty in the matching of NLO matrix elements to the
parton shower, a sample produced with the
\POWHEGBOX[v2]
generator was compared with a sample generated with \MGNLO[2.6.0]~\cite{Alwall:2014hca}, both using the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) and interfaced with
\HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the \HERWIG[7.1] default set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa}.
The decays of bottom and charm hadrons
were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

To assess the uncertainty in the matching of NLO matrix elements to the parton shower,
a \POWHEG sample was compared with a sample generated by \MGNLO~\cite{Alwall:2014hca}.
The first sample was produced with the same hard-scatter set-up as the nominal sample using the
\POWHEGBOX[v2]~\cite{Frixione:2007nw,Nason:2004rx,Frixione:2007vw,Alioli:2010xd}
generator, which provided matrix elements at next-to-leading
order~(NLO) in the strong coupling constant \alphas, with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF) and
the \hdamp parameter set to 1.5\,\mtop~\cite{ATL-PHYS-PUB-2016-020}.
The functional form of the renormalisation and factorisation scales was
set to the default scale \(\sqrt{\mtop^{2} + \pTX[2]}\).
The second sample used \MGNLO[2.6.0] with the
\NNPDF[3.0nlo]~\cite{Ball:2014uwa} PDF set for the calculation of the hard-scattering.
Top quarks were decayed at LO using
\MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve spin
correlations. The parton-shower starting
scale had the functional form \(\muQ = \HT/2\)~\cite{ATL-PHYS-PUB-2017-007},
where \HT is defined
as the scalar sum of the \pT of all outgoing partons.
The events from both generators were interfaced with
\HERWIG[7.13]~\cite{Bahr:2008pv,Bellm:2015jjp}, using the \HERWIG[7.1] default set
of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set
\cite{Harland-Lang:2014zoa}.
The renormalisation and factorisation scale choice in the \MGNLO set-up was the same as for the
\POWHEGBOX set-up. The decays of bottom and charm hadrons were simulated
using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf} in both set-ups.


\subsection[Sherpa 2.2.1]{\SHERPA[2.2.1]}
\label{subsubsec:ttbar_sherpa}

\paragraph{Samples}
%\label{par:ttbar_sherpa_samples}

The descriptions below correspond to the samples in \cref{tab:ttbar_sherpa}.
\begin{table}[htbp]
  \caption{\ttbar samples produced with \SHERPA[2.2.1].}%
  \label{tab:ttbar_sherpa}
  \centering
  \begin{tabular}{l l}
  \toprule
  DSID range & Description \\
  \midrule
  410249 & \ttbar all-hadronic  \\
  410250 & \ttbar single lepton  \\
  410251 & \ttbar single lepton  \\
  410252 & \ttbar dileptonic  \\
  \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Additional samples of \ttbar events were produced with the
\SHERPA[2.2.1]~\cite{Bothmann:2019yzt} generator using NLO-accurate
matrix elements for up to one additional parton, and LO-accurate
matrix elements for up to four additional partons calculated with the
Comix~\cite{Gleisberg:2008fv} and
\OPENLOOPS~\cite{Buccioni:2019sur,Cascioli:2011va,Denner:2016kdg} libraries. They were
matched with the \SHERPA parton shower~\cite{Schumann:2007mg} using
the \MEPSatNLO
prescription~\cite{Hoeche:2011fd,Hoeche:2012yf,Catani:2001cc,Hoeche:2009rj}
and the set of tuned parameters developed by the \SHERPA authors
to match the \NNPDF[3.0nnlo] set of PDFs~\cite{Ball:2014uwa}.

\textbf{Additional information}: The central scale had the functional
form \(\mu^{2} = \mtop^{2} + 0.5\times(\pTX[2][t]p + \pTX[2][\bar{t}])\).
The CKKW matching scale of the
additional emissions was set to \SI{30}{\GeV}.


==> template/MC_snippets/ttgamma.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              ttgamma                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\ttgamma production]{\ttgamma production}
\label{subsec:ttgamma}

This section describes the MC samples used for the modelling of \ttgamma\ production.
\Cref{subsubsec:ttgamma_aMCP8} describes the \MGNLOPY[8] samples,
and \cref{subsubsec:ttgamma_aMCH7} describes the \MGNLOHER[7] samples.

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:ttgamma_aMCP8}

\paragraph{Samples}
%\label{par:ttgamma_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:ttgamma_aMCP8,tab:ttgamma_aMCP8_addRad}.

\begin{table}[htbp]
  \caption{Nominal \ttgamma\ samples produced with \MGNLOPY[8].}%
  \label{tab:ttgamma_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410389 & \ttgamma, non-all-hadronic \\
    410394 & \ttgamma, all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[htbp]
  \caption{\ttgamma\ samples produced with \MGNLOPY[8] used to estimate initial-state radiation systematic uncertainties.}%
  \label{tab:ttgamma_aMCP8_addRad}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410404 & \ttgamma\, non-all-hadronic, A14Var3c up \\
    410405 & \ttgamma\, non-all-hadronic, A14Var3c down \\
    410410 & \ttgamma\, all-hadronic, A14Var3c up \\
    410411 & \ttgamma\, all-hadronic, A14Var3c down \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \ttgamma events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at LO with the \NNPDF[2.3lo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.212]~\cite{Sjostrand:2014zea} using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The uncertainty due to initial-state radiation (ISR) was estimated by
comparing the nominal \ttgamma sample with two additional samples,
where the Var3c up/down variations of the A14 tune were employed.


\paragraph{Long description:}

The \ttgamma sample was simulated as a 2\(\to\)7 process at LO including the decay of the top quarks by
\MGNLO[2.3.3]~\cite{Alwall:2014hca} with the \NNPDF[2.3lo]~\cite{Ball:2014uwa} parton distribution function~(PDF), interfaced with
\PYTHIA[8.212]~\cite{Sjostrand:2014zea}, using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set. The photon could be radiated from an initial charged parton, an intermediate top quark,
or any of the charged final-state particles. The top-quark mass, top-quark decay width, \(W\)-boson decay width,
and fine structure constant were set to \SI{172.5}{\GeV}, \SI{1.320}{\GeV}, \SI{2.085}{\GeV}, and 1/137, respectively.
The five-flavour scheme was used, where all the quark masses are set to zero, except for the top quark. The renormalisation and the
factorisation scales were set to \(0.5\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\), where the sum runs over all the particles generated
from the matrix element calculation.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.

The cross-section was calculated at NLO in QCD as reported in Ref.~\cite{Melnikov:2011ta}, resulting in a \(K\)-factor of 1.24 which was applied
to the samples, with a relative uncertainty of 14\% from variations of renormalisation and factorisation scales as well
as the choice of PDF set.

The uncertainty due to initial-state radiation (ISR) was estimated by comparing the nominal \ttV\ sample with two additional samples,
 which had the same settings as the nominal one, but employed the Var3c up or down variation of the A14 tune, which
corresponds to the variation of \alphas for initial-state radiation (ISR) in the A14 tune.

To evaluate the effect of renormalisation and factorisation scale uncertainties, the two scales were varied simultaneously by factors 2.0 and 0.5.
To evaluate the PDF uncertainties for the nominal PDF, the 100 replicas for \NNPDF[2.3lo] were taken into account.


\subsection[MadGraph5\_aMC@NLO+Herwig7]{\MGNLOHER[7]}
\label{subsubsec:ttgamma_aMCH7}

\paragraph{Samples}
%\label{par:ttgamma_aMCH7_samples}

The descriptions below correspond to the samples in \cref{tab:ttgamma_aMCH7}.

\begin{table}[htbp]
  \caption{\ttgamma\ samples produced with \MGNLOHER[7].}%
  \label{tab:ttgamma_aMCH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    410395 & \ttgamma non-all-hadronic \\
    410396 & \ttgamma all-hadronic \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

Additional \ttgamma samples were produced with the parton shower of the nominal samples replaced by
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp} to evaluate the impact of using using a different parton shower and hadronisation model.
The H7UE set of tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa} were used.


==> template/MC_snippets/tttt.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%              tttt                    %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section[\tttt production]{\tttt production}
\label{subsec:tttt}

This section describes the MC samples used for the modelling of \tttt\ production.
\Cref{subsubsec:tttt_aMCP8} describes the \MGNLOPY[8] samples,
and \cref{subsubsec:tttt_aMCH7} describes the \MGNLOHER[7] samples.

\subsection[MadGraph5\_aMC@NLO+Pythia8]{\MGNLOPY[8]}
\label{subsubsec:tttt_aMCP8}

\paragraph{Samples}
%\label{par:tttt_aMCP8_samples}

The descriptions below correspond to the samples in \cref{tab:tttt_aMCP8}.

\begin{table}[htbp]
  \caption{Nominal \tttt\ samples produced with \MGNLOPY[8].}%
  \label{tab:tttt_aMCP8}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412043 & \tttt \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Short description:}

The production of \tttt\ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator at NLO with the \NNPDF[3.1nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea}~ using the A14 tune~\cite{ATL-PHYS-PUB-2014-021} and the
\NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\paragraph{Long description:}

The production of \tttt\ events was modelled using the \MGNLO[2.3.3]~\cite{Alwall:2014hca}
generator, which provided matrix elements at next-to-leading order~(NLO) in the strong coupling constant \alphas
with the \NNPDF[3.1nlo]~\cite{Ball:2014uwa} parton distribution function~(PDF).
The functional form of the renormalisation and factorisation scales was set to \(0.25\times \sum_i \sqrt{m^2_i+p^2_{\text{T},i}}\),
where the sum runs over all the particles generated from the matrix element calculation, following the Ref.~\cite{Frederix:2017wme}.
Top quarks were decayed at LO using \MADSPIN~\cite{Frixione:2007zp,Artoisenet:2012st} to preserve all spin correlations.
The events were interfaced with \PYTHIA[8.230]~\cite{Sjostrand:2014zea} for the parton shower and hadronisation,
using the A14 set of tuned parameters~\cite{ATL-PHYS-PUB-2014-021} and the \NNPDF[2.3lo]~\cite{Ball:2014uwa} PDF set.
The decays of bottom and charm hadrons were simulated using the \EVTGEN[1.6.0] program~\cite{Lange:2001uf}.


\subsection[MadGraph5\_aMC@NLO+Herwig7]{\MGNLOHER[7]}
\label{subsubsec:tttt_aMCH7}

\paragraph{Samples}
%\label{par:tttt_aMCH7_samples}

The descriptions below correspond to the samples in \cref{tab:tttt_aMCH7}.

\begin{table}[htbp]
  \caption{\tttt\ samples produced with \MGNLOHER[7].}%
  \label{tab:tttt_aMCH7}
  \centering
  \begin{tabular}{l l}
    \toprule
    DSID range & Description \\
    \midrule
    412044 & \tttt \\
    \bottomrule
  \end{tabular}
\end{table}

\paragraph{Description:}

Additional \tttt\ samples were produced with the parton shower of the nominal samples replaced by
\HERWIG[7.04]~\cite{Bahr:2008pv,Bellm:2015jjp} to evaluate the impact of using a different parton shower and hadronisation model. The H7UE set of
tuned parameters~\cite{Bellm:2015jjp} and the \MMHT[lo] PDF set~\cite{Harland-Lang:2014zoa} were used.


==> template/SUSY/executive_summary.tex <==
\section{Executive Summary}

This section, ideally less than two pages, should be placed at the beginning of the supporting note.
It should give a high-level overview of the analysis including (but not limited to):
\begin{itemize}
\item physics target and the general characteristics of the signal;
\item analysis strategy;
\item general characteristics of the control, validation, and signal regions;
\item a background estimation strategy overview;
\item highlights of major or most important points of the analysis;
\item a table or list of all critical tasks and who is responsible for each.
\end{itemize}

This section should include explicit pointers to the items required for the PAR and FAR\@.  For reference, those items are listed below. Please feel free to modify these lists into references to document sections.

For a PAR (ed board request), the SUSY group looks for:
\begin{itemize}
\item A definition of the target scenarios
\item A brief run-down of the signal grids, in particular pointing to any production problems or places where the production has not yet begun
\item A discussion of any non-standard object definitions in the analysis, and any on-going development that might affect the object definition
\item A discussion of the derivations: whether any reprocessing is needed, and whether the required samples have been requested
\item Data/MC comparisons in some inclusive regions (demonstrating the technical ability to use the data from all periods in the team's framework)
\item Any signal region definitions that are available, with some preliminary optimization in place and some description of the optimization procedure
\item Plans for further optimization (e.g.\ optimization for different model space regions, or use of an MVA or multi-bin fit)
\item An outline of the plans to get from here to a paper (plan of work, noting if person power is insufficient for any of the areas), as a part of this summary
\item An explicit list of differences in object definitions from the recommendations of the \href{https://gitlab.cern.ch/atlas-phys-susy-wg/Combinations/readme/wikis/home}{Combination Team}, with justification.
\item The location of the analysis code in GIT and demonstration that you have set up containers (\href{https://recast-docs.web.cern.ch/recast-docs/building_images_on_ci/}{described here}).
\end{itemize}

If you are using SUSYTools, please include the current configuration file in the \href{http://gitlab.cern.ch/atlas-phys-susy-wg/AnalysisSUSYToolsConfigurations}{archive}.

For a FAR, the SUSY group looks for:
\begin{itemize}
\item Definitions of SR, CR, VR, including expected yields with the targeted luminosity for all backgrounds that will be estimated with transfer factors or pure MC\@.
    Include signal contamination in CR and VR\@.
\item Cutflow for the background and for representative signal points.
\item Outline of background estimation strategies, including validation and closure tests for data-driven estimations. Statistical uncertainties for transfer-factor (TF) estimated and data-driven estimated backgrounds.
\item Comparison of data and MC with the relevant dataset in CR and VR\@. Strategy for mitigation of mis-modelling wherever needed with proof of feasibility.
\item Estimate of the detector level systematic uncertainties through propagation of CP recommendations.
\item A clear statement on how all others systematic uncertainties will be evaluated, including theory uncertainties on both backgrounds and signal: all the procedures need to be defined before unblinding.
\item A clear plan for ``discovery regions'' as well as the statistical treatment of the signal regions.
\item Background only fit with pull plot for the nuisance parameters.
\item Estimated exclusion, including depth of exclusion within the normal exclusion contour, with Asimov fit.
\item To-do list for achieving final result and possible bottlenecks (can the rest of the SUSY WG help with anything?)
\item For analyses using machine learning methods, additional diagnostics are required, which are explained \href{https://twiki.cern.ch/twiki/bin/view/AtlasProtected/SusyMachineLearning}{here}.
\item The location in GIT where your code is using containers and the first implementation of workflows towards recast (\href{https://recast-docs.web.cern.ch/recast-docs/workflowauthoring/intro/}{described here}).
\end{itemize}

The background forum recommends the following diagnostic plots:
\begin{itemize}
\item Standard occupancy maps and plots that can reveal detector or non-collision background issues --- plot for CRs, VRs and SRs of MET phi, the leading jet and/or leading lepton eta vs.\ phi 2D map, and the leading jet and/or leading lepton phi distributions
\item Selection efficiencies as a function of mu (VR, SR, and CR): to check how dependent the analysis is on pileup (primarily for MC)
\item Run number and data period dependencies: plot lumi-normalized yields in CRs, VRs and SRs as a function of the run number and data period (data only).
    This is to check for potential temporary issues in the data present only for certain runs, and to reveal potential chunks of data not processed by mistake.
    You should normalize the per-run yield using the lumi as reported from an independent source (not the in-file metadata!),
    e.g.\ simply use \href{https://svnweb.cern.ch/trac/atlasoff/browser/PhysicsAnalysis/SUSYPhys/SUSYTools/trunk/scripts/ilumi2histo.py}{this script in SUSYTools} to build the luminosity-vs-run histogram from your \texttt{iLumiCalc} file.
\item In particular, for Full Run 2 dataset analyses, a plot of data from 2018 vs period, specifically to compare the efficiencies for the period with two dead tile modules to the periods without.
\item Check for missing data: Compare the total number of processed data events and compare to the reference numbers for the combination of GRL and derivation you're running over in \href{https://docs.google.com/spreadsheets/d/1LMioo0nvALkKgoCKRW_ihQThHyVwcOQVRJe4aXiENUs/edit#gid=424865170}{this spreadsheet}. If your total does not match this reference number, feel free to contact BG forum conveners and derivation contacts for help with debugging.
\item Check for duplicated events: several bugs in MC and DAOD production have caused duplicated events to appear in the derivations in the past. This can potentially happen in both MC and data. Please check that there are no duplicated events in your CRs, VRs or SRs. If you notice duplicated events in your derivations, please get in touch with the Background Forum conveners immediately.
\item Comparisons of data and MC in the CRs and VRs, as well as MC in the SRs, for 2015+2016, 2017, and 2018 separately, for key distributions and yields.
\item Debug stream yields in SR and CR\@. The full name of the debug stream is \texttt{debugrec\_hlt}, and derivation datasets can be found for both 2015 and 2016 data with a query like \texttt{rucio ls --short --filter type=container data*\_13TeV.00*.debugrec\_hlt*DAOD\_SUSY1*p2709*}.
\item Pileup reweighting check: plot the nvtx distribution before and after pileup reweighting (data Vs MC). Purpose: check that the pileup reweighting works as intended.
\end{itemize}

Again, if you are using SUSYTools, please include the current configuration file in the \href{http://gitlab.cern.ch/atlas-phys-susy-wg/AnalysisSUSYToolsConfigurations}{archive}.  Please also take care that you have looked into the \href{https://twiki.cern.ch/twiki/bin/viewauth/Atlas/DataPreparationCheckListForPhysicsAnalysis}{items recommended by DataPrep}.


==> template/atlas-auxmat.tex <==
\part*{Auxiliary material}
\addcontentsline{toc}{part}{Auxiliary material}
%-------------------------------------------------------------------------------

In an ATLAS paper, auxiliary plots and tables that are supposed to be made public 
should be collected in an appendix that has the title \enquote{Auxiliary material}.
This information will appear on the public webpage, but will not be included
in the document submitted to arXiv and to the journal.


==> template/atlas-detector.tex <==
% Footnote with ATLAS coordinate system
\newcommand{\AtlasCoordFootnote}{%
ATLAS uses a right-handed coordinate system with its origin at the nominal interaction point (IP)
in the centre of the detector and the \(z\)-axis along the beam pipe.
The \(x\)-axis points from the IP to the centre of the LHC ring,
and the \(y\)-axis points upwards.
Cylindrical coordinates \((r,\phi)\) are used in the transverse plane, 
\(\phi\) being the azimuthal angle around the \(z\)-axis.
The pseudorapidity is defined in terms of the polar angle \(\theta\) as \(\eta = -\ln \tan(\theta/2)\).
Angular distance is measured in units of \(\Delta R \equiv \sqrt{(\Delta\eta)^{2} + (\Delta\phi)^{2}}\).}

%-------------------------------------------------------------------------------
\subsection{Run 2 ATLAS detector example for a Letter}
\label{sec:atlas2a}
%-------------------------------------------------------------------------------

The ATLAS experiment~\cite{PERF-2007-01} at the LHC is a multipurpose particle detector
with a forward--backward symmetric cylindrical geometry and a near \(4\pi\) coverage in 
solid angle.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid
providing a \SI{2}{\tesla} axial magnetic field, electromagnetic and hadron calorimeters, and a muon spectrometer.
The inner tracking detector covers the pseudorapidity range \(|\eta| < 2.5\).
It consists of silicon pixel, silicon microstrip, and transition radiation tracking detectors.
Lead/liquid-argon (LAr) sampling calorimeters provide electromagnetic (EM) energy measurements
with high granularity.
A steel/scintillator-tile hadron calorimeter covers the central pseudorapidity range (\(|\eta| < 1.7\)).
The endcap and forward regions are instrumented with LAr calorimeters
for both the EM and hadronic energy measurements up to \(|\eta| = 4.9\).
The muon spectrometer surrounds the calorimeters and is based on
three large superconducting air-core toroidal magnets with eight coils each.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
The muon spectrometer includes a system of precision tracking chambers and fast detectors for triggering.
A two-level trigger system is used to select events.
The first-level trigger is implemented in hardware and uses a subset of the detector information
to accept events at a rate below \SI{100}{\kHz}.
This is followed by a software-based trigger that
reduces the accepted event rate to \SI{1}{\kHz} on average
depending on the data-taking conditions.
An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.

%-------------------------------------------------------------------------------
\subsection{Run 2 ATLAS detector example for a paper making use of the whole detector}
\label{sec:atlas2b}
%-------------------------------------------------------------------------------

The ATLAS detector~\cite{PERF-2007-01} at the LHC covers nearly the entire solid angle around the collision point.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid, electromagnetic and hadron calorimeters,
and a muon spectrometer incorporating three large superconducting air-core toroidal magnets.

The inner-detector system (ID) is immersed in a \SI{2}{\tesla} axial magnetic field 
and provides charged-particle tracking in the range \(|\eta| < 2.5\).
The high-granularity silicon pixel detector covers the vertex region and typically provides four measurements per track, 
the first hit normally being in the insertable B-layer (IBL) installed before Run~2~\cite{ATLAS-TDR-19,PIX-2018-001}.
It is followed by the silicon microstrip tracker (SCT), which usually provides eight measurements per track.
These silicon detectors are complemented by the transition radiation tracker (TRT),
which enables radially extended track reconstruction up to \(|\eta| = 2.0\). 
The TRT also provides electron identification information 
based on the fraction of hits (typically 30 in total) above a higher energy-deposit threshold corresponding to transition radiation.

The calorimeter system covers the pseudorapidity range \(|\eta| < 4.9\).
Within the region \(|\eta|< 3.2\), electromagnetic calorimetry is provided by barrel and 
endcap high-granularity lead/liquid-argon (LAr) calorimeters,
with an additional thin LAr presampler covering \(|\eta| < 1.8\)
to correct for energy loss in material upstream of the calorimeters.
Hadron calorimetry is provided by the steel/scintillator-tile calorimeter,
segmented into three barrel structures within \(|\eta| < 1.7\), and two copper/LAr hadron endcap calorimeters.
The solid angle coverage is completed with forward copper/LAr and tungsten/LAr calorimeter modules
optimised for electromagnetic and hadronic energy measurements respectively.

The muon spectrometer (MS) comprises separate trigger and
high-precision tracking chambers measuring the deflection of muons in a magnetic field generated by the superconducting air-core toroidal magnets.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
Three layers of precision chambers, each consisting of layers of monitored drift tubes, covers the region \(|\eta| < 2.7\),
complemented by cathode-strip chambers in the forward region, where the background is highest.
The muon trigger system covers the range \(|\eta| < 2.4\) with resistive-plate chambers in the barrel, and thin-gap chambers in the endcap regions.

Interesting events are selected by the first-level trigger system implemented in custom hardware,
followed by selections made by algorithms implemented in software in the high-level trigger~\cite{TRIG-2016-01}. 
The first-level trigger accepts events from the \SI{40}{\MHz} bunch crossings at a rate below \SI{100}{\kHz},
which the high-level trigger further reduces in order to record events to disk at about \SI{1}{\kHz}.

An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.

%-------------------------------------------------------------------------------
\subsection{Run 1 ATLAS detector example for a Letter}
\label{sec:atlas1a}
%-------------------------------------------------------------------------------

The ATLAS experiment~\cite{PERF-2007-01} at the LHC is a multipurpose particle detector
with a forward--backward symmetric cylindrical geometry and a near \(4\pi\) coverage in 
solid angle.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid
providing a \SI{2}{\tesla} axial magnetic field, electromagnetic and hadron calorimeters, and a muon spectrometer.
The inner tracking detector covers the pseudorapidity range \(|\eta| < 2.5\).
It consists of silicon pixel, silicon microstrip, and transition radiation tracking detectors.
Lead/liquid-argon (LAr) sampling calorimeters provide electromagnetic (EM) energy measurements
with high granularity.
A steel/scintillator-tile hadron calorimeter covers the central pseudorapidity range (\(|\eta| < 1.7\)).
The endcap and forward regions are instrumented with LAr calorimeters
for both the EM and hadronic energy measurements up to \(|\eta| = 4.9\).
The muon spectrometer surrounds the calorimeters and is based on
three large superconducting air-core toroidal magnets with eight coils each.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
The muon spectrometer includes a system of precision tracking chambers and fast detectors for triggering.
A three-level trigger system is used to select events.
The first-level trigger is implemented in hardware and uses a subset of the detector information
to accept events at a rate of at most \SI{75}{\kilo\hertz}.
This is followed by two software-based trigger levels that
together reduce the accepted event rate to \SI{400}{\hertz} on average
depending on the data-taking conditions during 2012.
An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.


%-------------------------------------------------------------------------------
\subsection{Run 1 ATLAS detector example for a paper making use of the whole detector}
\label{sec:atlas1b}
%-------------------------------------------------------------------------------

The ATLAS detector~\cite{PERF-2007-01} at the LHC covers nearly the entire solid angle around the collision point.\footnote{\AtlasCoordFootnote}
It consists of an inner tracking detector surrounded by a thin superconducting solenoid, electromagnetic and hadron calorimeters,
and a muon spectrometer incorporating three large superconducting air-core toroidal magnets.

The inner-detector system (ID) is immersed in a \SI{2}{\tesla} axial magnetic field 
and provides charged-particle tracking in the range \(|\eta| < 2.5\).
The high-granularity silicon pixel detector covers the vertex region and typically provides three measurements per track, 
the first hit normally being in the innermost layer.
It is followed by the silicon microstrip tracker (SCT) which usually provides eight measurements per track.
These silicon detectors are complemented by the transition radiation tracker (TRT),
which enables radially extended track reconstruction up to \(|\eta| = 2.0\). 
The TRT also provides electron identification information 
based on the fraction of hits (typically 30 in total) above a higher energy-deposit threshold corresponding to transition radiation.

The calorimeter system covers the pseudorapidity range \(|\eta| < 4.9\).
Within the region \(|\eta|< 3.2\), electromagnetic calorimetry is provided by barrel and 
endcap high-granularity lead/liquid-argon (LAr) calorimeters,
with an additional thin LAr presampler covering \(|\eta| < 1.8\)
to correct for energy loss in material upstream of the calorimeters.
Hadron calorimetry is provided by the steel/scintillator-tile calorimeter,
segmented into three barrel structures within \(|\eta| < 1.7\), and two copper/LAr hadron endcap calorimeters.
The solid angle coverage is completed with forward copper/LAr and tungsten/LAr calorimeter modules
optimised for electromagnetic and hadronic energy measurements respectively.

The muon spectrometer (MS) comprises separate trigger and
high-precision tracking chambers measuring the deflection of muons in a magnetic field generated by the superconducting air-core toroidal magnets.
The field integral of the toroids ranges between \num{2.0} and \SI{6.0}{\tesla\metre}
across most of the detector. 
A set of precision chambers covers the region \(|\eta| < 2.7\) with three layers of monitored drift tubes,
complemented by cathode-strip chambers in the forward region, where the background is highest.
The muon trigger system covers the range \(|\eta| < 2.4\) with resistive-plate chambers in the barrel, and thin-gap chambers in the endcap regions.

A three-level trigger system is used to select interesting events~\cite{PERF-2011-02}.
The first-level trigger is implemented in hardware and uses a subset of detector information
to accept events at a design value rate of at most \SI{75}{\kHz}.
This is followed by two software-based trigger levels which together reduce the event rate to about \SI{400}{\Hz}.

An extensive software suite~\cite{ATL-SOFT-PUB-2021-001} is used in the reconstruction and analysis of real
and simulated data, in detector operations, and in the trigger and data acquisition systems of the experiment.



==> template/atlas-hepdata.tex <==
\section{HepData material}
%-------------------------------------------------------------------------------

This file is available for detailed tables etc.\ that are going to be
submitted to HepData or other similar destinations.

==> template/atlas-note-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used for an ATLAS note.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{AtlasTitle: Bare bones ATLAS note}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in the final version.
\AtlasVersion{0.1}

% Abstract - % directly after { is important for correct indentation.
\AtlasAbstract{%
  This is a bare bones ATLAS note. Put the abstract for the document here.
}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis.
% \AtlasAuthorContributor also adds the name to the author list.
% Include package latex/atlascontribute to use this.
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute.
% \usepackage{authblk}
% Use the following 3 lines to have all institutes on one line.
% \makeatletter
% \renewcommand\AB@affilsepx{, \protect\Affilfont}
% \makeatother
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting
% \AtlasAuthorContributor{First AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasAuthorContributor{Second AtlasAuthorContributor}{b}{Author's contribution.}
% \AtlasAuthorContributor{Third AtlasAuthorContributor}{a}{Author's contribution.}
% \AtlasContributor{Fourth AtlasContributor}{Contribution to the analysis.}
% \author[a]{First Author}
% \author[a]{Second Author}
% \author[b]{Third Author}
% \affil[a]{One Institution}
% \affil[b]{Another Institution}

% If a special author list should be indicated via a link use the following code:
% Include the two lines below if you do not use atlasstyle:
% \usepackage[marginal,hang]{footmisc}
% \setlength{\footnotemargin}{0.5em}
% Use the following lines in all cases:
% \usepackage{authblk}
% \author{The ATLAS Collaboration%
% \thanks{The full author list can be found at:\newline
%   \url{https://atlas.web.cern.ch/Atlas/PUBNOTES/ATL-PHYS-PUB-2021-XXX/authorlist.pdf}}
% }

% ATLAS reference code, to help ATLAS members to locate the paper.
\AtlasRefCode{GROUP-2021-XX}

% ATLAS note number. Can be an COM, INT, PUB or CONF note.
% \AtlasNote{ATLAS-CONF-2021-XXX}
% \AtlasNote{ATL-PHYS-PUB-2021-XXX}
% \AtlasNote{ATL-COM-PHYS-2021-XXX}


==> template/atlas-paper-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{AtlasTitle: Bare bones ATLAS document}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of every other page, 
% and line numbers.
% Comment or remove in the final version.
\AtlasVersion{0.1}

% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
  This is a bare bones ATLAS document. Put the abstract for the document here.
}

% Author - this does not work with revtex (add it after \begin{document})
% This has to be commented out for TDR etc.
% For PUB notes, add package authblk and use \thanks if an ACE/STA should be added.
% See Section 4.2 of ATLAS LaTeX guide for more details.
% \author{The ATLAS Collaboration}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GROUP-2021-XX}

% CERN preprint number
% \PreprintIdNumber{CERN-EP-2021-XX}

% ATLAS date - arXiv submission; usually filled in by the Physics Office
% \AtlasDate{\today}

% ATLAS heading - heading at top of title page. Set for TDR etc.
% \AtlasHeading{ATLAS ABC TDR}

% arXiv identifier
% \arXivId{21XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
% \AtlasJournal{Phys.\ Lett.\ B.}
% \AtlasJournalRef{\PLB 789 (2021) 123}
% \AtlasDOI{}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
% \AtlasCoverSupportingNote{Short title note 1}{https://cds.cern.ch/record/XXXXXXX}
% \AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
% \AtlasCoverCommentsDeadline{DD Month 2021}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
% \AtlasCoverAnalysisTeam{Peter Analyser, Susan Editor1, Jenny Editor2, Alphonse Physicien}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair), EB~Member~1, EB~Member~2, EB~Member~3}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverReaderMember{Reader~2}

% Editors egroup
% \AtlasCoverEgroupEditors{atlas-GROUP-2021-XX-editors@cern.ch}

% EdBoard egroup
% \AtlasCoverEgroupEdBoard{atlas-GROUP-2021-XX-editorial-board@cern.ch}

